Maintaining Consistency of Data on the Web

Increasingly more data is becoming available on the Web, estimates speaking of 1 billion documents in 2002. Most of the documents are Web pages whose data is considered to be in XML format, expecting it to eventually replace HTML. A common problem in designing and maintaining a Web site is that data on a Web page often replicates or derives from other data, the so-called base data, that is usually not contained in the deriving or replicating page. Consequently, replicas and derivations become inconsistent upon modifying base data in a Web page or a relational database. For example, after assigning a thesis to a student and modifying the Web page that describes it in detail, the thesis is still incorrectly contained in the list of offered thesis, missing in the list of ongoing thesis, and missing in the advisor's teaching record. The thesis presents a solution by proposing a combined approach that provides for maintaining consistency of data in Web pages that (i) replicate data in relational databases, or (ii) replicate or derive from data in Web pages. Upon modifying base data, the modification is immediately pushed to affected Web pages. There, maintenance is performed incrementally by only modifying the affected part of the page instead of re-generating the whole page from scratch.

==> abstract.tex <==
\chapter*{Abstract}

Increasingly more data is becoming available on the Web, estimates speaking of 1 billion documents in 2002. Most of the documents are Web pages whose data is considered to be in XML format, expecting it to eventually replace HTML, the current lingua franca of the Web, e.g., by XHTML.

A common {\em problem} in designing and maintaining a Web site is that data on a Web page often replicates or derives from other data, the so-called base data, that is usually not contained in the deriving or replicating page. 
Two properties of Web sites account for this situation. 
First, the hypertext structure of a Web site not necessarily coincides with the structure of its underlying conceptual domain model, thus it may be necessary to present a single data item on several pages. 
Second, the content of pre-generated Web pages is often drawn from legacy systems, usually relational databases. In this case Web pages replicate data items from databases.

Consequently, replicas and derivations become inconsistent upon modifying base data in a Web page or a relational database.
For {\em example}, after modifying a product's price in the database, already pre-generated Web pages offer the product at an out-dated price.
Or, after assigning a thesis to a student and modifying the Web page that describes it in detail, the thesis is still incorrectly contained in the list of offered thesis, missing in the list of ongoing thesis, and missing in the advisor's teaching record.

The thesis presents a {\em solution} by proposing a combined approach
that provides for maintaining consistency of data in Web pages that 
(i) replicate data in relational databases, or 
(ii) replicate or derive from data in Web pages.
Upon modifying base data, the modification is immediately pushed to affected Web pages. There, maintenance is performed incrementally by only modifying the affected part of the page instead of re-generating the whole page from scratch.

The proposed approach provides for consistent, up-to-date Web pages any time. 
It is efficient by providing incremental page maintenance techniques,
generic by maintaining consistency of XML data in general,
flexible by reacting to modifications in Web pages of other businesses, 
transparent by maintaining a business' autonomy in managing its data,
open by allowing future extensions to be built on top of it, 
and 
extensible by enabling the integration of arbitrary legacy systems. 



==> axs/axml-knowledge-model.tex <==
\section{Knowledge Model}

\begin{figure}
    \begin{center}
        \includegraphics{axml-ecomo/axs_metaschema-1}
        \caption{Active XML Schema package ``{\sf axs}''}
        \label{fig:uml-metamodel-axs}
    \end{center}
\end{figure} 

\begin{figure}
    \begin{center}
        \includegraphics{axml-ecomo/axs_metaschema-2}
        \caption{Passive Behavior package ``{\sf psv}''}
        \label{fig:uml-metamodel-psv}
    \end{center}
\end{figure} 

\begin{figure}
    \begin{center}
        \includegraphics{axml-ecomo/axs_metaschema-3}
        \caption{Active Behavior package ``{\sf act}''}
        \label{fig:uml-metamodel-act}
    \end{center}
\end{figure} 

@@filter is not described yet/is a description necessary?


\begin{figure}
    \begin{center}
        \includegraphics{axml-ecomo/axs_metaschema-4}
        \caption{Event Type package ``{\sf evts}''}
        \label{fig:uml-metamodel-evts}
    \end{center}
\end{figure} 

==> axs/index.tex <==
\newcommand{\axsdir}{./axs/}

The chapter presents the basic Active XML Schema (AXS) approach. More advanced topics regarding the AXS approach are discussed in the following Chapters~\ref{section:cevts} and \ref{section:implementing-the-km}.

First, basic concepts of provided active behavior are presented in Section~\ref{section:activeExtensionOfXMLSchema}. They comprise event types, event classes, import and export of events, and rules. 
Second, advanced concepts of AXS are discussed in Section~\ref{section:AdvancedConcepts}, comprising timestamping of events, scheduling events, composite and logical event classes, and exception rules. 
Third, the problem of defining an order on distributed events caused by possibly unsynchronized clocks in distributed environments and how it is dealt with in AXS is shown in Section~\ref{section:DistributedEvents}.
%
Fourth, Section~\ref{section:ManagingActiveXMLSchemas} concludes the chapter by discussing briefly how active XML Schemas can be managed.

% *************************************************************************
% *
% *************************************************************************

\section{Active Extension of XML Schema}
\label{section:activeExtensionOfXMLSchema}

Adhering to an object-oriented approach, XML Schemas are enriched with additional components to provide for active and passive behavior of XML documents. While several schema languages have been proposed recently (e.g., \cite{OASIS2001RelaxNG,Jell01a}) to replace XML 1.0 Document Type Definitions \cite{W3C1998XML}, we use XML Schema \cite{W3C2001XMLSchema1,W3C2001XMLSchema2}. 

An active XML Schema defines a distinguished global complex type, the {\em active document type}, that defines the structure and behavior of its instance documents. This is done by enriching a global complex type as defined by XML Schema with the definition and implementation of operations (i.e., passive behavior), with a set of definitions of event types and event classes, with a set of import and export statements defining the publication and subscription of event classes, and with a set of rules (i.e., active behavior).

To assure interoperability with legacy applications (i.e., applications that are not capable of interpreting active XML Schemas) the enrichments are transparent to those applications. Transparency is obtained by enriching complex type definitions via annotations that hold data defining active and passive behavior. XML schemas are instances of the XML Schema schema for XML Schemas (i.e., the metaschema \cite{W3C2001XMLSchema1}). To be able to validate an active XML Schema with a conventional XML Schema validator, this metaschema is enriched with metatype definitions for active and passive behavior, constituting the {\em Active XML Metaschema}. Like active XML schemas are instances of the active XML metaschema, active XML documents are instances of active XML schemas. They comprise, aside of static data, data representing events as well as subscriptions. These additions belong to a separate namespace, which is referenced by namespace-prefix {\sf act:} in this chapter.

Along with the description of Active XML Schema concepts we repeatedly formalize the according part of the metaschema by an UML class diagram showing the contents of the dedicated UML package. The intention is to clarify details and to provide a concise representation of the metaschema. The datatypes of attributes are those defined by XML Schema Datatypes. For brevity we omit the namespace name when referring to a type, e.g., instead of {\sf xs:QName} we write {\sf QName}.
The implementation of the metaschema in XML is discussed in Chapter~\ref{section:implementing-the-km}.

In the examples for active XML Schemas throughout the chapter we use 
two notation to depict active XML Schemas: UML and XML.
First, we use an extended UML \cite{Rumb99aUML} notation. This form of presentation is favored over object diagrams that model instances of the metaschema for conciseness. It is necessary to extend UML to model Active XML Schema concepts not originally present in UML. We introduce new compartments that an UML class can feature, and tag each compartment by a letter to reflect its semantics. While we do not use the compartments for structural attributes in the thesis, we tag the operation compartment by ``{\sf O}''. The newly introduced event class compartment is tagged by``{\sf E}'', the exported event class compartment by ``{\sf $\uparrow$}'', the imported event class compartment by ``{\sf $\downarrow$}'', and the rule compartment by ``{\sf R}''.
Second, XML snippets show the serialization of the active XML Schema examples as part of XML Schema documents. In these, unprefixed elements are in the default namespace of the Active XML Metaschema\footnote{which is \url{http://big.tuwien.ac.at/axs/metaschema/1.0}}, elements prefixed {\sf actf} are in the namespace of the Active XML Framework\footnote{which is \url{http://big.tuwien.ac.at/axs/framework/1.0}} (cf. Section~\ref{section:EmployingAMixedApproachForAXS}).

The metaschema for active document types is depicted in Figure~\ref{fig:uml-metamodel-axs}, which shows package \uml{axs}. It depicts active document type \uml{ActiveDocTp} specifying definitions and implementations of operations by \uml{psv::Interface} and \uml{psv::Implementation}, event types by \uml{evts::EventType}, event classes by \uml{evts::EventClass}, and rules by \uml{rule::Rule}. Regarding the import and export of event classes, \uml{ixe::Proxy} is the only metaschema class of package \uml{ixe} that is referenced in package \uml{axs}, the other necessary classes are derived from \uml{evts::EventType} and \uml{evts::EventClass}. For detailed descriptions of these concepts and the metaschema packages \uml{psv}, \uml{evts}, \uml{ixe}, \uml{rule}, and \uml{cle}, see the following sections.
An active document type has a \uml{name}, a \uml{targetNamespace} similar to an XML schema, and import/include relationships to other active document types, which have the same semantics as import/include relationships in XML Schema. Moreover, class \uml{NamespacePrefix} represents declared namespace prefixes that are used in defining the active document type, and
\uml{NativeCode} is an auxiliary datatype which describes an expression or source code in another, native language such as an XQuery expression or Java code. \uml{NativeCode} is used in other packages.

\begin{figure}
    \begin{center}
        \includegraphics[scale=1.25]{\axsdir metaschema_axs}
        \caption{Metaschema for Active XML Schema (Package {\sf axs})}
        \label{fig:uml-metamodel-axs}
    \end{center}
\end{figure} 

In the following, we describe the basic behavioral components of Active XML Schema.

\subsection{Passive Behavior}
\label{section:AXS.PassiveBehavior}

So far passive behavior for XML documents is specified procedurally, i.e. separately from the data, falling behind the prevailing object-oriented paradigm that integrates structure with behavior. This is the case with DOM, SAX, or XSLT \cite{Clar99aW3C}. However, XML databinding can be utilized to narrow the gap between definition of data and behavior. In particular Sun's JAXB \cite{Sun2004JAXB} can be used to define a mapping from XML to Java classes, behavior can be added by extending these classes. 

Whereas XML databinding does not allow to integrate the definition of data and behavior, active XML Schemas define operations at XML document types in an object-oriented manner. They enrich XML types, which before described only structure, with passive behavior. Interfaces and implementations of operations are separated as in common practice in object oriented design. 

In this chapter, implementations are illustrated by XSLT templates, which can access an operation's parameters via variables. They are, before being applied to an active XML document, embedded into a default stylesheet that performs a carbon copy (they override the default stylesheet's templates). The transformation's output document replaces the original active XML document, thus performing the modification as described by the operation's templates.

The metaschema for passive behavior is depicted in Figure~\ref{fig:uml-metamodel-psv}, which shows package \uml{psv}. An active document type may define several interfaces (class \uml{Interface}) and implementations (class \uml{Implementation}), where each implementation realizes a single interface, which is possibly defined by a different active document type. As in object-oriented programming languages, an interface defines a set of operations (class \uml{Operation}), where each of them is described by its name, parameters (attribute \uml{params} of datatype \uml{ParamTp}), and return type. For every operation, up to two operation event types can be defined (see Subsection~\ref{section:event-types-and-classes}). Operations defined by interfaces have according implementations (class \uml{OperationImpl}), an implementation is obliged to implement all operations defined by its interface (expressed by the constraint in the figure's bottom left).

\begin{figure}[h]
    \begin{center}
        \includegraphics[scale=1.25]{\axsdir metaschema_psv}
        \caption{Metaschema for Passive Behavior (Package {\sf psv})}
        \label{fig:uml-metamodel-psv}
    \end{center}
\end{figure} 

\begin{example}
\label{example:axs.job-agency}
A job agency provides an active XML Schema defining active document type {\sf j:JobAnnounce} and a document {\sf academicJobs.xml} having that type, which comprises a list of current job offers (cf. Figure~\ref{exOperationAndMaterialization}). A new job offer is announced by the invocation of operation {\sf announce(j:Job)}, which adds a new job offer at the end of the list.
The part of the active XML Schema document representing document type {\sf j:JobAnnounce} that defines the interface of operation {\sf announce(j:Job)} is depicted in snippet {\sf 1a}. The operation's implementation with XSLT is depicted in snippet {\sf 1b}. The type or object a snippet is part of, is represented by references to snippets in the extended UML model.
\end{example}

\begin{sidewaysfigure}
    \begin{center}
        \includegraphics[scale=1.05]{\axsdir ex_operation_and_materialization} 
        \caption{Operations and Event Classes at Schema and Instance Layer}
        \label{exOperationAndMaterialization}
    \end{center}
\end{sidewaysfigure}

% *************************************************************************

\subsection{Event Types and Event Classes}
\label{section:event-types-and-classes}

Events are happenings of interest to a document. They are collected into event classes and are stored with documents as ``first class XML elements'' as any other XML element. 
Each event class has a member type that defines the structure of its member events.

Events can be distinguished into several {\em event categories}, which are: mutation events, operation events, calendar events, abstract events, and imported events. 
\begin{itemize}
\item {\em Operation events} reflect the execution of an operation. 
%
\item {\em Mutation events} reflect changes to XML documents as according to the DOM Level 2 Event Module Specification. They are relevant in particular when a document is manipulated by means of legacy applications and not by predefined operations. Because the mutation events provided by the DOM Event Module may be too fine-grained fine-grained for directly defining rules on them, an approach has been developed to combine these events to so called composite mutation events, or short composite events (see Chapter~\ref{section:cevts}).
%
\item {\em Calendar events} constitute past, current, or future calendar entries.
%
\item {\em Abstract events} comprise any other event explicitly raised or scheduled by users or rules.
%
\item {\em Imported events} wrap remote events and are discussed in the next subsection.
\end{itemize}

Event types form a type hierarchy. The hierarchy at the metaschema layer (M2) is depicted in Figure~\ref{fig:uml-metamodel-evts} and is described in detail later in this section. Instances of the metaschema layer represent event types at the schema layer (M1). Instances of event types at M1 represent occurred events.
Event types at M1 form a type hierarchy which is not shown for space limitations. Each event type at M1 defines various {\em parameters} reflecting the environmental setting in which it occurs. E.g., an operation event type will provide a parameter for each of the operation's parameters. The root event type defines the lowest common denominator of parameters (such as an identifier and an occurrence timestamp). For examples of event types at M1 see Subsection~\ref{section:FrameworkApproach} and Section~\ref{section:EmployingAMixedApproachForAXS}.

An event class is either a basic event class or a queried event class. The extension of a basic event class is defined by collecting every detected event of its member type. The extension of a queried event class is defined by a query over other event classes. A queried event class is either a composite event class or a logical event class which are discussed in Subsection~\ref{section:LogicalEventClasses}.

Events are stored as ``first class elements''. As such they are part of a document and are thus persistent.
%Constituting ``first class elements'', events are stored as members of event classes with XML documents and are, thus, persistent. 
This is different to most active database systems, whose events have a life span ending with the transaction in which they occurred. The extensions of all event classes of a document reflect the document's {\em event history}. 
Rules can query event classes and, thus, react according to the event history reflecting the document's past as well as the documents future as determined by scheduled events.

Event classes are modelled explicitly at the schema layer with document types and define the collections of events that are of interest at the instance layer. When an event class is defined with a document type, each document instance of that document type will maintain its extension of the event class.

The metaschema for event types and event classes is depicted in Figure~\ref{fig:uml-metamodel-evts}, which shows package \uml{evts}. An active document type defines several event types and event classes, represented by instances of classes \uml{EventType} and \uml{EventClass} respectively.
Every event class has a name (attribute \uml{name}), may be exported (indicated by attribute \uml{exported}), and has an event type as its member type (association \uml{hasMemberType}). An event class's name must be unique within all event classes of an active document type.
Class \uml{EventType} is the root of the type hierarchy of event types at the metaschema layer. Its name (attribute \uml{name}) must be unique like the name of an event class.
Its subclasses reflect the event categories mentioned above: 

\begin{itemize}
\item Operation events are represented by the {\em operation event type}, \uml{OperationEvtTp}. For a single operation (class \uml{psv::Operation}) up to two operation event types can be defined per active document type, one for events that occur before and one for events that occur after the execution of the operation.

\item Mutation events are represented by the {\em mutation event type}, \uml{MutationEvtTp}. Events of a mutation event type occur in a certain part of the document defined by the event type's path type (attribute \uml{pathTp}). Subclass \uml{PrimitiveMutEvtTp} describes so called primitive mutation events, which reflect modifications of an XML document's contents, e.g., as defined by the DOM Event Module, while subclass \uml{CompositeMutEvtTp} represents composite mutation events, which are detected according to the declarative specification of the accompanying composite event class. For details on composite events see Chapter~\ref{section:cevts}, for details on composite event classes see Subsection~\ref{section:LogicalEventClasses}.

\item Calendar events are represented by the {\em calendar event type}, \uml{CalendarEvtTp}. Calendar events can be either periodical (class \uml{PeriodicCalEvtTp}), meaning that they occur between a start time and an end time every given interval, or absolute (class \uml{AbsoluteCalEvtTp}) meaning that the event occurs at a single point in time. Undefined calendar event types (class \uml{UndefinedCalEvtTp}) are special in that their events are not specified at the schema layer. Instead, absolute events can be raised in event classes having this member type, e.g., by a rule's actions. Special control events, which again can be raised, e.g., by a rule's action, allow to initiate and cancel periodic events that occur in such event classes.

\item Abstract events are represented by the {\em abstract event type}, \uml{AbstractEvtTp}. The serialization of events of an abstract event type must accord to the schema defined in attribute \uml{instanceSpec} which is expressed using the schema language identified by \uml{instanceSpec.lang}.

\item Finally, imported events are represented by the {\em imported event type}, \uml{ixe::ImportedEvtTp}. For details see (the following) Subsection~\ref{section:im-export-ecs} and Figure~\ref{fig:uml-metamodel-ixe} therein.
\end{itemize}

\begin{sidewaysfigure}
    \begin{center}
        \includegraphics[scale=1.25]{\axsdir metaschema_evts}
        \caption{Metaschema for Event Types and Event Classes (Package {\sf evts})}
        \label{fig:uml-metamodel-evts}
    \end{center}
\end{sidewaysfigure} 

\begin{example}
\label{example:axs.ec-announce}
Figure~\ref{exOperationAndMaterialization} shows the definition of event class {\sf announce} with document type {\sf j:JobAnnounce}, collecting all {\sf announce} operation events representing invocations of operation {\sf announce}  (cf. snippet {\sf 2}), and the materialization of this event class in document instance {\sf acadamicJobs.xml} (cf. snippet {\sf 3}).
\end{example}

Storing occurred events with documents as first class XML elements causes the documents to grow in size with modifications to them. To control a document's size, one can express size constraints on event classes and the document as a whole, which are enforced by the reactive service the document is stored at (see Subsection~\ref{section:AXS.ReactiveService}). If the constraints on event classes are satisfied, but the one on the document is not, the reactive service enforces the latter constraint by following some procedure to reduce the size of event classes. A size constraint on an event class can be specified in terms of maximum kilobytes, number of events, or age. The latter can only be enforced if the location provides time service level {\sf tsl-2} or {\sf tsl-3}. A size constraint on a document can be specified in terms of maximum kilobytes.

\subsection{Import and Export of Event Classes}
\label{section:im-export-ecs}
\input{axs/import-export}

\subsection{Rules}
\label{section:axs-rules}
\input{axs/rules}


\section{Advanced Concepts}
\label{section:AdvancedConcepts}

In this section, we motivate and discuss advanced concepts of Active XML Schema: event timestamps, scheduling events, composite and logical events, and exception rules.

\subsection{Event Timestamps}

When an event occurs (at its {\em occurrence time}) that is stored in an exported event class, it is subsequently delivered to subscribing documents.
Such a communication is characterized by two timestamps, the {\em publication time}, which records the time when the remote document publishes the event, and the {\em delivery time}, which records the time the event is delivered.
These timestamps may be of different importance to different applications, like the time of the post mark (corresponding to publication time) is relevant to meet the deadline of a postal vote or the time of delivery to meet an application deadline.

To comply with these three notions of timestamps, every local event is described by an occurrence time while every imported event is described by all three timestamps.
%An imported event type, which wraps the member type of a remote event class, provides for the recording of these two timestamps. 
The occurrence time of an imported event reflects the time the event is stored in the imported event class opposed to the other two timestamps which describe the communication.
%
An example given later shows how the distinction between publication time and delivery time can be used in an exception rule. 

Timestamps are defined with event types at the schema layer, as already mentioned in Subsection~\ref{section:event-types-and-classes}. How this can be done is discussed in Chapter~\ref{section:implementing-the-km} in detail, which briefly describes how it has been done in Section~\ref{section:EmployingAMixedApproachForAXS}.
As will be shown in more detail in Subsection~\ref{section:timeSvcLevels}, a timestamp comprises several components, recording, e.g., a logical clock count and a physical clock count.

\subsection{Scheduling Events}
\label{section:SchedulingEvents}

Comprehensive support for web content management requires not only to handle event occurrences
that were caused by modifications to the document or were explicitly raised, but also to schedule events in the future. 
A typical application is to schedule an event in the future to trigger removal of then outdated content.
%E.g., one may schedule an event that triggers the removal of then out-dated content. 
With active XML Schemas, events can be scheduled by operations or rules. Such a {\em scheduled event} has an occurrence time in the future.
% and its status ``scheduled'', as long its occurrence time is in the future or its actual occurrence has not been detected.

\begin{example}
To remove a job offer from a faculty's document when its application deadline is over, rule {\sf scheduleJobRemovalRule} is defined on event class {\sf postJob}, which collects invocations of operation {\sf postJob(j:Job)} (as depicted in Figure~\ref{fig:ExScheduleEvent}). The rule schedules the removal of a job offer by adding an event that is scheduled to occur when the application deadline ends to event class {\sf jobExpired}. Rule {\sf removeJobRule} defined on event class {\sf jobExpired} removes an expired job offer, whose identifier was bound to the event, by invoking operation {\sf unpostJob(xs:ID)}.
\end{example}

\begin{sidewaysfigure}
    \begin{center}
        \includegraphics[scale=1.05]{axs/ex_scheduleevent.eps}
        \caption{Scheduling an Event}
        \label{fig:ExScheduleEvent}
    \end{center}
\end{sidewaysfigure}

% ##########

\subsection{Composite and Logical Events}
\label{section:LogicalEventClasses}
\input{axs/logical}

\subsection{Exception Rules}

Situations that do not constitute ``standard'' situations during deployment of active XML Schemas may occur.
They originate in effects of an active XML Schemas' environment. In particular extraordinary behavior in communicating events between documents, such as the delayed delivery of a subscribed event, builds the ground for these situations.
Exceptional situations can be anticipated in schema design and should be dealt with by exception rules, providing a meaningful design distinction.
%While no additional concepts are necessary to model exception rules, it is a meaningful design design distinction to organize such rules into a seperate category.
No additional concepts are necessary to model exception rules. They react to specific logical events, which determine exceptional situations, and trigger necessary corrections.

\begin{example}
Figure~\ref{ExLogicalEC} shows event class {\sf pubDeliveredLate}, which collects exceptional situations, i.e. {\sf published} events that are delivered late. Exception rule {\sf redetermineActResRule} (cf. snippet {\sf 2}) defined on {\sf pubDeliveredLate} reacts to the late delivery by redetermining the researcher's active researcher status by invoking operation {\sf publishActResStatus}.
\end{example}

\input{axs/distributed-events}

\begin{figure}
    \begin{center}
        \includegraphics[scale=1.05]{\axsdir ex_distributed-evts}
        \caption{Distributed Events in AXS}
        \label{fig:AXS.ExampleDistributedEvents}
    \end{center}
\end{figure}

\begin{example}
An international corporation uses an extended version of active document type {\sf j:JobAnnounce} to announce internal job offers and scholarships for training programs at their subsidiaries in New York, Paris, and Vienna (as depicted in Figure~\ref{fig:AXS.ExampleDistributedEvents}, where event classes without any events are not shown for presentation purposes).
Offers for jobs and scholarships are published at the headquarters in Vienna ({\sf vienna.xml}) and replicated in the other subsidiaries ({\sf paris.xml} and {\sf nyc.xml}) by importing event class {\sf announceScholarship}. An employee can apply for a job or scholarship by locally invoking {\sf apply(xs:ID, j:Application)} through some user interface. An according event is stored in event class {\sf apply} which is imported by {\sf vienna.xml}.

After the application deadline for a scholarship is over, rule {\sf selectApplicantsRule} is executed to select the people to which the scholarship is granted. If the number of applicants is larger than the number of scholarships, a ranking is established based on 
a) the applications, and 
b) the order of their application if two applicants have the same qualification.

If all three locations provide time service level {\sf tsl-3}, a temporal order between applications can be established, otherwise a causal order will be used.
\end{example}

% ############################################################

\input{axs/managing}



==> composite-events/adaption.tex <==
\section{Refined Event Algebra}
\label{section:adaption}

This section shows how the event algebra Snoop is refined so that it can be used with XML events. First it presents the employed abstract model for XML data, a syntax for referrers to portions of XML data at the schema and instance level, and operators on referrers in Subsection~\ref{section:pi-and-pts}. Second, an abstract model for events and event types is introduced in Subsection~\ref{section:evts-and-evtps}. Finally, Subsection~\ref{section:motivating-example} briefly introduces Snoop and shows an example that uses the refined event algebra with contexts from Snoop.

\subsection{Path Types and Path Instances}
\label{section:pi-and-pts}

An XML document is represented by a tree of nodes where an XML document's elements, attributes and text is represented by the tree using element, attribute, and text nodes respectively. As such it is a subset of the XML Infoset \cite{W3C2001XMLInfoset}. Each node has an identifier.

A \textit{path type} identifies a node of a tree by using type information, i.e., independently of concrete documents. A path type accords to a restricted XPath expression \cite{W3C1999XPath} that refers to either element, attribute, or text nodes in each of its steps via respective axis and node tests. A path type is absolute or relative with respect to the root of the tree, e.g., ${\sf /order/item/price}$ denotes an absolute path type while ${\sf item/price}$ denotes a relative path type to element ${\sf price}$. Path type $pt$ is a tuple  comprising a $kind \in \{{\sf absolute}, {\sf relative}\}$ and an ordered set of steps, thus $pt=\langle kind, steps\rangle$ or $pt=null$.
Two single steps are equal if they equal in their respective axis (${\sf child}$ or ${\sf  attribute}$) and node test (test for an XML-QName or ${\sf text()}$).
%no wildcards yet -> complicated to define operators and their results

A \textit{path instance} identifies a node of a tree representing a concrete document. For node ${\sf price_1}$ its path instance comprises an ordered set of identifiers that starts with the identifier of the tree's root node and ends with ${\sf price_1}$'s identifier and is thus always absolute. A path instance is denoted similar to a path type by using ``/'' to separate nodes, e.g., ${\sf /order_1/item_1/price_1}$ denotes a path instance to node ${\sf price_1}$. Path instance $pi$ is a tuple comprising its absolute path type and an ordered set of node identifiers, thus $pi=\langle pt, ids \rangle$ or $pi=null$.

To compare and operate on path types, operators for testing for equality ($=$), containment ($\subset$), ending ($\subset_{\sf e}$), and intersection ($\cap_{\sf lb}$, $\cap_{\sf ab}$) are defined. The operators complement the ones defined by XPath which operate on path instances only, such as ${\sf =}$ \cite{W3C1999XPath} and ${\sf intersection}$ \cite{W3C2003XPathFunc}.
The result of applying operators on path types are defined as follows (where $m=|pt_1.steps|$ and $n=|pt_2.steps|$):

\begin{itemize}
\item $pt_1 = pt_2$ \\
Path type $pt_1$ equals $pt_2$ iff $pt_1.kind=pt_2.kind \wedge m=n \wedge \forall 1\leq i \leq m: pt_1.steps[i]=pt_2.steps[i]$.

\begin{example}
\parbox[t]{\textwidth/2}{
${\sf item/price} = {\sf item/price}$, \\
${\sf /order} = {\sf /order}$, \\
${\sf order} \neq {\sf /order}$.
}
\end{example}

\item $pt_1 \subset pt_2$ \\
Path type $pt_2$ uniquely contains path type $pt_1$ iff 
%[false] there exists a $j$ and $k$ (where $j<k \leq |pt_1.steps|$) such that  $\forall j \leq i \leq k: pt_1.steps[i]=pt_2.steps[i+c]$ where $c$ is a constant offset in $pt_2$'s steps and $k+c \leq |pt_2.steps|$. No $j' \neq j$ and $k' \neq k$ may exist for which the expression above applies as well.
$\forall 1 \leq i \leq m: pt_1.steps[i]=pt_2.steps[c+i]$ where $c$ is a constant offset and $m+c \leq n$.
No $c' \neq c$ may exist for which the expression above applies as well.
Additionally, if $pt_1$ and $pt_2$ are both absolute $c=0 \wedge m < n$ must apply, if both are relative only $m < n$ must apply.
%[false] Moreover, if $pt_1$ and $pt_2$ are both absolute $|pt_2.steps|>|pt_1.steps| \wedge j=1$ must apply, if both are relative only $|pt_2.steps|>|pt_1.steps|$ must apply.
A relative path type cannot contain an absolute one.

\begin{example}
\parbox[t]{\textwidth/2}{
    ${\sf item/price} \subset {\sf /order/item/price}$,  \\
    ${\sf order/\-item}$ $\subset$ ${\sf /order/\-item/price}$, \\
    ${\sf /order} \not\subset {\sf order/item}$.
}
\end{example}

\item $pt_1 \subset_{\sf e} pt_2$ \\
Relative path type $pt_1$ ends path type $pt_2$ if the end of $pt_2.steps$ contains $pt_1.steps$ and $pt_2$ is more special than $pt_1$, i.e., $pt_1 \subset_{\sf e} pt_2$ iff $pt_1.kind={\sf relative} \wedge (m<n \vee (pt_2.kind={\sf absolute} \wedge m=n)) \wedge \forall 1 \leq i \leq m: pt_1.steps[i]=pt_2.steps[n-m+i]$.

\begin{example}
\parbox[t]{\textwidth/2}{
    ${\sf item/price \subset_e /order/item/price}$, \\
    ${\sf price \subset_e item/price}$, \\
    ${\sf order/item \not\subset_e /order/item/price}$.
}
\end{example}

\item $r:=pt_1 \cap_{\sf lb} pt_2$ \\
The left-bound intersection operator is commutative and determines for path types $pt_1$ and $pt_2$ equal steps at the beginning of $pt_1.steps$ and $pt_2.steps$.
If $pt_1.kind = pt_2.kind$, $r.kind:=pt_1.kind$, otherwise it is ${\sf absolute}$. Resulting $r.steps:=\{pt_1.steps[i] | pt_1.steps[i]=pt_2.steps[i]\}$ where $1 \leq i \leq j$ where $j$ is either the largest index for which $pt_1.steps[j] = pt_2.steps[j]$ applies 
%[false] smallest index for which $pt_1.steps[j] \neq pt_2.steps[j]$ applies 
or the minimum out of $m$ and $n$.
The result is $null$ if $pt_1=null \vee pt_2=null \vee pt_1.steps[1] \neq pt_2.steps[1]$.

\begin{example}
\parbox[t]{\textwidth/2}{
    ${\sf order/item \cap_{\sf lb} /order/billTo = /order}$, \\
    ${\sf item/@partnum \cap_{\sf lb} item = item}$, \\
    ${\sf order \cap_{\sf lb} item} = null$.
}
\end{example}

\item $r:=pt_1 \cap_{\sf ab} pt_2$ \\
The absolute-path intersection is not commutative and makes path type $pt_1$ absolute according to absolute path type $pt_2$. If $pt_1 \subset pt_2 \vee pt_1=pt_2$, $r$ is defined by $r.kind:={\sf absolute}$ and $r.steps:=\{pt_2.steps[i]|1 \leq i \leq j\}$ where $j$ is the last index where $pt_2$ contains $pt_1$. 
The result is $null$ if $pt_1=null \vee pt_2=null \vee (pt_1 \not\subset pt_2 \wedge pt_1 \neq pt_2)$.

\begin{example}
\parbox[t]{\textwidth/2}{
    ${\sf item \cap_{ab} /order/item/price = /order/item}$, \\
    ${\sf item \cap_{ab} /order} = null$.
}
\end{example}

\end{itemize}

To compare and operate on path instances, operators for testing for equality ($=$) and projection ($\pi$) are defined. The result of applying operators on path instances are defined as follows:

\begin{itemize}
\item $pi_1=pi_2$ \\
Two path instances $pi_1$ and $pi_2$ equal iff $pi_1.pt=pi_2.pt \wedge \forall 1 \leq i \leq |pi_1.ids|: pi_1.ids[i]=pi_2.ids[i]$.

\begin{example}
${\sf /order_1/item_1 = /order_1/item_1}$.
%(ii) {\sf /order$_1$/item$_1$ $\neq$ /order$_1$/item$_2$}.
\end{example}

\item $r:=\pi_{pt}(pi)$ \\
A projection of path instance $pi$ on path type $pt$ is a path instance iff $pt \subset pi.pt \vee pt=pi.pt$. Then $r.pt:=pt$ and $r.ids := \{pi.ids[i]| j \leq i \leq k\}$ where $j$ and $k$ are the indexes between which $pi.pt.steps$ contains $pt.steps$. 
The result is $null$ if $pi=null \vee pt=null \vee (pt \not\subset pi.pt \wedge pt \neq pi.pt)$.

\begin{example}
\parbox[t]{\textwidth/2}{
    ${\sf \pi_{\sf item}(/order_1/item_1/price_1) = item_1}$, \\
    ${\sf \pi_{\sf /order}(/order_1/item_1) = /order_1}$, \\
    ${\sf \pi_{\sf item}(/order_1)} = null$.
}
\end{example}

\end{itemize}

\subsection{Event Types and Events}
\label{section:evts-and-evtps}

The DOM Event Module defines among others event types for mutation events, which reflect modifications of DOM documents' data. They basically comprise one event type for the insertion of nodes, one for the deletion of nodes, %(event types {\tt DOMNodeInserted} and {\tt DOMNodeRemoved}) 
one for manipulation of attributes, %({\tt DOMAttrModified}) 
and one for manipulations of text nodes. %({\tt DOMCharacterDataModified}).

While the DOM event types are sufficient for a procedural handling of occurred events, they are too coarse grained for a declarative handling by an event algebra.
Hence, for \textit{every} path type $pt$ the presented approach distinguishes three \textit{primitive event types}, denoted as ${\sf ins}(pt)$, ${\sf upd}(pt)$, and ${\sf del}(pt)$. Like in the DOM Event Module, ${\sf ins}$ and ${\sf del}$ events reflect insertions and deletions of element, attribute, and text nodes, while ${\sf upd}$  events reflect modifications of text nodes and attribute nodes. Moreover, instead of an operation wildcard ``$*$'' can be used. The path type defines where events of that type occur. It can be relative or absolute.
%Since all text nodes that are children of the same element node have the same path type, there may still exist text data in path type $p$ after a {\sf del($p$)} event occurs.
Primitive event type $et$ is a tuple comprising an operation, which is one of $\{{\sf ins}, {\sf upd}, {\sf del}, *\}$, and a path type, thus $et=\langle op, pt \rangle$.

A \textit{primitive event} occurs whenever a node is manipulated. Primitive event $e$ is represented by a tuple comprising its identifier $id$, timestamp $ts$, event type $et$, and path instance $pi$ which identifies the manipulated node, thus $e=\langle id, ts, et, pi\rangle$. 
The event type's operation does not equal wildcard ``$*$'', its path type is absolute, and the path instance's path type $pi.pt$ equals $et.pt$.
%The event type is formed by the occurred operation ({\sf ins}, {\sf upd}, or {\sf del}) and the manipulated node's absolute path type. The path instance identifies the manipulated node (where $pi.pt=et.pt$).
%As shorthand notations $\rho(e)$ refers to the event's operation, $\tau(e)$ to its path type, and $\iota(e)$ to the path instance.
%The event type of $e$ comprises its operation $e.et.op$ (short $\rho(e)$) and its path type $e.evttp.pathtype$ (short $\tau(e)$). As a shorthand notation for $e.pathinst$ notion $\iota(e)$ is used. An event's path type and path instance must be absolute.

A \textit{composite event type}, i.e., the event type of a composite event, is a tuple that comprises a unique name and a path type, thus $et = \langle name, pt \rangle$. Wildcard ``$*$'' can be used instead of a name, referring to any composite event type having the path type. 
A composite event type is denoted as ${\sf name}(pt)$ analogously to a primitive one.
The path type of a composite event type defines, like the path type of a primitive event type, where events of that type occur. It can be relative or absolute.

A \textit{composite event} is formed by combining primitive and other composite events, which are referred to as constituent events. Composite event $e^c$ is represented by a tuple comprising its identifier $id$, composite event type $et$, path instance $pi$, which identifies where the event occurred, and a set of constituent events $cevts$, thus $e^c=\langle id, et, pi, cevts \rangle$. The composite event type's name does not equal wildcard ``$*$'', its path type is absolute, and the path instance's path type $e^c.pi.pt$ equals $e^c.et.pt$.

The notion of ``event type'' as used in this Chapter subsumes the notions of ``event type'' and ``event class'' from Subsection~\ref{section:event-types-and-classes} as follows:

\begin{enumerate}
\item
A tuple representing a primitive event type denotes an instance of metaschema class {\sf evts::PrimitiveMutEvtTp}. The instance's attribute {\sf timeSpec}, which defines whether the event should be detected before or after the respective manipulation takes place, is not of relevance in the context of detecting composite events and is thus not dealt with in this chapter. The same applies for the instance's attribute {\sf name}, which is derived as the concatenation of operation {\sf op} and path type {\sf pathTp} (cf. Figure~\ref{fig:uml-metamodel-evts}).
%
\item
A tuple representing a composite event type denotes an instance of metaschema class {\sf cle::CompositeMutEvtTp}. The tuple's $name$ correspond to the instances {\sf name}, and $pt$ to {\sf pathTp}.
%
\item
An event expression denotes an instance of metaschema class {\sf cle::CompositeMutEvtCs}. Conceptually, the expression specifies a query over event classes with mutation events, thereby defining the extension of the composite event class. It thus corresponds to the instance's attribute {\sf querySpec}. 
When an event expression refers to another event expression via its assigned composite event type (see Subsection~\ref{section:hierarchical-context}), it uses the latter type to refer to the class's extension (thus using the notion ``type'' to refer to both intensional and extensional aspects). To assure that an event class with the composite event type's name exists, a constraint is specified with metaschema class {\sf cle::CompositeMutEvtCs} (see Figure~\ref{fig:uml-metamodel-loev}).
\end{enumerate}

The logical clock of time service level {\sf tsl-1} (see Subsection~\ref{section:timeSvcLevels}) is sufficient for detecting composite events.
%The clock for measuring the timestamps of primitive events is a logical one, i.e., a counter. 
Primitive events occur at distinct points in time and for simplicity it is assumed that the detection of composite events takes no time. Therefore one primitive and multiple composite events may be detected at a single point in time.

Primitive as well as composite event types are hierarchically related via their path type and lead to \textit{more expressive} composite event type definitions than in Snoop. Most important this allows to constrain the combination of event types by an operator to related event types. For the constraints on operator nodes see Subsection~\ref{section:hierarchical-context}.

An event can be an instance of more than one event type, providing for \textit{more reusable} composite event type definitions than in Snoop. 
Event $e$ is a direct instance of its type $e.et$ and an indirect instance of event types $et_i \neq e.et$ to which the event's type is compatible to, denoted by $e.et \succeq et_i$ (not commutative).
Primitive event type $et_1$ is \textit{compatible to} primitive event type $et_2$, i.e., $et_1 \succeq  et_2$ iff $((et_1.op = et_2.op) \vee (et_2.op=$``$*$''$)) \wedge ((et_2.pt \subset_{\sf e} et_1.pt) \vee (et_2.pt=et_1.pt))$. 
Analogously, for two composite event types 
$et^c_1 \succeq et^c_2$ iff $((et^c_1.name = et^c_2.name) \vee (et^c_2.name=$``$*$''$)) \wedge ((et^c_2.pt \subset_{\sf e} et^c_1.pt) \vee (et^c_2.pt=et^c_1.pt))$. For more details on reuse see Subsection~\ref{section:hierarchical-context}, especially Examples~\ref{example:reusable-event-trees-1} and \ref{example:reusable-event-trees-2}.

%[LEAVE] As one can see, multi-classification of primitive events is done by comparing operations and by partially matching path types. 
%[FALSE] For two composite event types $et^c_1 \geqslant et^c_2$ iff $(et^c_1.opr=et^c_2.opr) \wedge (et^c_2.pt \subseteq_e et^c_1.pt) \wedge (|et^c_1.cevttps|=|et^c_2.cevttps|) \wedge (\forall 1 \leq i \leq |et^c_1.cevttps|: et^c_1.cevttps[i] \geqslant et^c_2.cevttps[i])$.

\begin{example}
\label{exmp:type-compatibility}
Primitive event $e_{p_1}$ reflecting an insertion in path type $e_{p_1}.et.pt = {\sf /order/item/price}$ is an instance of event types such as 
$E_1 = {\sf ins(/order/item/price)}$ and 
%${\sf E_2 := ins(item/price)}$, and
%${\sf E_3 := *(/order/item/price)}$, and 
$E_2 = {\sf *(price)}$ since $e_{p_1}.et \succeq E_1$ and $e_{p_1}.et \succeq E_2$.
Analogously, composite event $e_{h_1}^c$ with path type $e_{h_1}^c.et.pt = {\sf /order/item}$ and name ${\sf Nm}$ %$e_{h_1}^c.et.name = {\sf Nm}$ 
is an instance of composite event types such as
$E_1^c = {\sf Nm(/order/item)}$ and 
$E_2^c = {\sf *(item)}$ since $e_{h_1}^c.et \succeq E_1^c$ and $e_{h_1}^c.et \succeq E_2^c$.
\end{example}

Like in Snoop, composite event types are defined by event expressions according to an event algebra. An expression combines events by the algebra's operators. The presented approach uses operators $\bigtriangleup$, $\bigtriangledown$, and {\tt ;} from Snoop to form conjunction, disjunction, and sequence of events. An expression is realized by an event tree, e.g., Figure~\ref{fig:evtgraph-pt-derivation} depicts the event tree that realizes the expression described in Subsection~\ref{section:motivating-example}.

An event tree comprises event type nodes and operator nodes.
An \textit{event type node} is a tuple $\langle et, evts \rangle$ which stores a set of events $evts$. All events in $evts$ are a direct or indirect instance of event type $et$. 
An \textit{operator node} combines events from child nodes $nds$ to events of composite event type $et$ according to operator $opr$ and stores them in a set of composite events $evts$, and is thus a tuple $\langle opr, nds, et, evts \rangle$. Leaf nodes in an event tree are event type nodes while inner nodes are operator nodes. 

In the presented approach the event type of an event tree node (i.e., of an event type node or operator node) can be compared to the \textit{static type} of a variable in strongly typed object-oriented programming languages (e.g., Java), while the event type of an event can be compared to the \textit{dynamic type} of an expression,  e.g., an object. 
An occurred event is stored in all leaf nodes that have a compatible event type. By using the ending operator in the definition of type compatibility a leaf node only stores events that occur directly in the node's path type and not in descendants.

\begin{example}
Continuing Example~\ref{exmp:type-compatibility}, when primitive event $e_{p_1}$ with (dynamic) event type $e_{p_1}.et$ occurs, it is stored in event type nodes that have compatible (static) event types such as $E_1$ and $E_2$. 
Analogously, when composite event $e_{h_1}^c$ is raised, it is stored in event type nodes that have event types such as $E_1^c$ and $E_2^c$.
\end{example}

%he path type of $e^c$'s event type can be compared to a static type and the path type of $e^c$'s path instance to a dynamic type in strongly typed object-oriented programming languages. A static type is compatible to a dynamic type if $e^c.et.pt \subseteq e^c.pi.pt$, i.e., if it is the same or more general.
% Again, comparing event types with types in object-oriented programming languages, $e.et$ can be compared to a dynamic type and $et$ to a static type, e.g., of an event type node (cf. later in this section).

\subsection{Motivating Example}
\label{section:motivating-example}

\input{composite-events/example_chak-ct}

This section exemplifies the need for composite events in XML and demonstrates the application of the refined event algebra.
Consider an XML document that represents a purchase order (document element ${\sf order}$) comprising items to be ordered (element ${\sf item}$), each in turn described by a price (element ${\sf price}$) and a quantity (element ${\sf quantity}$). 
When defining a rule that reacts on the insertion of an item and re-calculates the overall order value by multiplying price by quantity of each item and summing it up, one encounters the problem to decide which primitive mutation event to react upon. Upon the insertion of element ${\sf item}$ it does not comprise any of the necessary child elements, and upon the insertion of element ${\sf price}$ the ${\sf quantity}$ element may not be available and vice versa.

The problem can be overcome by using composite events. A composite event is raised according to its definition after certain primitive events have occurred. In the example, a composite event should occur after the occurrence of events reflecting insertions of an ${\sf item}$, a ${\sf price}$, and a ${\sf quantity}$ element (where the latter two are children of the first) so that a rule can be defined on it.
This can be achieved by event expression ``${\sf E_i}$ {\tt ;} $({\sf E_p} \bigtriangleup {\sf E_q})$'', where 
${\sf E_i:= ins(item)}$, 
${\sf E_p:= ins(item/price)}$, and 
${\sf E_q:= ins(item/quantity)}$.
%,defines composite events to be raised after an event of event type $E_i$ occurs followed by an event occurrences of both $E_p$ {\em and} $E_q$.

\begin{figure}[h]
    \begin{center}
        \includegraphics[scale=1.1]{./composite-events/example.eps}
        \caption{Recalculate Order Value upon Insertion of an Item}
        \label{fig:AXSExampleForCevts}
    \end{center}
\end{figure}

Figure~\ref{fig:AXSExampleForCevts} shows the example's active XML schema. It defines composite event class {\sf InsertItem} whose query is set to the  mentioned event expression. Thereby detected composite events are stored in the event class upon their occurrence. Upon occurrence of a such a composite event, rule {\sf recalculateOrderValueRule} is executed, recalculating the overall order value by invoking operation {\sf calculateTotal()}.

The event tree realizing the example's event expression is depicted in Figure~\ref{fig:evtgraph-pt-derivation}. 
The event tree's behavior when using contexts from Snoop, i.e., its processing of four sequences of primitive events $S_1..S_4$ is shown in Table~\ref{tab:adapted-evt-graphs}.
The sequences reflect the insertions of ${\sf item}$ (abbreviated as $i_n$), ${\sf price}$ ($p_n$), and ${\sf quantity}$ ($q_n$) elements.
Numerical index $n$ of an element represents its hierarchical position, meaning that elements with the same numerical index are hierarchically related, e.g., $p_1$ is a child of $i_1$. In case two numerical indices are separated by a dot, the first number represents the element's hierarchical position and the second one the time of its insertion, e.g., the insertion of $q_{1.1}$ occurs before the insertion of $q_{1.2}$.

Briefly and informally introducing the contexts from Snoop, a composite event is raised by a conjunction operator node as soon as a child node's set of stored events is modified, i.e., an event is added (the so called ``terminator'') and every child node contains at least one event. 
Note that only the conjunction operator is described here, however, sequence and disjoint operator are defined analogously.
%[leave] (in the correct order) for the conjunction and sequence operator or at least one child node contains an event for the disjunction operator. The composite event is defined as follows for the conjunction and sequence operator, for the disjunction operator it is defined analogously:
A raised composite event's constituent events are defined as follows:

\begin{itemize}
\item in \textit{cumulative context} they comprise all events from every child node wherefrom they are removed.
%
\item in \textit{chronicle context} they comprise the oldest event from every child node wherefrom they are removed, i.e., all constituent events are consumed in chronological order of occurrence.
%
\item in \textit{recent context} they comprise the most recent event from each child node. All events that cannot be the earliest constituent event of subsequently raised composite events (i.e., that cannot be an ``initiator'') are removed from child nodes.

\item in \textit{continuous context} its constituent events comprise the terminator and the most recent event from every child node except the one of the terminator. Subsequently all constituent events are removed from child nodes except the terminator. The procedure is repeated until there are no events left to be combined with the terminator. Finally the terminator is removed if it cannot be an initiator of subsequently raised composite events. %[unnecessary] Note that this context is the only one that possibly raises multiple composite events upon a single event occurrence.
\end{itemize}

The rationale of Table~\ref{tab:adapted-evt-graphs} is 
to introduce the unfamiliar reader to Snoop's contexts and 
to exemplify that incorrect composite events are raised when any of Snoop's contexts is used (for which one falsifying event sequence would suffice).
Incorrect events are raised because events are selected only by their occurrence time and not their hierarchical position. Where under a correct composite event it is referred to a composite event whose constituent events are hierarchically related.
Composite events raised by the root of the tree are shown by their constituent events, e.g., $\{e_{i_1}e_{p_1}e_{q_1}\}^c$.
Unconsumed composite events that remain in the tree after $t_6$ are shown at the time they are raised, but in brackets, e.g., $(\{e_{p_2}e_{q_2}\}^c)$.
The table does not show the unrestricted context which basically forms the cartesian product of all events. Naturally, it raises even more incorrect composite events.

Summarized, the refined event algebra as presented in this section is still not applicable to detect composite events in XML when used with contexts from Snoop. The reason is that the requirements on applications using such an event algebra are inadequate, which would have to use the unrestricted context and filter out huge amounts of incorrect events or manipulate XML data in a defined temporal order so that some context only detects correct events. Still, the satisfaction of multiplicity constraints cannot be detected using the refined algebra.


==> composite-events/extension.tex <==
\section{Extended Event Algebra}
\label{section:extension}

This section presents an extension to the refined event algebra. The extension comprises the hierarchical context presented in Subsection~\ref{section:hierarchical-context}, the multiplicity operator in Subsection~\ref{section:multiplicity-operator}, and operator modifiers in Subsection~\ref{section:operator-modifiers}.
%
Event trees which are generated from event expressions are used for presentational purposes throughout the section.

%@@Due to the mapping of event expressions to event trees, two trees that seem to represent logically equal expressions may be semantically unequal. For example, $E_a \bigtriangleup E_b \bigtriangleup E_c \neq (E_a \bigtriangleup E_b) \bigtriangleup E_c$, because tree of the former has a single operator node opposite to the latter which has two operator nodes. Both event trees differ in their semantics because the operator nodes may differ in their path types and thus may combine different events. Nevertheless, $E_a \bigtriangleup E_b \bigtriangleup E_c = E_a \bigtriangleup E_c \bigtriangleup E_b$. The right of Figure~\ref{fig:evtgraph.mult-op} shows another example where a node's path type is denoted beside it.

% ############################################################
% #
% # CONTEXT
% #
% ############################################################

\subsection{Hierarchical Context}
\label{section:hierarchical-context}

The hierarchical context is introduced since it is necessary to combine events according to their hierarchical position, which is not supported by existing contexts. It raises only correct composite events, i.e., composite events whose constituent events are hierarchically related.
%[leave] Table~\ref{tab:hierarchical-context} (cf. Appendix) shows raised composite events according to the hierarchical context for the example presented in Section~\ref{section:motivating-example}.

To combine events according to their hierarchical position an event tree maintains data concerning hierarchy. Therefore, as mentioned earlier, every node $n$ in an event tree has an assigned path type $n.et.pt$.
Naturally, an event type node specifies a path type, however, the path type of an operator node, if not specified by the event expression, has to be derived from its child nodes $c_1, c_2, ... ,c_n$ by evaluating $c_1.et.pt \cap_{\sf lb} c_2.et.pt \cap_{\sf lb} ... \cap_{\sf lb} c_n.et.pt$ (left-bound intersection is used for simplicity). 
%[FALSE it is not reasonable to use a conj., discj., or sequ. with only one child, nor is it more reasonable to set it to the parent] If $n=1$, i.e., if $o$ has only one child node the default path type is the child node's path type without the last step (so that it identifies the parent node).
The derivation of path types for all operator nodes is done bottom up. For an event tree to be valid, every node $n$ must have a non-$null$ path type whose steps are not empty and do not violate the constraints on child nodes (cf. later in this section).

\begin{example}
\label{example:derivation-of-path-types}
Figure~\ref{fig:evtgraph-pt-derivation} shows an exemplary event tree on the left defining composite event type ${\sf E^c_i} := {\sf E_i}$ {\tt ;} $({\sf E_p} \bigtriangleup {\sf E_q})$ for the insertion of ${\sf item}$ elements and the derivation of path types for operator nodes on the right. The derivation is done bottom up, step 1 determines the path type of operator node $\bigtriangleup$ by evaluating ${\sf item/price} \cap_{\sf lb} {\sf item/quantity} = {\sf item}$. Subsequently, step 2 determines the path type of operator node {\tt ;} by evaluating ${\sf item} \cap_{\sf lb} {\sf item} = {\sf item}$.
\end{example}

\begin{figure}[h]
    \begin{center}
        \includegraphics[scale=1.2]{composite-events/evtgraph2_small}
        \caption{Derivation of Operator Nodes' Path Types}
        \label{fig:evtgraph-pt-derivation}
    \end{center}
\end{figure}

%When a primitive or composite event occurs it is stored in all event type nodes it is an instance of. Remember that a primitive event can be an instance of multiple event types. Each event type node and each operator node can store multiple events.

An operator node raises a composite event by selecting events from its child nodes that satisfy certain conditions. Basically, (a) at least one child node of a disjunction operator node must hold an event, (b) all child nodes of a conjunction operator node must hold an event, and (c) all child nodes of a sequence operator node must hold an event and they must have occurred in the specified order.
%[FALSE] Composite event $e^c$'s path type is set to the combining operator's path type, i.e., $e^c.pt:=o.et.pt$.

If operator node $o$ combines multiple events from child nodes they must all have the same ancestor node, i.e., $\forall 1 \leq i \leq m-1: \pi_{o.et.pt}(e_i.pi) = \pi_{o.et.pt}(e_{i+1}.pi)$ where $m$ is the number of events in $o$'s child nodes that are to be combined. Events for which the projection evaluates to $null$ are not combined. Raised composite event $e^c$'s path instance, which must be absolute, is derived from constituent events by $\pi_{o.et.pt \cap_{\sf ab} e_1.pi.pt}(e_1.pi)$. Event $e_1$ is the first constituent event, however, any other constituent event $e_i$ could be used instead because if all constituent events $e_i$ equal in $\pi_{o.et.pt}(e_i.pi)$ they equal in $\pi_{o.et.pt \cap_{\sf ab} e_i.pi.pt}(e_i.pi)$ as well. 
%The event's path type $e^c.et.pt$ is set to absolute path type $e^c.pi.pt$.

\begin{example}
How the event tree in Figure~\ref{fig:evtgraph-pt-derivation} forms composite events in hierarchical context is shown in Figure~\ref{fig:evtgraph1}.
Its status after the occurrence of the event sequence $e_{i_1}, e_{i_2}, e_{p_1}, e_{p_2}, e_{q_1}$ is shown on the left. In path instances and event indices, $o$ abbreviates ${\sf order}$, $i$ abbreviates ${\sf item}$, $p$ abbreviates ${\sf price}$, $q$ abbreviates ${\sf quantity}$, and the numerical index indicates the hierarchical position, e.g., $p_1$ is a child of $i_1$.
Events $e_{p_1}$ and $e_{q_1}$ are combined by operator $\bigtriangleup$ to form composite event $e^c_{h_1}$, since $\pi_{\sf item}(e_{p_1}.pi)=\pi_{\sf item}(e_{q_1}.pi)$ ($={\sf i}_1$). With the creation of $e^c_{h_1}$ the two primitive events are consumed (step 1). Subsequently, $e_{i_1}$ and $e^c_{h_1}$ are combined by operator {\tt ;} since $\pi_{\sf item}(e_{i_1}.pi)=\pi_{\sf item}(e^c_{h_1}.pi)$ ($={\sf i}_1$) (step 2). 
Upon the occurrence of $e_{q_2}$ later on the same combination process starts over again.
\end{example}

\begin{figure}[h]
    \begin{center}
        \includegraphics[scale=1.3]{composite-events/evtgraph1b_small}
        \caption{Event Selection and Event Consumption in Hierarchical Context}
        \label{fig:evtgraph1}
    \end{center}
\end{figure}

\textit{Constraints} on operator node $o$'s path type are enforced so that the projection of an event's path instance on $o$'s path type is likely to return a non-$null$ value, i.e., so that for child event $e_j$ expression $\pi_{o.et.pt}(e_{j}.pi) \neq null$ applies. The constraints seek a compromise between the operator's expressiveness for the reuse of event trees (see later in this section) and restrictions on child nodes and do thus not guarantee a non-$null$ value. They are as follows (where $E_j$ refers to a child node's event type): 
(a) if both $o.et.pt$ and $E_j.pt$ are absolute, $o.et.pt \cap_{\sf lb} E_j.pt
\neq null$ must apply, 
(b) if only $E_j.pt$ is absolute, $o.et.pt \subset E_j.pt$ must apply. 
If $E_j.pt$ is relative no constraints must apply so that it may contain only a single step that is not contained in $o.et.pt$.
In such cases one must rely that an event's (dynamic) event type is compatible to the operator's (static) event type so that the event's path instance can be projected on the operator's path type. 
This can be compared to a type-cast in strongly typed object-oriented programming languages where an object's dynamic type must be compatible to the static casted type which can only be determined at runtime. For examples see Example~\ref{example:reusable-event-trees-1} and \ref{example:reusable-event-trees-2}.
%[COMMENT] the most restrictive constraint would be $o.et.pt \subseteq E_j.pt$, irrespective of whether the path types are absolute or relative

Operators combine events with \textit{interval-based semantics} not detection-based semantics, since composite events detected with the latter are not always exactly as, presumably, intended (cf. \cite{Adai2002TR,Galt2002DEXA}).
Basically, this means that operators do not combine events according to their detection time but take the intervals during which the events occurred into account.
A primitive event detected at $t_d$ occurs in interval $[t_d,t_d]$, and a composite event starts at the beginning of the smallest interval and ends at the end of the latest one. Comparing intervals, $[t_a',t_a''] < [t_b',t_b'']$ iff $t_a''<t_b'$.
Interval-based semantics only affect the sequence operator, so that expression $E_i${\tt ;}$E_j$ combines two hierarchically matching events $e_i$ and $e_j$ only if the occurrence interval of the former is smaller than the other.

%Combination of composite events follows a distinction between event selection and event consumption as encouraged by \cite{Zimm99DE}. While event selection of events in child nodes is based on hierarchical XML structure as described above, event consumption is like in cumulative context, meaning that once events are selected, they are consumed.

The hierarchical context is \textit{orthogonal} to existing contexts from Snoop, because selection by XML hierarchy is orthogonal to selection by time. Thus it can be combined with any existing context, acting like a filter. For operator node $o$, first the hierarchical context groups all events from child nodes according to $o$'s path type, and second $o$ selects and consumes events within each group according to its context from Snoop. 
%An example showing combinations of the hierarchical context with contexts from Snoop is presented in Table~\ref{tab:hierarchical-snoop-contexts} (cf. Appendix).

%As noted in Section~\ref{section:hierarchical-context} each of the contexts of Snoop can be combined with the hierarchical context, since selection by hierarchy and time are orthogonal. Example~\ref{example:hierarchical-snoop-ct} shows how every combination of the hierarchical context with contexts from Snoop raises composite events.

\input{composite-events/example_hier-chak-ct}

\begin{example}
\label{example:hierarchical-snoop-ct}
To detect when both price and quantity information of an order item are modified, event expression $*({\sf item/quantity})$ $\bigtriangleup$ ${\sf upd(item/price})$ can be used. Table~\ref{tab:hierarchical-snoop-contexts} shows raised composite events, represented by their constituent events for the above expression in the hierarchical variants of Snoop's contexts. Events that remain in the event graph after $t_5$ are shown in the rightmost column for completeness.
\end{example}

A composite event type definition can \textit{reuse} other, existing event type definitions, i.e., and event tree can reuse other event trees. All event trees together form the \textit{event graph}.
% ERROR: A tree that defines composite event type $E^c_i$ is reused in another tree through an event type node with event type $E^c_j$ iff $E^c_i \succeq E^c_j$. 
A composite event $e^c_i$ of type $E^c_i$ raised by an event tree is reused in another tree by an event type node with a compatible event type, i.e., if $e^c_i.et \succeq E^c_j$, presuming that $E^c_i.name=E^c_j.name$.
%
It may be the case that the node's parent operator node $o$'s path type $o.et.pt$ cannot be derived from its child nodes, because the left-bound intersection of $E^c_j.pt$ with the path types of $o$'s other child nodes is $null$, e.g., if their path types are of different kind or $E^c_j.pt$ contains only a single step. In either case $o$'s path type must be specified explicitly.

\begin{example}
\label{example:reusable-event-trees-1}
The ${\sf order}$ element has aside from ${\sf item}$ elements a ${\sf billTo}$ and a ${\sf shipTo}$ child element. When two composite event types ${\sf E^c_b}$ and ${\sf E^c_s}$ for complete insertions of the latter two elements are defined in addition to ${\sf E^c_i}$ (from Example~\ref{example:derivation-of-path-types}), a fourth composite event type can use the three to define a composite event that occurs after both addresses and at least one item have been inserted by ${\sf E^c_i} \bigtriangleup {\sf E^c_s} \bigtriangleup {\sf E^c_b}$. Since, e.g., ${\sf E^c_i}.pt \cap_{\sf lb} {\sf E^c_s}.pt \cap_{\sf lb} {\sf E^c_b}.pt = {\sf item} \cap_{\sf lb} {\sf shipTo} \cap_{\sf lb} {\sf billTo} = null$, the conjunction operator's path type must be specified explicitly, e.g., as ${\sf order}$. Because the (dynamic) event types of occurred events have absolute path types, the projection of their path instances on ${\sf order}$ is not $null$.
\end{example}

Reuse of event type definitions is facilitated by using type compatibility instead of type equality for storing occurred events in event type nodes, as mentioned before and in Subsection~\ref{section:evts-and-evtps}. 
The reason is that the more leaf nodes with ``general'' event types an event tree has (i.e., nodes with event types that have relative path types and/or wildcard ``$*$'' as operator or name), the more events will be stored in it because an event's ``special'' event type (i.e., one with absolute path type and given operation) may be compatible to a general one but not to another special one. The more events are stored, the more composite events are raised, and the more the tree, i.e., the event definition is reusable.

%Because every node in an event tree stores events whose event type is compatible with the node's event type, a single event may be stored in multiple nodes, especially if the node has an event type with a relative path type and/or with wildcard ``*'' as operator. An event tree that uses relative path types will raise composite events for primitive events that occur in different absolute path types. It can thus be reused by possibly multiple event trees.

\begin{figure}[h]
    \begin{center}
        \includegraphics[scale=1.3]{composite-events/evtgraph4}
        \caption{Reuse of Event Trees}
        \label{fig:evtgraph.reuse}
    \end{center}
\end{figure}

\begin{example}
\label{example:reusable-event-trees-2}
The order's ${\sf shipTo}$ and ${\sf billTo}$ elements both have an ${\sf address}$ child element that comprises other elements such as ${\sf street}$ and ${\sf city}$. By defining composite event type ${\sf E^c_a}$ for the insertions of ${\sf address}$ elements and using only relative path types that start with ${\sf address}$, the according event tree in Figure~\ref{fig:evtgraph.reuse} raises composite events for complete insertions of ${\sf address}$ elements as childs of both ${\sf shipTo}$ and ${\sf billTo}$. Thus ${\sf E^c_a}$ can be reused by both ${\sf E^c_b}$ and ${\sf E^c_s}$ from Example~\ref{example:reusable-event-trees-1}.
\end{example}

% ############################################################
% #
% # MULTIPLICITY
% #
% ############################################################

\input{composite-events/multiplicity}

% ############################################################
% #
% # MODIFIERS
% #
% ############################################################

\subsection{Operator Modifiers}
\label{section:operator-modifiers}

To enrich the expressiveness of event type definitions, operator nodes are parameterized by two modifiers to exactly define the points in time when composite events are raised. When an operator node detects events in child nodes that satisfy the operator's semantics, a ``potential composite event'', which is not stored in the tree, is detected. A composite event, which is stored in the tree, is raised with the detection of the potential event or is deferred to a later date. This is of importance, e.g., when a multiplicity operator or the hierarchical cumulative context is used, because the later a composite event is raised the more constituent events it will possibly have. Thus applications can react to deferred composite events comprising a rich set of constituent events and can determine the net-effect \cite{Pato99aACM}, i.e., overall effect of multiple events more easily.

First, the operator's \textit{termination mode} determines when a composite event is raised relative to the detection of a potential event.
If the termination mode is ${\sf earliest}$, composite event $e^c_i$ is raised with the detection of potential composite event $e^c_p$.
If it is ${\sf non}$-${\sf local}$, $e^c_i$ is raised after the detection of $e^c_p$ and the first occurrence of event $e_j$, where $\pi_{o.et.pt}(e^c_p.pi) \neq \pi_{o.et.pt}(e_j.pi)$. This means that operator node $o$ waits until an event occurs that reflects a manipulation in another subtree of the document, i.e., it assumes that the manipulation of a document is done hierarchically.
If the termination mode is ${\sf custom}$, composite events are raised upon flushing or closing the event tree (cf. later in this section).

\input{composite-events/example_tmodes}

\begin{example}
For the event tree depicted in Figure~\ref{fig:evtgraph.mult-op} and four exemplary event sequences $S_6..S_9$ Table~\ref{tab:termination-modes} shows when composite events are raised depending on the termination mode of (i) the conjunction operator node and (ii) the multiplicity operator node of the ${\sf quantity}$ element. The other two operator nodes have termination mode ${\sf earliest}$.
To clearly point out the consequences of termination modes the table shows composite events raised by any operator node. A composite event is denoted by $e^c$ with an alphabetical index indicating its event type and a numerical index indicating its hierarchical position. 
Note that due to the order of occurred events in $S_6..S_9$ the same composite events are raised irrespective of the context from Snoop that is combined with the hierarchical context.
\end{example}

Second, the operator's \textit{termination condition} must be fulfilled for a composite event to be raised.
It is a condition on the subtree of the XML document with root node $e^c_p.pi$ in the form of an arbitrary XPath expression which is evaluated relative to the subtree's root.\footnote{The restriction of querying the subtree only can be waived easily so that the condition is an arbitrary XPath expression which is evaluated relative to node $e^c_p.pi$. This, however, negatively affects performance because it is necessary to evaluate the termination condition in {\tt processTree($t$,$E$)} with every modification to the document, not only with every modification to the subtree.}
%It is a condition on the XML document in the form of an arbitrary XPath expression which is evaluated relative to the node represented by $e^c_p.pi$.
%\footnote{This differs from \cite{} where a termination condition was proposed to be evaluated against the subtree of the XML document with root node $e^c_p.pi$ only.}
%
The XPath expression must evaluate to boolean.
The termination condition differs from operators and termination modes in that it is used to test the instance document, not events. 
Termination conditions can be arbitrarily used.
E.g., they can ease the handling of events representing modifications of text nodes in case an element's text content may consist of multiple adjacent text nodes as in DOM (for which we have implemented a prototype, see Section~\ref{section:implementation}). In this case, termination conditions can be used, e.g., to test if an element's child text nodes contain any or certain text such as a number.
In certain situations, a termination condition can also be used to resemble the {\tt NOT} operator from Snoop by using an XPath expression with a negation and a node test.

\begin{example}
Instead of adding event type nodes and operator nodes that test for the insertion of text nodes to the event tree depicted in Figure~\ref{fig:evtgraph.mult-op}, termination condition ``${\sf item/price \geq 0 \wedge item/quantity > 0}$'' can be defined on the root node so that a composite event is only raised when both ${\sf price}$ and ${\sf quantity}$ element contain a value that is a number. This has also the advantage that text nodes can be arbitrarily inserted, updated, and deleted because its their value that matters, not the operations that lead to it.
\end{example}

The presented approach does not provide for termination conditions that test potential events themselves for two reasons.
%
First, this requires a defined binding of data to events that is more detailed than the one presented in Subsection~\ref{section:evts-and-evtps}, a defined representation of the binding and/or a defined syntax for expressing conditions. This is, however, outside the focus of this work. Second, related approaches for detecting composite events in the active database literature (e.g., cf. \cite{Chak94DKE,Gatz93RIDS,Geha92VLDB,Zhan96TR,Zimm99DE}) do not provide this capability too. There usually the environment in which composite event detection is employed provides this capability, i.e., the condition of an ECA rule may usually test the composite event in active databases \cite{Pato99aACM}.
The second reason also applies for termination conditions that test the document (provided by the approach), however, only partially because there are differences in semantics: While a termination condition that tests events and resembles a rule's condition is intended to avoid an action's execution by avoiding raising a composite event, a termination condition that test the document may be also intended to defer raising a composite event.

An event tree/graph can be opened, flushed, and closed by an application. 
After opening (or ``registering'' with a document) it stores occurring primitive and composite events. 
If it is flushed, remaining composite events are raised by operator nodes with ${\sf non}$-${\sf local}$ or ${\sf custom}$ termination mode. Closing an event tree/graph first flushes it and afterwards takes it out of order, e.g., when an XML document is closed after manipulation. An event tree/graph is automatically closed if the document is unloaded\footnote{cf. DOM event \url{ http://www.w3.org/2001/xml-events\#unload} \cite{W3C03DOM3EvtMod})}.



==> composite-events/implementation.tex <==
\section{Implementation}
\label{section:cevts.implementation}

The implemented proof-of-concept prototype extends the DOM event module of Apache's Xerces \cite{ApacheXerces} and thus provides Java applications with composite events. Detected composite events are dispatched to the DOM node identified by the event's path instance. This has the advantage that the API to react to composite events is the same as for DOM mutation events (comprising event listeners etc.). This section briefly describes the prototype's execution model.

Every occurred primitive event is inserted into the event graph, which is processed to detect composite events. 
To determine the order in which the event trees of the graph are processed, which remains the same as long as neither the graph nor the trees are modified, the notion of \textit{event tree dependency} is introduced. 
Event tree $t_b$ directly depends on event tree $t_a$, denoted as $t_a \rightarrow t_b$, iff $t_b$ uses composite event type $et_b$ to which event type $et_a$ defined by $t_a$ is compatible to, i.e., if $et_a \succeq et_b$. Naturally, direct dependency is not transitive. 
%Event trees may also depend on each other indirectly, i.e., via other event trees. 
%, e.g., $t_a \rightsarrow t_c$ if $t_a \rightarrow_d t_b$ and $t_b \rightarrow_d t_c$.
The transitive closure of a tree $t_a$ refers to the set of trees that directly and indirectly depend on it and is denoted by $(t_a)^+$.
An event tree may not be in its own closure, i.e., it may not depend directly or indirectly on itself.

Algorithm {\tt processGraph} for processing event graph $G$ upon the occurrence of primitive event $e$ is shown below. It processes every event tree of the graph exactly once. %Its complexity is $O(n^2)$.
Line {\tt 2} determines the ordered set of event trees that do not directly depend on any other event tree and assigns it to $T$. Subsequently, the set of occurred and raised events $E$ is initialized to $e$ (line {\tt  3}). While there are event trees left that need to be processed (line {\tt 4}), every event tree $t_i \in T$ is processed (line {\tt 5}--{\tt 6}, see later in this section), where $t_i$ denotes the $i^{th}$ element of $T$. Subsequently, all event trees that directly depend on any $t \in T$ and thus need to be processed are determined and assigned to $T$ (line {\tt 7}).
Finally, $T$ is purged (line {\tt 8}, see later in this section).

%can a pre-selection of an event tree be done so that not all have to be processed upon the occurrence of an event?

\begin{minipage}[h]{\textwidth}
\vspace{0.5cm}
\begin{tabbing}
\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \kill
{\tt 1}\>{\tt processGraph($e$}) \\
{\tt 2}\>\>$T := \{t \in G | \not\exists u \in G: u \rightarrow t\}$ \\
{\tt 3}\>\>$E := \{e\}$ \\
{\tt 4}\>\>\keyw{while} $T \neq \emptyset$ do \\
{\tt 5}\>\>\>\keyw{for} $i=1$ to $|T|$ do \\
{\tt 6}\>\>\>\>$E:=$ {\tt processTree($t_i$, $E$)} \\
{\tt 7}\>\>\>$T := \{t' \in G | \exists t \in T: t \rightarrow t'\}$ \\
{\tt 8}\>\>\>$T :=$ {\tt purge($T$)} \\
\end{tabbing}
\end{minipage}

Algorithm {\tt processTree($t$,$E$)} processes event tree $t$ with the set of events $E$ as follows. The tree is traversed in postorder (a form of depth-first traversal) during which 
(a) every visited event type node $n$ is tested for type compatibility with the event type of every event $e \in E$ and if they are compatible, i.e., $e.et \succeq n.et$, $e$ is stored in $n.evts$ (but not taken out of $E$), and 
(b) every visited operator node $o$ is evaluated if 
(i) an event was stored in a (direct) child node, 
(ii) if $o$ specifies a termination condition and for the primitive event 
$e \in E$ it applies that $o.et.pt \subset e.pt \vee o.et.pt = e.pt$,
%at least one event $e \in E$ has a path type which is ended by or equals the operator node's path type,
(iii) if $o$ has ${\sf non}$-${\sf local}$ termination mode, or 
(iv) if $o$ is a multiplicity operator node with $l=0$ and for the primitive event $e \in E$ it applies that $o.et.pt \subset_{\sf e} e.pt \vee o.et.pt=e.pt$.
%at least one event $e \in E$ has a path type which is ended by or equals the operator node's path type.
Finally, composite events that are raised in the root node of event tree $t$ are added to $E$ to be processed by dependent event trees later on.

Algorithm {\tt purge($T$)} 
%orders the set of event trees $T$ so that for every $t_i \in T$ holds that $t_i$ only depends directly on event trees $t_j \in T$ such that $j<i$ (it may depend arbitrarily on event trees not contained in $T$).
removes every event tree $t_k \in T$ from $T$ if it is contained in the transitive closure of another event tree $t_j \in T$. Executing {\tt purge($T$)} in {\tt processGraph} above guarantees that an event tree is processed exactly once at the latest time possible. 

%\begin{minipage}[h]{\textwidth}
%\vspace{0.5cm}
\begin{tabbing}
\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \kill
{\tt 1}\>{\tt purge($T$}) \\
{\tt 2}\>\>$T' := \{\}$ \\
{\tt 3}\>\>\keyw{for} $i=1$ to $|T|$ do \\
{\tt 4}\>\>\>\keyw{if} $\not\exists t_j \in T, j \neq i: t_i \in (t_j)^+$ \\
{\tt 5}\>\>\>\>$T' := T' \cup t_i$ \\
{\tt 6}\>\>\keyw{return} $T'$ \\
\end{tabbing}
%\end{minipage} 

The prototype including additional examples is available on the Web\footnote{at  \url{http://www.big.tuwien.ac.at/research/prototypes/composite-events/}}. Naturally the approach for composite mutation events is independent of an implementation and can be used by any application in need of composite events in XML, presumably, such as \cite{Bail02WWW} and \cite{Boni01aWWW}. 

==> composite-events/index.tex <==
The chapter discusses the functionality of the Active XML Schema (AXS) approach to compose occurred primitive mutation events to more complex ones, as already mentioned in Subsections~\ref{section:event-types-and-classes} and \ref{section:LogicalEventClasses}.
After introducing and motivating the problem of composite events in XML in Section~\ref{section:cevts.Introduction}, 
the refinement of an event algebra and a motivating example is shown in Section~\ref{section:adaption}. The event algebra that is refined is one from active database literature, where event algebras have been commonly used to define the composition of primitive events.
The main contribution of this chapter is made in Section~\ref{section:extension}, where the algebra's extension is presented.
Finally, Section~\ref{section:cevts.implementation} briefly discusses the implementation of a proof-of-concept prototype.

Note that this chapter, opposite to Chapter~\ref{chapter:ActiveXMLSchema}, uses the notion of ``type'' to refer to both intensional and extensional aspects of events, because this is how the active database literature dealing with composite events uses it (e.g., cf. \cite{Chak94DKE,Gatz93RIDS,Geha92VLDB,Zhan96TR,Zimm99DE}).
The reason may be that a clear distinction between intensional and extensional aspects is not required to describe the semantics of composite events. Moreover, it is expected that this loss in precision results in a presentation that is more concise and better readable.
How the notion of ``event type'' as used in this chapter subsumes the notions of ``event type'' and ``event class'' from Chapter~\ref{chapter:ActiveXMLSchema} is clarified in Subsection~\ref{section:evts-and-evtps}.

\input{composite-events/introduction}

%[abstract] Recently, active behavior has received attention in the XML field to automatically react to occurred events. Aside from proprietary approaches for enriching XML with active behavior, the W3C standardized the Document Object Model (DOM) Event Module for the detection of events in XML documents. When using any of these approaches, however, it is often impossible to decide which event to react upon because not a single event but a combination of multiple events, i.e., a composite event determines a situation to react upon. The paper presents the first approach for detecting composite events in XML documents by addressing the peculiarities of XML events which are caused by their hierarchical order in addition to their temporal order. It also provides for the detection of satisfied multiplicity constraints defined by XML schemas. Thereby the approach enables applications operating on XML documents to react to composite events which have richer semantics.

%@@\underline{not} distributed composite events!

% ############################################################

\input{composite-events/adaption}

% ############################################################

\input{composite-events/extension}

% ############################################################

\input{composite-events/implementation}







==> composite-events/introduction.tex <==
\section{Introduction}
\label{section:cevts.Introduction}

Recently, several approaches for active XML, i.e., for enriching XML documents with active behavior have been proposed, comprising Active XML Schema (AXS, see Chapter~\ref{chapter:ActiveXMLSchema}) and the ones described in Subsection~\ref{section:IR.xmlview-xml}. All provide for the definition of ECA rules on primitive mutation events, which occur upon, e.g., element insertions and attribute modifications.

In parallel, the W3C standardized the Document Object Model (DOM) Event Module \cite{W3C03DOM3EvtMod}. It provides for detection of events in DOM documents so that application programs can react accordingly. Defined events comprise among others mutation events, which are events that represent modifications of XML data. The Event Module may thus be used to provide the proprietary approaches for active XML and custom applications with mutation events.

When using any of the approaches for active XML, however, it is sometimes impossible to decide upon which event to react. The reason is that often not a single event but a combination of multiple events determines a situation where some action has to be executed.
A potential work-around in such a situation is to use the event that always occurs at last of multiple events or to use another event that usually occurs after multiple events.
Using such a work-around, however, makes rules dependent on applications which define the order of event occurrences.

Obviously, a technique is needed to detect occurrences of combinations of multiple events, i.e., to detect so called \textit{composite events}. 
%Previous approaches that have been proposed to detect composite events in active systems such as \cite{Chak94VLDB,Gatz93RIDS,Geha92VLDB,Zimm99DE} cannot be reasonably employed to detect composite events in XML due to the peculiarities of events in XML which are as follows.
%Detecting composite events 
This has long been studied in the active database literature where \textit{event algebras} have been proposed for the description of composite events (e.g., cf. \cite{Chak94DKE,Gatz93RIDS,Geha92VLDB,Zhan96TR,Zimm99DE}) and several techniques for realizing detection of composite events have been proposed, namely event graphs \cite{Chak94VLDB}, state automata \cite{Geha92VLDB}, and petri nets \cite{Gatz94RIDE}.

Events in XML, however, differ from the concept of events in literature as follows:

\begin{itemize}
\item[(1)] XML events are not only ordered by time but also by hierarchical structure. It is mostly undesired to use hierarchically unrelated events to form composite events as previous approaches do.
%
\item[(2)] An XML schema may constrain the number of element and attribute occurrences in documents. Existing approaches do not support the detection of when such constraints are satisfied.
%
\item[(3)] Event types, which are descriptions of events at the schema level, are hierarchically related as their events are. This allows for more expressive and more reusable event type definitions than in previous approaches.
%
\end{itemize}

Due to the above peculiarities of XML events, existing approaches for detecting composite events, such as \cite{Chak94DKE,Gatz93RIDS,Geha92VLDB,Zhan96TR,Zimm99DE}, cannot be reasonably employed for XML events because one encounters the following problems: (i) depending on the order of multiple modifications that all result in the same XML data different composite events are detected, (ii) most of the detected composite events are meaningless since they are not hierarchically related, they have to be filtered out by application code, (iii) it cannot be detected when multiplicity constraints defined by an XML schema are satisfied, and (iv) event types are unrelated and their extents are disjunct, limiting expressiveness and reusability of composite event type definitions.
For a motivating example that shows problems i and ii when using a refined existing approach see Subsection~\ref{section:motivating-example}.

The contribution of the chapter is to present an approach to detect composite events in XML that takes the above peculiarities of XML events into account.
It \textit{refines} an event algebra known from literature by defining the employed abstract model for XML data, XML events, and XML event types. Thereby it provides for more expressive and reusable event type definitions (addressing peculiarity 3).
Moreover, it \textit{extends} the semantics of the refined event algebra by introducing the hierarchical context to combine events according to hierarchy (addressing peculiarity 1), by introducing the multiplicity operator to detect when multiplicity constraints are satisfied (addressing peculiarity 2), and by introducing operator modifiers to provide for more expressive event type definitions. 

In particular, the presented approach refines and extends the event algebra Snoop \cite{Chak94VLDB,Chak94DKE}, because it is both extensible and well suited for XML. 
Snoop is extensible because it uses contexts to define the semantics of an event expression, thus by defining a new context semantics can be extended. 
Snoop is well suited for XML because \textit{event trees} are used to realize event  expressions and demonstrate event detection. Event trees fit well for processing XML events because they are hierarchically ordered as well.
Moreover, Snoop is used in the Sentinel active DBMS, is prominent among \cite{Gatz93RIDS,Geha92VLDB,Zhan96TR,Zimm99DE} according to CiteSeer\footnote{\url{http://citeseer.nj.nec.com}}, and is still subject to active research \cite{Adai2002TR}.



==> composite-events/multiplicity.tex <==
\subsection{Multiplicity Operator}
\label{section:multiplicity-operator}

%Motivation: snoop's contexts selektieren bzw. kennen keine Anzahl, daher muss operator eingeführt werden

Because an XML schema can define multiplicity constraints on XML elements and attributes it is desirable to be able to detect when multiplicity constraints are satisfied by observing occurred events. A multiplicity constraint is defined by lower bound $l$ and upper bound $u$ ($l \leq u$), meaning that between $l$ and $u$ child elements or attributes with the same name may occur as child of a parent element. After $l$ events reflecting insertions the multiplicity constraint is satisfied (if the parent element did not contain any such child elements before).
The operator from Snoop that closest resembles the required functionality is the {\tt ANY} operator. It detects a fixed number $>0$ of events of distinct event types, however, in XML the required number is $\geq 0$, since 0 events reflect optional elements, and the events are of the same event type.

To detect when multiplicity constraints are satisfied unary multiplicity operator ``$\times$'' is introduced, denoted as $\times [l,u]E_i$. It raises a composite event as soon as $l$ events of $E_i$ occurred, thereby indicating the constraint's satisfaction. The consumption of the composite event, however, may take place after other events of $E_i$ occurred. To provide composite events with most extensive sets of constituent events, the multiplicity operator has \textit{integrative semantics}.

Event integration starts after composite event $e^c_1$ is raised upon the occurrence of the $l^{th}$ event of $E_i$. A subsequently occurring event gives rise to the new composite event $e^c_2$ which integrates $e^c_1$'s constituent events. Event $e^c_1$ is waived because it has been integrated and is thus assumed not to be of interest any longer. If $u$ is reached or the integrating composite event is consumed, integration is suspended and starts over after the $l^{th}$ occurrence of $E_i$. 
%[LEAVE OUT] If $l=0$ an integrating composite event is raised without child events at $t=0$ and immediately after the last integrating composite event has been consumed.

When employed in a hierarchical context, the multiplicity operator shows the above behavior for every distinct path instance of its path type.
If not specified explicitly, a multiplicity operator's path type is set to the child node's path type omitting the last step. The same constraints on a multiplicity operator's path type must apply as on other operator's path types (see Subsection~\ref{section:hierarchical-context}).
Multiplicity operator $o$ raises a composite event $e^c_{1}$ as soon as there exist $l$ child events that equal in $\pi_{o.et.pt}(e_{i_j}.pi)$ for $1\leq j \leq l$. Thereafter it raises new composite event $e^c_{2}$ upon the occurrence of child event $e_{i_k}$ where $\pi_{o.et.pt}(e_{i_k}.pi) = \pi_{o.et.pt}(e^c_{1}.pi)$ if $e^c_{1}$ has not been consumed yet, where $e^c_{2}.cevts$ is defined by the union of $e^c_{1}.cevts$ and $e_{i_k}$. 

\begin{example}
% Example for multiple events
The event tree depicted in Figure~\ref{fig:evtgraph.mult-op} allows multiple insertions of ${\sf quantity}$ elements as childs of element ${\sf item}$. 
For two insertions of ${\sf quantity}$ elements $e_{q_{1.1}}$ and $e_{q_{1.2}}$ the multiplicity operator first raises composite event $e^c_{q_1}$ upon the occurrence of $e_{q_{1.1}}$. 
If $e^c_{q_1}$ has not been consumed upon the occurrence of $e_{q_{1.2}}$ new composite event $e^c_{q_2}$ is raised, where $e^c_{q_2}.cevts=\{e_{q_{1.1}}, e_{q_{1.2}}\}$, and $e^c_{q_1}$ is waived.
Otherwise, i.e., if $e^c_{q_1}$ has been consumed new composite $e^c_{q_2}$ is raised as well, however, with $e^c_{q_2}.cevts=\{e_{q_{1.2}}\}$.
\end{example}

\begin{figure}[h]
    \begin{center}
        \includegraphics[scale=1.3]{composite-events/evtgraph3c}
        \caption{Event Tree using a Multiplicity Operator}
%and (2) semantically unequal trees for $E_i {\tt ;} (E_p \bigtriangleup E_{pt} \bigtriangleup E_q \bigtriangleup E_{qt})$ and $E_i {\tt ;} ((E_p \bigtriangleup E_{pt}) \bigtriangleup (E_q \bigtriangleup E_{qt}))$}
        \label{fig:evtgraph.mult-op}
    \end{center}
\end{figure}

A multiplicity operator in hierarchical context with a lower bound of zero raises a composite event without the occurrence of a child event.
Instead, composite event $e^c_1$ is raised with the event representing the creation of (absolute) path instance $pi$ that satisfies the constraint of multiplicity operator $o$ by having $o.et.pt \subset_{\sf e} pi.pt \vee o.et.pt=pi.pt$. It does not comprise any constituent event, its path type is set to $pi.pt$, and its path instance to $pi$. 
%
Analogously, such composite events are raised when an event graph is registered with a document for every path instance $pi$ in the document that satisfy the condition above.
%
When event $e_i$ with $\pi_{o.et.pt}(e_i.pi)=\pi_{o.et.pt}(e^c_1.pi)$ subsequently occurs in $o$'s child node before $e^c_1$ is consumed, new composite event $e^c_2$ which integrates $e^c_1$ is raised. If composite event $e^c_2$ is consumed later on and $e^c_2.pi$ still exists, new composite event $e^c_3$ is raised since $o$'s constraints are still satisfied.

\begin{example}
% Example for optional event
The event tree depicted in Figure~\ref{fig:evtgraph.mult-op} allows optional element ${\sf comment}$ as child of element {\sf item}. With the insertion of ${\sf item}$ element ${\sf i_1}$ composite event $e^c_{c_1}$ occurs with $e^c_{c_1}.et.pt={\sf /order/item}$ and $e^c_{c_1}.pi={\sf /o_1/i_1}$. Thereafter, the conjunction operator raises composite event $e^c_{h_1}$ as soon as matching events are stored in its other child nodes, i.e., as soon as ${\sf p_1}$ and ${\sf q_1}$ are inserted as childs of ${\sf i_1}$. If matching ${\sf comment}$ element ${\sf c_1}$ is inserted before both elements ${\sf p_1}$ and ${\sf q_1}$ are inserted, event $e^c_{c_2}$ integrating $e^c_{c_1}$ is raised which becomes a part of $e^c_{h_1}$ later on.
\end{example} 

==> composite-events/open.tex <==
\section{Open}

\begin{itemize}

\item OK: reuse of event graphs with relative path types

\item ``inverse actions'': ins($e_1$), del($e_1$)

\item net effect of actions: e.g., multiple upd($s/text()$), or multiple *(/a/@x). 

\item New primitive event (wildcard) ```*''? Wildcard primitive event for xs:any?

\item is a not operator necessary, what happens in an active subtree if an event therein occurs that does not match an event node in the subtree?

\item how can one differentiate between an update and an insert? e.g., in Example below, an ins(/a/b) may be both Ins(A)@/a/b and Upd(A)@/a/b? Analogously an del(/a/b) may be both Del(A)@/a/b or Upd(A)@/a/b.
Can this only be decided from the context, i.e., Ins(a) or Upd(a)? Thus fire both and see what happens?

\item optional element: shall there be an element node and $\star[0,n]$ node in the event graph, or shall there be no nodes at all?

\item delete

\item Schema validity?

\item Substitution

\item Generalization

\item Treat attributes equal to Elements?

\end{itemize} 

==> dank2.tex <==
\chapter{Acknowledgements}

% ä:ä ü:ü ö:ö

{\em Es war einmal vor langer Zeit und das war eine sehr gute Zeit da war eine Muhkuh die kam die Straße herunter gegangen und diese Muhkuh die da die Straße heruntergegangen kam die traf einen schönen tleinen Tnaben und der hieß Tucktuck-Baby...}

\medskip
Indem ich also den Einstieg, den ersten Satz, mit obigem Zitat antrete, das übrigens seinerseits der erste Satz eines Buches von James Joyce ist, habe ich den für mich schwierigsten Teil der Danksagung bewältigt. Dass durch die Auswahl des einen eine Unzahl anderer nicht berücksichtig werden kann, muss verziehen werden. 
Dabei ist unter Umständen zu bedenken, dass die Wissenschaft einer persönlichen Eigenschaft förderlich zu sein scheint, die Flaubert in seinem Wörterbuch der Gemeinplätze den Advokaten zuschreibt: ``Vor lauter Für und Wider ist ihre Urteilskraft verdorben''.

\medskip
Wem mein Dank gilt, ist ungleich einfacher zu bestimmen, denn alleine hätte ich diese Arbeit nicht zu Stande gebracht:

Ich danke meinen Betreuern, Gerti Kappel und Michael Schrefl, die einen wesentlichen Beitrag zu dieser Arbeit, direkt und indirekt, geleistet haben. 
Danke für euren Einsatz, eure uneingeschränkte Hilfsbereitschaft,
%Danke Gerti, 
für das produktive Umfeld, in dem es ausreichend Freiheit für die Erfüllung abwechslungsreicher und ambitionierter Aufgaben gab, und
%Danke Michael, 
für das Vorleben eines wissenschaftlichen Enthusiasmus und eines Ideenreichtums, der ständiger Motivator war.

Danke meinen Kolleginnen und Kollegen, für die interessante Zusammenarbeit in Forschung und Lehre. Für die fruchtbaren Diskussion, die ausgetauschten Ideen, für die sinnvollen als auch die sinnlosen, die Anregungen und die Unterstützung. Namentlich bedanke ich mich bei Margit Brandl, Sabine Graf, Stefan Lechner, Elke Michlmayr, Günther Preuner, Michael Schadler, Sonja Willinger
und insbesondere meinen jahrelangen Bürokollegen Gerhard Kramler, der mir durch seinen Blick hinter die Dinge sehr viel gezeigt hat, und Thomas Thalhammer, der mir mit seiner typischen Tatkraft beim Einstieg immer hilfsbereit zur Seite stand.

Danke auch an die Studierenden, die durch die prototypische Realisierung der Ansätze und ihr Feedback ihren Anteil an der Arbeit haben, namentlich Werner Enser, Jan Wenger, Florian Sonntag und Christian Sokop.


==> document-flows/conclusion-webs.tex <==
In this paper, we presented an infrastructure model and an ontological
framework for semantically describing document flows.
%that are comprised of all existing distributed versions of a document as together with the relationships between these versions. The latter evolved when exchanging documents in a peer-to-peer setting.
As we showed in Section~\ref{section:applicationscenarios}, this light-weight communication
infrastructure for information exchange and collaboration can be used
in a variety of application scenarios. In addition, we demonstrated
that semantic descriptions considerably improve collaboration.

%Future Work: user interface.



==> document-flows/implementation.tex <==
\section{Implementation}
\label{section:implementation}

We have implemented a proof-of-concept prototype using JXTA as our P2P platform. Regarding identifiers, PIDs are URNs in the {\sf jxta} namespace, DIDs and VIDs are UUIDs expressed as URNs. Thereby the prototype is independent of physical network addresses, i.e., peers and versions can be physically moved on a network without affecting their identifiers. The resolution of URNs to network addresses is provided by JXTA.
%
%\begin{figure}[h]
%    \begin{center}
%        \includegraphics[scale=0.9]{peerinfo}
%        \caption{Browsing Document Flows}
%        \label{fig:prototype-browse}
%    \end{center}
%\end{figure} 
%
%[shorten] Figure~\ref{fig:prototype-browse} depicts a screenshot of the prototype while browsing a document flow. 
Using the prototype, the user can navigate to preceding and following versions starting from any peer and any version, can retrieve more information including annotations about the version, and can read the version's contents. 
Because, among others, peers and versions are published using so called JXTA advertisements, they can be dynamically discovered using JXTA's Peer Discovery Protocol as well. 
%[shorten] aside of navigating from one peer/version to another.
%[shorten] The list of peers shown in the figure comprises dynamically discovered peers using the JXTA Discovery Service. The user interface of a check-out has already been shown in Figure~\ref{fig:prototype-checkout}.

For a different user interface to peers and a seamless integration with standard email clients, we have implemented a dedicated component. 
It comprises an SMTP-Filter and an IMAP/POP3-Agent, as shown in Figure~\ref{fig:semantic-email}. They are transparent to users and operate in a non-intrusive
way. When a user wants to re-distribute a version to another user, she simply creates an email and attaches the version's data file to it. The SMTP-Filter checks out a following version on behalf of the user, thereby receiving the data- and metadata file from the peer. Subsequently it either 
sends the version to the recipient by email (step {\sf a.1} in the figure)
or checks it in at the destination peer (alternative step {\sf b}). In the former case, the recipient's IMAP/POP3-Agent detects the received email and checks the version in on behalf of the recipient (step {\sf a.2}). In either case the recipient is notified by an email which also contains the original message sent by user {\sf A} (not comprising the attached file).
Other user interface to peers, such as via HTTP and Web Services, are reasonable, but have not been implemented yet.

\begin{figure}[t]
    \begin{center}
        \includegraphics[scale=1.1]{document-flows/semantic-email}
        \caption{Sending and Receiving Traceable and Queryable Email}
        \label{fig:semantic-email}
    \end{center}
\end{figure}

%@@describe implementation of event delivery and measurements comparing it with JXTA 

==> document-flows/index.tex <==
%[TDF abstract from paper] Ad-hoc data exchange, e.g., by sending email attachments, leads to multiple copies or versions of a document at dispersed nodes in a network. However, their relationships such as is-a-version-of are lost. The relationships between a single document's existing versions together with the versions themselves form a so-called document flow, which allows to trace where a document originated and how it was distributed from node to node. The paper proposes an ontological, machine-processable framework for semantically describing and thus revealing document flows. The presented approach provides a light-weight communication infra\-structure for information exchange and collaboration that is based on distributed versioning of documents and offers flexible document annotation mechanisms. After describing our infrastructure model, we present the implemented prototype and discuss a range of application scenarios for traceable document flows (TDFs). 

This chapter describes the first layer of the two-layered extension to AXS. It provides for traceable document flows, abbreviated {\em TDFs}, and is also referred to as {\em layer IM-1}.

To exemplify the layer's, i.e., TDFs' usefulness, consider the following problems with which on is regularly confronted in today's personal ad-hoc data exchange, e.g., via email.
First, it is hardly possible to determine where
a document in one's file system originated. Usually answers to this
question are found after human inquiries using one's email system.
Second, it is even more difficult to determine who read or edited a
document before. Usually this involves lengthy inquiries and requires
interviewing other people.  Third, metadata about the document, if not
stored proprietarily as part of the document, e.g., as it is the case
with documents in Sun StarOffice or Microsoft Office format, are lost
during data exchange between individuals. Again, harvesting metadata
is a human task carried out by determining and interviewing people
who read or edited the document before.

Section~\ref{section:applicationscenarios} continues to exemplify TDFs' usefulness by describing four application scenarios where TDFs can be beneficial.
The first scenario in Subsection~\ref{section:AppScens-Email} shows how TDFs can be
used to trace documents exchanged via email, e.g., for the use by a
program chair who sends papers and review forms to program committee
members. 
The second scenario in Subsection~\ref{section:AppScens-CollabAuthoring} describes the use of TDFs for
collaborative authoring, e.g., when editing or writing a book. 
The third scenario in Subsection~\ref{section:AppScens-Workflows} shows how TDFs can be used as a light-weight
infrastructure to support workflows, either to discover existing
workflows (bottom-up) or to model workflows and constrain document
flows (top-down). 
The last scenario in Subsection~\ref{section:InformationExchange} shows how TDFs can be utilized to
share papers in a scientific community, e.g., to share metadata about
papers and determine domain experts.

The chapter is organized as follows.
Section~\ref{section:document-flow} presents the infrastructure model for traceable document flows. It comprises documents, versions, locations, and
interactions thereon. In parallel, an ontological framework is
presented with which artifacts such as a concrete document or a concrete version can be described.
Section~\ref{section:applicationscenarios} presents
the above application scenarios, 
Section~\ref{section:implementation} sketches a prototypical implementation 
and 
finally Section~\ref{section:related-work} discusses related work.

\section{Infrastructure Model and Ontological Framework}
\label{section:document-flow}
\input{document-flows/versioning}

\input{document-flows/usecases-webs}

\input{document-flows/implementation} 

\input{document-flows/related} 

==> document-flows/ontological-framework.tex <==
\onecolumn
\section{Appendix: Ontological Framework}
\label{section:appendix-rdf}

This section shows the ontological framework expressed in RDF Schema
\cite{W3C2004RDFS} for modeling documents, versions, and
peers. Whenever possible, we rely on properties defined by the Dublin
Core Metadata Initiative \cite{DCES2003}. The properties
that model the interactions with peers, such as \texttt{checkin},
\texttt{checkout}, and \texttt{read} are omitted for brevity.

\begin{Verbatim}[fontsize=\small]

\end{Verbatim}


==> document-flows/related.tex <==
\section{Related Work}
\label{section:related-work}

Regarding traceable document flows many distantly related approaches exist which provide the generic functionality of exchanging documents.
Among them are e-Mail systems, ebXML, BPEL, and SOAP. When using any of these, however, identities of exchanged documents are not preserved and thus the flow is not traceable.
Approaches that are closer related are those from office information systems in the 1980s dealing with form management, e.g., \cite{Tsic1982CACM} presents among others forms that can flow through an organization. It differs from traceable document flows with respect to flowing artifacts (only proprietary forms can flow), the data model (versioning is not employed), and the architecture (using central nodes).

Traceable document flows are new to P2P applications, which provide for distributed computing, file sharing, and online collaboration \cite{Milo02HP}. Among them, the closest related application is instant messaging, but again, identities of exchanged documents are not preserved.
Nevertheless, techniques of existing approaches can be employed, e.g., for version discovery using a central index as in Napster\footnote{\url{http://napster.com}}, flooded requests as in Gnutella\footnote{\url{http://rfc-gnutella.sourceforge.net}}, or distributed index structures using super-peers as in FastTrack\footnote{\url{http://www.fasttrack.nu}}. Approaches for directed routing using distributed hash tables (DHTs), which assign an identifier to a version based on a hash of its content and name and store it at peers with similar identifier (cf. \cite{Bala03CACM,Milo02HP} for an overview), cannot be used for discovery because versions in our model cannot be allocated freely.

Concerning distributed concurrent versioning systems, the most
prominent existing systems are CVS\-up~\cite{CVSUp04} and
DCVS~\cite{DCVS04}. However, both of them are based on the
client/server-paradigm and provide repository replication.
They can thus only provide for virtual document flows and can
not be compared to TDFs which are based a P2P model and
support physical document flows.

There is a model for encoding semantic information in P2P networks,
namely the SWAP metadata model~\cite{Broe03WWW} that takes a similar
approach of annotating information with metadata about its
origin. Unlike our approach which does not change the format of
documents, all information is additionally converted to RDF
representations. The SWAP model assumes that data is not physically
replicated between peers but rather queries are used for information
exchange. Since document distribution is an important enabler for
TDFs, this a a major difference. An interesting approach is the query
routing algorithm REMINDIN'~\cite{Temp04WWW} designed for the SWAP
platform. It uses observation of other peers' queries and answers to
determine their domain knowledge and to decide who is the right peer
to answer a certain query. An adaption of this %idea resp. its
algorithm for TDFs would be useful for the information exchange
scenario presented in Subsection \ref{section:InformationExchange}.



==> document-flows/usecases-webs.tex <==
\section{Application Scenarios}
\label{section:applicationscenarios}

% @@The main area of application for TDFs is document exchange across company or organization boundaries. The premise is that there is no common information infrastructure to rely on. TDFs are useful in every environment where individuals are discussing or working on a shared subject under the use of artefact documents and where traceability of the exchange of these documents is important.

This section present four exemplary application scenarios for TDFs. 
Namely, these are traceable email, collaborative authoring, workflows, and information exchange. 
In the second and the third scenario, it can safely be assumed that the
contents of versions are not private and that people are willing
to let others know where their documents originated, i.e., it is
agreed that user specific data is available for others. 
%
In the first and the fourth scenario, however, privacy concerns may arise. There are several
possibilities which can be used alone or in combination to resolve
them: First, user data can be made anonymous while still exploiting its
value. This is possible by aggregating the metadata and providing
statistical data interpretation, e.g., for features like ``users who read
this document also read...''. Second, one can implement
authentification and authorization to specify and reveal what users
are allowed to read.  It is not dealt with details of privacy
issues, which is assumed to be outside the focus of this work.

\subsection{Traceable Email}
\label{section:AppScens-Email}

Usually when sending and receiving files via email knowledge is lost. 
This knowledge comprises, among others, who originally created the file, who else received and read or edited the file before or after myself, and what other people know about this file in the form of semantic annotations. The loss is caused by (1) missing support of file systems, e.g., for globally unique identifiers; (2) by missing support of email clients, e.g., for functionality like querying where a file originated or querying remotely stored annotations; and (3) by missing integration of the two, e.g., for determining whether I have sent a file to someone else or for determining that a received file is a successor version of a locally stored file.

By providing a component that transparently enables people to use TDFs for files they have sent and received via email we provide them with {\em traceable email}. The component we have developed is described in more detail in Section~\ref{section:implementation}. 
Basically it filters outgoing email messages and in case it detects a version's datafile attached to an email, a succeeding version is checked out from the sender's peer and sent to the recipient. There, an agent filters incoming email messages and in case a version is attached to an email it automatically checks it in at the recipient's peer. 
%This neutralizes reasons (1) to (3) of knowledge loss mentioned before and provides the user with functionality described below.

When using traceable email for tracing files that are exchanged via email otherwise lost knowledge is preserved and new knowledge is unveiled.
%
Using traceable email, users can easily determine not only from whom a file was received, but also where it originated and who else was in possession of the file before. Users can determine to which persons a file they have sent is re-distributed further on. They can also read the contents of any of these versions of the file.
%
Moreover, traceable email provides a non-proprietary possibility for storing and querying also remotely stored annotations about files that were received or sent as email attachments, thereby unveiling annotations of other people.

An exemplary use of traceable email is the management of a paper review process. 
After submission, e.g., via a web application, which created a document and an initial version, the program chair checks out a following version of each paper and sends it (i.e., the data file) and the review form (i.e., the metadata file) to program committee members. Note that the review form is an annotation to the version, expressed according to an ontology for reviews.
%To manage revised submissions, {\it following versions} can be utilized. 
%Since committee members receive the papers to review by email,
Committee members possibly forward received papers to additional (sub-) reviewers. After each reviewer has filled out his/her review form, he/she sends it back to the super-reviewer or to the chair where it is checked.
% In the last step they send the documents, which are now annotated with the reviews, back to the program chair. 
This approach is very flexible and allows the chair to query for the status of each review at any time. Also an aggregated report summarizing all reviews of a paper can be easily created by querying the annotations.
%about the overall status of all reviews is possible on the fly by metadata querying.

%@@vorteil gegenueber existierenden webbasierenden systemem?

Comparing traceable email with related work \cite{Etzi03WebDB}, the latter focusses on defining machine-processable email contents, while we focus on revealing a document's flow that is established via email.

\subsection{Collaborative Authoring}
\label{section:AppScens-CollabAuthoring}

TDFs can be employed for collaboratively editing documents like version systems in general can be used for this purpose. 
%
Different from version systems, however, TDFs do not imply the need for a central shared document repository, which may be not available. 
%
Moreover, the annotation mechanism of TDFs is superior compared to the log facility of version systems such as CVS.
While in both cases annotations marked up using an ontology can be made, where the ontologies used can be freely chosen, only with TDFs the annotations are hooked into the provided ontological framework. Thereby, semantic descriptions of version graphs, not available in CVS, are provided along and aligned with annotations.
%

%The advantages that peer-to-peer networks provide are fully exploited when authors work offline, e.g. can not access network resources. If they are able to connect their devices, e.g. using Bluetooth or a network cable, they still can exchange document versions.

For example, consider the complex collaborative task of writing an
edited book. For each book chapter, there are multiple authors working
together. Hence it is necessary to create a document for each
chapter. For all of these documents, {\sf df:FreezeNonCurrentVersions} is
set to true. Thus only the author in possession of a current version
owns the ``edit token''. She/he can edit the draft of the chapter and
hand it on to a co-author afterwards. It is also possible that
authors work in parallel on branched versions and merge their changes afterwards. At any moment, the editor can determine the status of each chapter. In addition, the authors can have a look at the current versions of the other chapters, e.g. to align their terminology or their references.

\subsection{Workflows}
\label{section:AppScens-Workflows}

In environments where a workflow management system (WfMS) is not available and/or where it is impossible to deploy one (e.g., when a shared, central WfMS cannot be negotiated) or where it is unreasonable to deploy a WfMS (e.g. too costly or time-consuming), TDFs are a light-weight alternative infrastructure for workflow management. Such environments are faced more and more often with the increase of workflows crossing organizational boundaries. And, starting from the observation that documents are the basis of collaborative work applications, it is natural to think about documents as basic coordination entities for workflows.

Employed {\em top-down}, TDFs enables one for the definition of workflows in the form of document flows. In particular, a workflow type at the schema level is defined by describing a document flow type to which certain document flows must adhere to.
This assumes that the workflow can be modelled in term of a document flow, however, if a document flow from the application domain cannot be used, an artificial ``control'' document flow can be introduced.
As an example (assuming every user has its own peer), user A can instruct user B to proofread a document by handing it over to him, followed by user C who has to add a reference into an internal library catalog, and user D who has to give her permission for its publication (e.g., stored as signed annotation), where user C and D can work in parallel.
With TDFs, users can query for subsequent steps at any time and peers can restrict the document flow to a valid one, i.e., to one that accords to its type.

Obviously, an extension to TDFs is needed to model and execute document flow types.
%
First, for modelling document flow types, an appropriate ontology has to be defined and used. One could start from the workflow patterns defined in \cite{Aalst03DDB} and map the control flows defined there to document flows. This may involve defining the concept of composite document or record, which contains multiple documents and might control the document flow, e.g., by using reactive rules as described in \cite{Kapp95IEEE} and the functionality provided by the active extension to TDFs described in Section~\ref{section:ActiveExtensionForTDFs}.
%
Second, for executing document flow types, peers must be extended to either interpret descriptions of document flow types directly or indirectly. A possibility for the latter would be, as mentioned before, to map document flow types to reactive rules and to interpret the rules as provided by the active extension to TDFS described in Section~\ref{section:ActiveExtensionForTDFs}.

TDFs can also be used in a {\em bottom-up} way for workflows. Since the metadata describing document flows logs how versions were distributed across a network, it can be analyzed ex post to discover document flows that took place regularly. They can be possibly abstracted to document flow types further on. This way, workflow analysis can be carried out by investigating existing document flows. 

\subsection{Information Exchange}
\label{section:InformationExchange}

This scenario is comparable to well-known P2P filesharing applications like
Gnutella\footnote{\url{http://rfc-gnutella.sourceforge.net}}. The focus is on exchanging {\em static}
documents, meaning that all versions of a document have the same
content. Thus annotations are not longer specific for a single version of a
document but for all of them. 
Here, the revelation of document flows, the possibility to annotate versions, and the possibility to query this metadata distinguishes TDFs from other filesharing applications. Of course users are not forced to annotate their documents,but decide by themselves how much time they spend for annotation.

An example of this application scenario is that of scientists working
on the same subject. Typically, they all use a folder in their local
file system to store and manage their collection of scientific papers
related to their research field. 
%
If they use TDFs to share their folder and annotations with others, every user can benefit from observing which documents other users have read, e.g., for answering questions like ``users who read this document also read...'' or for determining researchers working in the same field.
%
Furthermore, using TDFs it is possible to find out all existing versions of a given document or all documents having at least a single version that share the same datafile.
The total number of these can then be used to rank documents, and the peers where these are stored may form a list of potential contact addresses for comments and questions.
%
Summarized, most value of employing TDFs for information exchange can be expected to come from sharing annotations and semantic descriptions of stored files, not from revealing particular document flows.

% The outcome of a query determining all peers where a document's versions are stored at may form a list of potential contact addresses (e.g., persons). 
% @@Most value can be gained from these features if the shared documents are related to a single domain. ->??
% Moreover, one can determine researchers working in the same field, determine domain experts for a field, or simply read annotations of other users.
% Moreover, using TDFs previously unknown information can be discovered by exploiting document flow metadata. 

==> document-flows/versioning.tex <==
This section presents the infrastructure model for TDFs, which employs versioning as known from configuration management \cite{Conr1998ACMSurvey}. 
%Basically, it is the result of mapping an extended version model to a P2P model.
%@@TDFs use several concepts (see later in this section). 
To make instantiations of the model's concepts interoperable and thus available for other applications, we employ Semantic Web technology to describe them, i.e., OWL \cite{W3C2004OWLGuide}. 
We define an ontological framework for document flows comprising these concepts, which are used when describing instantiations.
%[shorten] (the framework is shown in detail in Appendix~\ref{section:appendix-rdf}). 
Being a framework, any other ontology can be used in addition, e.g., for annotating documents. The use of additional ontologies is influenced by the  given application as is exemplified in Section~\ref{section:applicationscenarios}.

\subsection{Documents and Versions}
\label{section:basic-model}

A document is identified by a {\em document identifier} (DID) and keeps its identity across modifications. Since the model is intended to be implemented on the Web, a DID is a URI \cite{IETF1998URI}. Between two subsequent modifications a document is represented by a static concrete occurrence having certain contents. In the presented model a document exists both as an abstract concept represented by its DID (referred to as {\em document}) and as set of concrete occurrences (referred to as {\em versions}). 
%[shorten] The term  {\em document} concisely refers  to a document as an abstract concept throughout the rest of the thesis.

%[shorten] To represent a concrete occurrence of a document at a point in time we use the concept of a {\em version} as known from configuration management. 
A version is identified by a {\em version identifier} (VID) which is a URI. A modification to a version in the presented model does not necessarily result in a new version, i.e., a version's content may change over time. All versions of a document together represent its history. 
A version's VID is globally unique, i.e., unique across documents so that it suffices to identify and retrieve the version.

\begin{example}
A document representing a purchase order and containing items to be ordered is identified by its DID, e.g., $d_{order}$. Each time an order item is added, modified, or deleted, a version of the document is modified. Selected versions may be made persistent and have an assigned VID, e.g., $v_1$ and $v_2$.
\end{example}

The underlying version model is organized as a two-level {\it acyclic version graph} (cf. \cite{Conr1998ACMSurvey}) that is composed of branches, each consisting of a sequence of versions. This model is employed in several version management systems such as WebDAV \cite{IETF1999WebDAV,IETF2002WebDAV} and CVS \cite{CVS.org}. While versions constitute the nodes in the graph, three relationships between versions are distinguished, namely successor, offspring (starting a new branch), and predecessor. Each version has at most one successor and possibly several offsprings in different branches. Successor and offspring versions together are also referred to as following versions. Because a version can be merged into a version of another branch, a version can have several predecessors.

Additionally to the used concepts known from version models, we introduce the concepts of a current version and a frozen version.
A {\em current version} is a version that has no succeeding version. Multiple current versions may exist per document in different branches. To provide for a consistent version graph, versions that are non-current can be {\em frozen} to prevent them from further being modified, avoiding that they become inconsistent with succeeding versions. Whether non-current versions are frozen is determined by configuration for each document separately (see below).
By not freezing a version a very unconstrained exchange of versions can take place, because a succeeding version does not prevent the version from being modified.

\begin{figure}[h]
    \begin{center}
        \includegraphics[scale=1.2]{document-flows/version-graph}
        \caption{Exemplary Version Graph}
        \label{fig:exemplaryVersionGraph}
    \end{center}
\end{figure}

\begin{example}
An exemplary version graph of $d_{order}$ is depicted on the left of Figure~\ref{fig:exemplaryVersionGraph}, showing five versions and three branches. Version numbers used throughout the thesis have an odd amount of numbers (digits) separated by periods, whereas numbers at odd digits count versions (e.g., $v_2$ for the second version) and numbers at even digits count branches (e.g., $v_{1.2.3}$ refers to the third version in branch $v_{1.2}$, which is the second branch following version $v_1$). In Figure~\ref{fig:exemplaryVersionGraph} versions $v_1$, $v_{1.1.1}$, $v_{1.2.1}$, and $v_2$ are frozen, while $v_3$ is a current version.
\end{example}

To talk about the topology of a version graph, {\em path} $p=(v_i, ... ,v_j)$ is defined as a sequence of versions starting with $v_i$ and ending with $v_{j}$, where version $v_k$  ($i \leq k < j$) is followed by $v_{k+1}$ in the version graph. Since version $v_k$ can have one successor and multiple offspring versions, several paths between $v_i$ and $v_j$ may exist.

\begin{example}
Concerning the version graph of document $d_{order}$ shown in Figure~\ref{fig:exemplaryVersionGraph}, paths $p_1=(v_1,v_{1.1.1},v_2,v_3)$, $p_2=(v_1,v_{1.2.1},v_2,v_3)$, and $p_3=(v_1,v_2,v_3)$ exist between $v_1$ and $v_3$.
\end{example}

Documents and versions are modelled as classes {\sf tdf:Document}\footnote{prefix ``{\sf tdf}'' denotes namespace \url{http://www.big.tuwien.ac.at/research/documentflows/1.0/}} and {\sf tdf:Version} and are described by several properties.
%
At minimum a document as wells as a version must be described by properties {\sf tdf:title} and {\sf tdf:description}. Being URIs, a document's DID as well as a version's VID are used directly as identifiers in semantic descriptions.
%
Each document must be additionally described by property {\sf tdf:freezeNonCurrentVersions}, which defines whether its non-current versions are frozen. Its value is specified when the document is created.
%
Each version must be additionally described by property {\sf tdf:isVersionOf}, which relates it to the document it is a version of.
Moreover, a version may have successor versions (property {\sf tdf:hasSuccessorVersion}), offspring versions (property {\sf tdf:hasOffspringVersion}), and preceding versions (property {\sf tdf:hasPrecedingVersion}). A version may be stored at a peer (property {\sf tdf:isStoredAt}).
%
Of course, additional ontologies can be used to further describe documents and versions, i.e., to describe a user's annotations.

Classes and properties describing documents and versions are closely linked to elements and qualifiers of the Dublin Core \cite{DCES2003}, thereby grounding them on commonly understood semantics. 
%
The relationships are as follows:

\begin{enumerate}
\item {\sf tdf:name $\sqsubseteq$ dc:title}\footnote{prefix ``{\sf dc}'' denotes namespace \url{http://purl.org/dc/elements/1.1/}, see \cite{DCNSPolicy2001}}, \\
{\sf tdf:title $\sqsubseteq$ dc:title}, and \\
{\sf tdf:description $\sqsubseteq$ dc:description};
%(1) properties {\sf tdf:name}, {\sf tdf:title} and {\sf tdf:description} are sub-properties of {\sf dc:title} and {\sf dc:description}\footnote{prefix ``{\sf dc}'' denotes namespace \url{http://purl.org/dc/elements/1.1/}, see \cite{DCNSPolicy2001}} respectively;

\item {\sf tdf:isVersionOf $\sqsubseteq$ dcterms:isVersionOf}\footnote{prefix ``dcterms'' denotes namespace \url{http://purl.org/dc/terms/}, see \cite{DCNSPolicy2001}};

\item {\sf tdf:hasSuccessorVersion $\sqsubseteq$ tdf:hasFollowingVersion}, \\
{\sf tdf:hasOffspringVersion $\sqsubseteq$ tdf:hasFollowingVersion}, and \\
{\sf tdf:hasFollowingVersion $\sqsubseteq$ dcterms:isReplacedBy};
%(3) properties {\sf tdf:hasSuccessorVersion} and {\sf tdf:hasOffspringVersion} are both sub-properties {\sf tdf:hasFollowingVersion} which is a sub-property of {\sf dcterms:isReplacedBy};

\item {\sf tdf:hasPrecedingVersion $\sqsubseteq$ dcterms:replaces}, where \\
{\sf tdf:hasPrecedingVersion $\equiv$ tdf:hasFollowingVersion$^-$}, and \\
{\sf dcterms:replaces $\equiv$ dcterms:isReplacedBy$^-$}.
%(4) property {\sf tdf:hasPrecedingVersion} is sub-property of {\sf dcterms:replaces}, the inverse of {\sf dcterms:isReplacedBy}.
\end{enumerate}

\subsection{Locations}
\label{section:locations}

Since a document as an abstract concept cannot be allocated itself, versions are allocated at {\em locations}. Each version is allocated at a single location, while one location can host multiple versions of the same document. Note that the concept of location is new to version models and thus makes the presented version model more expressive. Locations form the basis for modelling the distribution aspect of documents.

The meaning that is associated with a location can be very diverse. It is assumed, however, that a location is in a close relationship to a natural or juristic person such as a version's creator and owner. This relationship may also be ``weaker'', e.g., to persons who process a version or are simply interested in its contents. Usually, locations have autonomy in how to handle allocated versions, e.g., in how to store, to version, and to control access. Thus a modified relationship to a person, such as modified ownership, is likely to go in parallel with a modified location.

A location is represented by a document peer, short {\em peer}, that serves as a repository for versions, communicates with other peers, and performs interactions requested by users on versions. Peers may differ in the interactions they support, however, they must minimally support the interactions described in Subsection~\ref{section:basic-interaction}. A peer is identified by a {\em peer identifier} (PID) which is a URI.
% [leave because negative] Because we see a peer as a Web server that is enabled for document flows, peers are assumed to have high availability in that they do not arbitrarily join and leave the network of peers. Thus peers do not have the ad-hoc connectivity that peers usually have in P2P systems \cite{Milo02HP}.

A peer is modelled by class {\sf tdf:Peer} and described by properties {\sf tdf:name} and {\sf tdf:description}. Moreover, property {\sf tdf:serves} has a peer as its domain and class {\sf tdf:Served\-Entity} as its range. 
%
The latter is the superclass of a set of predefined classes
{\sf wdn:Person}\footnote{prefix ``{\sf wdn}'' denotes namespace \url{http://xmlns.com/wordnet/1.6/} and identifies concepts defined by WordNet \cite{WordNet}},
{\sf wdn:Social\_group} (in turn superclass of, e.g., {\sf wdn:Organization}),
and {\sf wdn:Role}.
The set of predefined subclasses can be extended (by adding sibling classes) as well as further refined (by adding subclasses).
%@@{\sf storage device}
The predefined classification reflects addressees to whom document delivery in real life is targeted: (1) to persons; (2) to social groups such as organizations, departments of organizations, or clubs; and (3) to roles that are fulfilled by agents as in workflows. 
%
If a peer does not have property {\sf tdf:serves}, the entity the peer serves is unknown as it is the case with post office boxes.
%
By using classes defined by WordNet \cite{WordNet} the description is based on commonly understood semantics.

To maintain a document's version graph, the dependencies between multiple versions, which are likely stored at different locations, have to be maintained.
Following a P2P model, the version graph is maintained distributed. Because of the requirement of low coupling in a Web context, only references to directly preceding and following versions are maintained with each version stored at a peer.
This decision is also influenced by the assumption that navigation and communication from a version to its directly preceding and following versions is more likely to be possible (e.g., by a firewall configuration) and will occur more often than therefrom to other versions, e.g., the initial one. 

Having introduced locations, the rationale behind employing versioning can be refined which is different from the rationale in version management. While in the latter capturing modifications and identifying configurations is of primary concern, i.e., the {\em evolution aspect} of documents, the presented model employs versions to distinguish between and keep track of versions stored at different locations in a network, i.e., the {\em distribution aspect} of documents. Nevertheless, because the presented model is more expressive than known version models, it captures the evolution aspect as well.

A peer stores semantic descriptions of individuals of the concepts presented so far -- documents, versions, and peers -- and of interactions (see Subsection~\ref{section:basic-interaction}). It can be queried about locally stored individuals of these concepts, e.g., remote versions can be discovered by querying a local version to determine its preceding versions, offspring versions, and successor version. Aside of querying for other versions, semantic descriptions with application semantics of local versions can be queried as well. 

The presented approach can well be combined with related approaches to provide enhanced functionality.
First, for the replication of semantic descriptions which are currently only available locally, e.g., Edutella's replication service \cite{Nejd02WWW} can be used.
Second, for answering queries that search for an arbitrary version (i.e., not by navigating, starting from a known version), existing discovery mechanisms, e.g., provided by Gnutella\footnote{\url{http://rfc-gnutella.sourceforge.net}} or JXTA \cite{jxta.org} can be used. 
Third, for the resolution of a DID to a VID, e.g., of the initial version or current versions, existing mechanisms for resolving location-independent identifiers, e.g., URNs, can be used (cf. \cite{Werf1999a} for an overview).
Fourth, for querying semantic descriptions of a set of peers, related approaches such as Edutella \cite{Nejd02WWW} can be used.

% ############################################################
% # 

\subsection{Interactions on Documents and Versions }
\label{section:basic-interaction}

Because the presented model for TDFs is based on a version model, the interactions that are provided by peers mostly have counterparts in version management systems such as WebDAV and CVS, however, there are major differences.
First, the presented model is richer by dealing with locations, and second, there is no central control. Thus the semantics of interactions with counterparts differ to cope with locations and decentralization. Moreover, interactions without counterparts are introduced.

Depending on a version's environment it is in a certain state. When being allocated at a peer, the version is {\em checked-in}. Using appropriate interactions, a following version can be retrieved from a peer. The retrieved version has status {\em checked-out}. A checked-in version is {\em online} when the peer it is allocated at can communicate with other peers. Otherwise, or when the version is checked-out, it is {\em offline}. A checked-out version can be checked in using interaction \cmd{checkin}.

On checked-in version $v_i$ basically three basic interactions can be performed.
First, interaction \cmd{read} retrieves the version's content (or in Web terms a ``representation'' of the version).
Second, interaction \cmd{checkout} retrieves successor version $v_{i+1}$ or offspring version $v_{i.j.1}$ when used with option \cmd{successor} or \cmd{offspring}, respectively. 
Third, checked-in version $v_k$ that resides in another branch than $v_i$ can be merged into $v_i$ using interaction \cmd{merge}. Thereby, $v_i$ becomes the successor of $v_k$. The merged versions may be allocated at different peers. 
Merging the versions' contents can be done manually or automatically by approaches such as \cite{Font2002XMLEurope}.
%[shorten] Figure~\ref{fig:prototype-checkout} depicts a screenshot of performing a checkout with our prototype (cf. Section~\ref{section:implementation}).

%\begin{figure}[h]
%    \begin{center}
%        \includegraphics[scale=0.9]{checkout}
%        \caption{Checking out a Version}
%        \label{fig:prototype-checkout}
%    \end{center}
%\end{figure} 

When a version is checked out two files are retrieved from the peer its predecessor is allocated at. The first file contains the contents of the version and is thus called the {\em data file}. The second file comprises semantic descriptions concerning the version and the version graph (i.e., at least a single statement that uses the {\sf tdf:precedingVersion} property). The file is thus called the {\em metadata file}. 
Semantic descriptions that are available for the checked-out version's predecessor are taken over to the metadata file of the checked-out version. Which data is taken over depends on 
(a) what the user performing the checkout is allowed to read from the 
data available for the checked-out version's preceding version, and 
(b) which data the user performing the checkout is interested in.
For a checkin at a later date, both the data and the metadata file are necessary. The descriptions that were taken over are marked as such using appropriate statements. %(property {\sf df:takenOver}).

Note that different to WebDAV and CVS the \cmd{checkout} interaction in the presented model retrieves a following version not a representation, thus creating a following version at checkout time instead of the time when the modified representation is checked-in at a later date. 
It is essential to check out a version, which has its own VID assigned to it, so that it can be recognized as a version by humans and machines, making it possible, e.g., to send it to other people via email and most important to make statements about it using an appropriate language, e.g., RDF or OWL.
Moreover, if non-current versions are frozen, a checked-out succeeding version cannot become inconsistent with its predecessor. Whereby consistency means that the succeeding version cannot lack modifications that have been performed on its predecessor.

Aside of the interactions presented so far, which allow to construct version graphs, two interactions allow to modify version graphs. First, interaction \cmd{delete} removes a version from the version graph. Second, interaction \cmd{reallocate} stores a version at another peer which may involve modifying its VID if the VID is a location dependent identifier. 
%[shorten] In both cases the version graph is modified accordingly, e.g., property {\sf df:successorVersion} of a preceding version is modified.
A user who requests to perform an interaction on a version which has been deleted or reallocated is notified of the modification. Both interactions have to be used with caution, since external references to the version become ``broken''. 

%Semantic descriptions are updated upon deletion or reallocation.
The effects of a \cmd{delete} interaction are more complex than at first sight.
When version $v_i$ is deleted, the event graph has to be modified accordingly by connecting versions from the set of preceding versions $V_p$ with versions of the set of following versions $V_f$. If $v_i$ is an offspring version of preceding version $v_p \in V_p$, then $v_p$ is connected with each $v_f \in V_f$ by an offspring relationship. If $v_i$ is the successor version of preceding version $v_p$, and a following version $v_f$ is the successor version of $v_i$, $v_p$ and $v_f$ are connected by a successor relationship, otherwise by an offspring relationship. 
This is shown in Figure~\ref{fig:effects-delete}, where the upper part depicts version graphs before performing interaction \cmd{delete $v_2$} and the lower part after the deletion.
Furthermore, on the left side 1:1 connections are shown, while on the right side other combinations (n:1, 1:n, and m:n) are shown which can be inferred from from 1:1 connections.
Note that, while the descriptions of preceding and following versions are updated automatically, replications of descriptions of the affected part of the version graph maintained by other applications may become inconsistent.

\begin{figure}[h]
    \begin{center}
        \includegraphics[scale=1.1]{document-flows/eg-delete} %[width=6cm]
        \caption{Effects of \cmd{delete} Interaction on Version Graphs}
        \label{fig:effects-delete}
    \end{center}
\end{figure} 

For convenience three interactions are provided that are composed of previously mentioned interactions and which are therefore called {\em composite interactions}. Like the previously mentioned interactions, to which we refer to as simple interactions henceforth, composite interactions are atomic, i.e., they are performed as a whole or not at all.
Composite interactions determine the flow of a document, which is caused by allocating following versions at possibly different peers, more directly than simple interactions.
Namely, interaction \cmd{proceed} proceeds a version with a succeeding version, \cmd{branch} proceeds a version with an offspring version, and \cmd{copy} copies a version to a new document. 
As one can easily see, each of \cmd{proceed} and \cmd{branch} composes a \cmd{checkout} and \cmd{checkin} interaction, while \cmd{copy} composes a \cmd{read} and \cmd{checkin} interaction.
The composite interactions correspond to how paper forms and documents are handled in real life, i.e., they can be handed on or copied and distributed.
For a more precise characterization of composite interactions see the Appendix.

A peer does not only store semantic descriptions of documents and versions it hosts but also of semantic descriptions of interactions it has performed. 
An interaction is represented by an individual of class {\sf tdf:Interaction}, which is described 
by the user or peer who issued the interaction (property {\sf tdf:isIssuedBy}), 
by the peer that performed the interaction (property {\sf tdf:isPerformedBy}),
by the date and  time it was performed (property {\sf tdf:isPerformedAt}), 
and by the version the interaction is targeted at (property {\sf tdf:hasTargetVersion}).
%
Particular interactions are represented by pairwise disjunct subclasses, e.g., {\sf tdf:Read $\sqsubseteq$ tdf:Interaction} and {\sf tdf:CheckIn $\sqsubseteq$ tdf:Interaction}, where {\sf tdf:Read $\sqcap$ tdf:CheckIn $=$ $\emptyset$}.
Interactions {\sf tdf:CheckOut}, {\sf tdf:Reallocate}, and {\sf tdf:Merge} are additionally described by property {\sf tdf:hasSourceVersion}, which identifies (a) the preceding version of the target version being checked out, (b) the version being merged into the target version, or (c) the version being reallocated to the target version in case the VID changes due to reallocation (i.e., if the VID is a location dependent identifier).
%
Composite interactions are represented by individuals of class {\sf tdf:CompositeInteraction} and are composed of two simple interactions (property {\sf tdf:isComposedOf}). Three pairwise disjunct subclasses are distinguished for each particular composite interaction, e.g., {\sf tdf:Proceed $\sqsubseteq$ tdf:CompositeInteraction}.
%For details regarding the ontological framework see Appendix~\ref{appendix:ontological-framework}.

Like with documents and versions, additional semantic descriptions can be stored along each interaction. They can can be either 
application-independent, such as a comment in natural text (e.g., using property {\sf dc:description}), 
or application-specific, e.g., if the interaction corresponds to some state change in a workflow description.

Semantic descriptions of interactions can be useful in several situations.
%
This strongly applies for descriptions of \cmd{read}s, which can be used, e.g., for recommendations (see Subsection~\ref{section:InformationExchange}), as well as for descriptions of \cmd{delete}s and \cmd{reallocate}s can be used to inform users of deleted versions or to navigate to reallocated ones.
%
Descriptions of \cmd{checkin}s, \cmd{checkout}s, and \cmd{merge}s are less useful (which, however, depends on the application domain), because they also manifest in the version graph, which is not entirely the case for \cmd{read}s, \cmd{delete}s, and \cmd{reallocate}s. Therefor, their semantic descriptions primarily enable one to query versions' histories describing performed interactions.


==> eid.tex <==
\chapter*{Eidesstattliche Erklärung}

Ich erkläre hiermit an Eides Statt, dass ich die vorliegende Dissertation selbständig verfasst, andere als die angegebenen Quellen und Hilfsmittel nicht benutzt und die aus anderen Quellen entnommenen Stellen als solche gekennzeichnet habe. Diese Dissertation habe ich bisher weder im Inland noch im Ausland in irgendeiner Form als Prüfungsarbeit vorgelegt.

\bigskip
\bigskip
\bigskip
\bigskip
Wien, im Advent 2004



==> event-flows/active-extension.tex <==
This section presents layer IM-2 on top of the layer for document flows (IM-1) to enrich them by active behavior, thus providing for active traceable document flows. 
Basically, it is the result of mapping the publish/subscribe protocol to a P2P model.
By implementing this layer, peers become active and are henceforth called {\em active peers}. To define active behavior, the layer employs Active XML Schema (AXS).

The running example is a document flow from the workflow domain as mentioned in Subsection~\ref{section:AppScens-Workflows}.

\begin{figure}[h]
    \begin{center}
        \includegraphics[scale=1.3]{event-flows/example-df}
        \caption{Exemplary Document Flow}
        \label{fig:document-flow}
    \end{center}
\end{figure} 

\begin{example}
The procurement department quarterly determines the need for higher priced office supplies of operating departments. Therefore, it creates order document $d_{order}$ and initial version $v_1$. Furthermore, offspring versions $v_{1.1.1}$, $v_{1.2.1}$, etc. are created, one for each operating department and sent to them as shown in Figure~\ref{fig:document-flow}. After a month, the offspring versions are merged into version $v_{2}$ which succeeds $v_1$, consolidating the overall need (they cannot be merged  into $v_1$ since this would cause cycles in the version graph). Different locations represent different departments, i.e., $l_{proc}$ denotes the procurement department and $l_{op_1}$, $l_{op_2}$, etc. denote operating departments. Versions are persistent and can be used at a later date, e.g., operating departments can use $v_{1.1.1}$, $v_{1.2.1}$, etc. later on to look up office supplies ordered in that quarter.

To perform this document flow, the procurement department performs multiple interactions ``\cmd{checkout offspring of $v_1$}'' of document $d_{order}$ to retrieve offspring version $v_{1.i.1}$ for each operating department $l_{op_i}$. These versions are checked in at $l_{op_i}$ using interaction \cmd{checkin}. 
A successor version $v_2$ of $v_1$ is retrieved by performing ``\cmd{checkout successor of $v_1$}'' followed by a \cmd{checkin} at the same location. After one month branched versions $v_{1.i.1}$ are merged into $v_2$ by performing ``\cmd{merge $v_{1.i.1}$ into $v_2$} '' for each branched version, resulting in a single version $v_2$ at the procurement department comprising all items to be ordered.
Instead of using simple interactions as above, composite interactions \cmd{proceed}, \cmd{branch}, and \cmd{copy} can be used to perform the same document flow as done in Figure~\ref{fig:document-flow}.

After determining the overall need in office supplies the procurement department sends the order to the distribution department of a supplier company at $l^*_{distr}$ (again, cf. Figure~\ref{fig:document-flow}). To assure that the supplier company can handle the order independently of the purchasing company, the latter performs interaction ``\cmd{copy $v_2$ to $v^*_1$ at $l^*_{distr}$}'', which copies the version to the distribution department, assigning it to a new document. Throughout the rest of the chapter, locations, documents, and versions of the supplier company are marked by an superscripted asterisk.
\end{example}


\subsection{Employing Active XML Schema}

Active XML Schema (AXS) is employed on top of layer IM-1. Since AXS provides active behavior to XML documents only, the format of data files participating in document flows for which active behavior can be provided is restricted to XML.

{\em Briefly recalling AXS}, it allows one to specify active behavior by ECA rules and passive behavior by operations with XML schemas, thereby specifying behavior of XML documents that are valid instances of the schema. When an operation is executed on an XML document, an according event occurs, being of an event type (the event's intensional aspect) and stored in an event class (the event's extensional aspect). The event class in turn is stored as part of the XML document. When an event occurs, all rules defined upon the event class it is stored in are triggered, i.e., executed.

\begin{example}
AXS is used to define operations with the document type of $d_{order}$. Among others, operation \op{addItem(my:OrderItemType)} adds the item given via the parameter to an order and operation \op{removeItem(xs:integer)} removes the item with the given part-number from an order. When one of these operations is invoked on an XML document, an event occurs therein which is stored in an event class of the same name.
\end{example}

In addition to the event types already provided by AXS new {\em interaction event types} are specified.
Where the event types already provided by AXS comprise operation events, mutation (primitive and composite) events, and calendar events (see Subsection~\ref{section:event-types-and-classes}). The new interaction event types are defined as specialization of the abstract event type. When an interaction is performed, being either one on TDFs (see previous Subsection~\ref{section:basic-interaction}) or on ATDFs (see following Subsection~\ref{section:active-interactions}), an according event occurs which is stored in an event class.

In AXS an event class of an XML document can be subscribed by remote XML documents which replicate the event class. Events that subsequently occur in the subscribed document are delivered to the subscribing documents. This provides for distributed active behavior, allowing a document to react to events that occurred in other documents. By using the publish/subscribe protocol documents are loosely coupled.

Summarized, an active peer is capable 
of detecting events occurred in a version, 
of receiving events from versions of subscribed documents,
of distributing events to versions of subscribing documents,
of executing operations, and 
of executing ECA rules. 
In the following, Subsection~\ref{section:active-interactions} introduces new interactions on active documents and versions, and Subsection~\ref{section:routing-model} presents the realization of the publish/subscribe protocol on top of the P2P model of layer IM-1 and describes the event routing algorithm. 

\subsection{Interactions on Active Documents and Versions}
\label{section:active-interactions}

Three additional interactions are provided by active peers to deal with active behavior defined by AXS.
First, interaction \cmd{invoke} executes an operation on a checked-in current version. Second, interactions \cmd{subscribe} and \cmd{unsubscribe} are used to establish and release subscriptions between documents. The latter two are special in that subscriptions have effects on possibly all versions of a document (depending on the employed event routing model, see Subsection~\ref{section:routing-model} and Subsection~\ref{section:optimized-event-flows}), i.e., when document $d_s$ subscribes document $d_p$, possibly all versions of $d_s$ are notified of events that occur in some version of $d_p$. A document may subscribe itself.

Interactions \cmd{subscribe} and \cmd{unsubscribe} can only be issued against a particular version of the subscribing document, called the event recipient. Thereupon this version notifies a particular version of the publishing document, called the event distributor (see Subsection~\ref{section:routing-model} for these two particular versions). This ensures that data can be exchanged freely between those two versions. Moreover, restricting the versions these interactions can be issued against facilitates control over authentification, authorization, etc. by centralization, which accords to having effects on all current versions.

A peer stores semantic descriptions of interactions on active documents and versions as it stores descriptions of interactions on (passive) documents and versions (see Subsection~\ref{section:basic-interaction}). Each of the above interactions are represented by an according class, namely {\sf tdf:Invoke}, {\sf tdf:Subscribe}, and {\sf tdf:Unsubscribe} which are all subclasses of {\sf tdf:ActiveInteracion $\sqsubseteq$ tdf:Interaction}.
Thus they are described by the properties describing {\sf tdf:Interaction}s (see Subsection~\ref{section:basic-interaction}).
Moreover, the invocation of an operation is described by the name of the invoked operation (property {\sf tdf:ofOperation}), by the passed parameters (property {\sf tdf:withParamValue}), and by the operation's return value (property {\sf tdf:hasReturnValue}).
Interactions subscribe and unsubscribe are described by property {\sf tdf:ofPublishingDocument}.

When an interaction is performed an according event occurs. Every AXS schema defines per default an event type for each interaction from Subsection~\ref{section:basic-interaction}, be it simple or composite, except for operation invocations, and for interactions \cmd{subscribe} and \cmd{unsubscribe}. Event classes storing events of those types can be materialized on demand, they must be named after the invoked interactions their events represent, e.g., {\sf CheckIn} or {\sf Merge}.
%
For operation invocations an event type is defined for every single operation specified by the AXS schema (and not for the \cmd{invoke} interaction). 
%
An event representing an interaction is stored in an event class of the version it was targeted at.
Interested documents can subscribe these event classes to be informed of interactions.

\begin{example}
Because the procurement department wants to be alerted when a department has orders above average or when the overall budget is used up, it creates document $d_{alert}$ and an initial version. This document subscribes event classes of document $d_{order}$ that reflect executions of operations \op{addItem} and \op{removeItem}. Thus, if any current version of $d_{order}$ is modified, the initial version of $d_{alert}$ is notified of the occurred event. By aggregating data of such events alerting situations can be detected.
\end{example}

It is possible to embed interactions on documents and versions in operations and rules defined by AXS. Thus interactions cannot only be performed by users but also by versions, enabling them to automatically perform an interaction in reaction to occurred events.

\begin{example}
Upon copying $v_2$ to $l^*_{distr}$, which creates $v^*_1$ of newly created document $d^*_{order}$ at $l^*_{distr}$, the purchaser's document $d_{order}$ subscribes the supplier's document $d^*_{order}$ to be informed of the order's acceptance, shipment, and billing, which are represented by invocations of operations \op{accept}, \op{reject}, \op{ship}, and \op{bill}.
\end{example} 



==> event-flows/event-flow-optimize.tex <==
\section{Optimization}
\label{section:ATDF.optimization}

The model for document flows in Section~\ref{section:document-flow} as well as the model for event flows in Subsection~\ref{section:routing-model} assume high availability of peers, however, this assumption restricts peers in their autonomy. Moreover, low coupling of peers is gained at the cost of network traffic, since events can only be forwarded to directly preceding or following versions, resulting in unnecessary event forwarding.
This section presents an optimized model that overcomes these two properties. First, it provides for higher autonomy of peers by waiving the expectation of high availability, and second, it provides for event flows that are in need of less network traffic by avoiding unnecessary event forwarding.

Both improvements of the optimized model are gained by having {\em version graph indices} available locally at each peer. Thereby each peer does not only know a version's direct predecessors and successors but also indirect ones. Version graph indices are maintained by employing active behavior provided by layer IM-1 and the basis of IM-2 so that the infrastructure model presented so far does not have to be adapted. How version graph indices are maintained is presented in detail in Subsection~\ref{section:MaintainingVGIs}.

The improvement of {\em higher autonomy} is gained by by-passing offline peers.
By by-passing them in the sending and receiving phase of event forwarding a peer can be offline without blocking event flows.
By by-passing offline peers during manual version discovery, a peer can be offline without preventing people from determining an online version's (indirectly) following versions, e.g., when one wants to determine current versions by querying a frozen version she knows of.

The improvement of {\em reduced network} traffic is gained by by-passing peers that have no responsibilities regarding event distribution of a certain document.
Having a version graph available locally at each peer, it is possible to forward an event not only to a directly preceding or following version as employed in the basic model for event flows, but to any version. Thereby unnecessary event forwarding can be avoided and network traffic reduced.

How the active extension is employed to realize the optimized model is described in detail in the following two subsections.

\subsection{Maintaining Version-Graph Indices (Layer IM-2.2)}
\label{section:MaintainingVGIs}

This layer, which is situated side-to-side with the basic event routing model in layer IM-2.1 (see Figure~\ref{fig:ATDF.layers}), maintains a {\em version graph index} at each peer for every version the peer stores, which is a local view on the version graph the version is part of.
To be able to construct the version graph index, denoted as $G_{v_i}$, for every version $v_i$ of document $d$ the peer stores, the document subscribes event classes that reflect document flows of itself, i.e., $d$ subscribes $d$.
Thereby each of the document's versions receives an event upon a modification of the version graph. 
Subscription of the set of event classes $E^G:=\{{\sf CheckIn}, {\sf CheckOut}, {\sf Merge}, {\sf Delete}, {\sf Reallocate}\}$ is sufficient to construct $G_{v_i}$.
Note that due to outstanding event deliveries caused by offline peers, version graph $G_{v_i}$ at one peer may differ from version graph $G_{v_j}$ of the same document at another peer. 

A version graph index is defined as a view over the set of event classes $E^G$. Simplified, the view defining query selects the latest event for each version from the {\sf CheckOut} and the {\sf Merge} event class to determine dependencies between versions, the latest from {\sf CheckIn} and {\sf Reallocate} to determine the version's location, and uses {\sf Delete} to filter out deleted versions. As views in databases, a version graph index can be either virtual or materialized. If it is materialized it may be maintained incrementally, depending on the peer's capabilities, meaning that with a newly imported event $e \in E^G$ the view is updated according to $e$ without access to any other event in $E^G$.

\begin{example}
\label{exmp:local-vg-1}
Consider the version graph depicted in Figure~\ref{fig:document-flow} when comprising $v_1$, $v_{1.1.1}$, and $v_2$. Further assume that the document subscribes the set of event classes $E^G$ of itself that reflect document flows.
Version $v_{1.1.1}$ then comprises a checkin event reflecting interaction ``\cmd{checkin $v_1$ of $d$}'',
and a checkin and checkout event reflecting each of the two interactions ``\cmd{branch $v_1$ to $v_{1.1.1}$}'' and ``\cmd{proceed $v_1$ by $v_2$}''. 
Upon performing interaction ``\cmd{branch $v_1$ to $v_{1.2.1}$}'', two according events are imported into and stored in $v_{1.1.1}$. 
From the events in event classes {\sf CheckIn} and {\sf CheckOut} version graph index $G_{v_{1.1.1}}$ can be constructed.
\end{example}

If a peer is not capable of maintaining version graph indices incrementally, frozen versions need special attention.
By definition, these versions are immutable and thus cannot store any event that occurred after the time they became frozen. Such events, however, are necessary to construct $G_{v_i}$ for frozen version $v_i$ if the index is not maintained incrementally.
To resolve this issue, a peer stores such events in so called {\em auxiliary event classes} in addition to the event classes of a frozen version.
By providing an integrated view over these event classes, a version graph index can be transparently specified over them as if all event classes were stored within the version.

\begin{example}
Continuing Example~\ref{exmp:local-vg-1}, when version $v_{1.1.1}$ is merged into $v_2$ next, an according merge event occurs, which is first forwarded to the document's event distributor $v_1$ which is also the event recipient. From there it is delivered to current version $v_2$ and $v_{1.2.1}$. The event also passes frozen versions $v_1$ and $v_{1.1.1}$ where the event is stored as well (possibly in auxiliary event classes).
\end{example}

Summarized, the optimized model for document flows provides higher autonomy for peers with respect to their availability. The model offers the advantage of having a version graph index available at each peer where a version of the document is allocated at. This allows to query a version arbitrarily about its version graph an not only about directly preceding and directly following versions. 
The model, however, inherently provides version graph indices only for versions that (indirectly) follow the event recipient. Thus one can only benefit from this layer when looking for related versions that (indirectly) follow the event recipient.
Note that this layer assumes that the event routing layer IM-2.1 guarantees that an imported event (caused by self-subscription) passes every version following the event recipient either during the event distribution or event reception phase.

%@@online path

\subsection{Optimized Event Routing (Layers IM-2.1R/RL)}
\label{section:optimized-event-flows}

This section presents two optimized event routing algorithms provided by layers IM-2.1R and IM-2.1RL which both reduces network traffic and deliver events more robustly (i.e., unaffected by offline peers) compared to basic event routing IM-2.1B presented in Subsection~\ref{section:routing-model}. 
For short we refer to the event routing algorithms as \{B$|$R$|$RL\} event routing.
The layers are intended to supplement IM-2.1B, nevertheless, for a single document a dedicated event routing algorithm has to be chosen.
Optimization builds upon version graph indices and can thus only supplement IM-2.1B if IM-2.2 is deployed (also see Figure~\ref{fig:ATDF.layers}).

R event routing provides {\em \underline{R}obust event delivery} by forwarding imported events from the event recipient directly to all versions (indirectly) following the event recipient using its version graph index. Thus event delivery can no longer be blocked by offline peers. Network traffic in R routing is reduced by forwarding an event occurring in some version immediately to the event distributor, i.e., without using intermediate versions.

RL event routing is equally robust as R routing and moreover results in {\em \underline{L}owest network traffic}. In principal, its event routing is a specialized form of R routing, in that imported events are only delivered to current versions, resulting in the lowest network traffic possible.

The optimized event routing models need to know which version in a version graph index is the event distributor and which one is the event recipient.
Thus in addition to the event classes mentioned in Section~\ref{section:MaintainingVGIs}, a document subscribes event class {\sf Relay} of itself. Then, due to self-subscription, this data is available at every version (indirectly) following the event recipient (and of course the event recipient itself). If the event distributor precedes the event recipient, it has to observe the events it distributes to keep track of possible reallocations or relays affecting the event recipient.

A choice between the event routing models is likely to depend on an application's requirements because they differ in whereto events are delivered. Remember, R event routing delivers events to all versions following the event recipient, while RL only delivers them to current versions to minimize network traffic. If non-current versions are frozen, which is defined by property {\sf tdf:freezeNonCurrentVerions} (see Subsection~\ref{section:basic-model}), it is likely that RL event routing will be employed, since frozen versions are immutable and can neither store events nor trigger rules. Vice versa, if non-current versions are not frozen, it is likely that R event routing will be employed, since events may be of interest at every version, e.g., to keep the versions consistent.

{\em Optimizing the sending phase} in R and RL event routing, events are forwarded directly from the version where they occur to the event distributor instead of using other version as intermediaries (as shown in Figure~\ref{fig:opt-event-flow}). This works well as long as the event distributor is online, however, it may change its status to offline and vice versa. Thus the following two cases have to be dealt with (remember that peers hosting event distributors and recipients should be online most of the time):

\begin{enumerate}
\item Event distributor $v_d$ may be offline. If an event is to be forwarded to $v_d$ from current version $v_c$, the version's peer which tries to forward events buffers them until $v_d$ is back online, except when the event is a \cmd{checkin} event. In the latter case, the event is forwarded to the $v_c$'s directly preceding version, so that some other version ``knows'' about it and buffers it. 
This version is then responsible of forwarding events during the receiving phase to $v_c$ as long as $v_d$ is offline. If the directly preceding version is offline as well, the same action is applied to some other current version. If neither $v_d$ nor any current version is online, the peer of the checked-in version periodically tests whether one of them went online. As soon as this happens, an appropriate action is performed so that the checked-in version becomes part of the version graph and is notified of events. 
If an event is to be forwarded from a non-current version to (offline) $v_d$, it is forwarded to a current version's peer and is buffered there so that it is forwarded to the event distributor later on (see below).

\item If event distributor $v_d$ goes online after being offline, it performs the following steps:
(1) it notifies all peers that host a current version according to the version's (possibly  out-dated) $G_{v_d}$ to receive buffered events therefrom,
(2) if such received events reflect changes to the version graph, e.g., reveal new versions, step 1, i.e., the notification and reception is recursively applied to those versions as well. Thereby $G_{v_d}$ becomes up-to-date and buffered events are harvested from the versions where they occurred. And
(3) harvested events are sent to event recipients of subscribing documents.
\end{enumerate}

\begin{figure}[h]
    \begin{center}
        \includegraphics[scale=1.3]{event-flows/example-opt-ef}
        \caption{Optimized Event Flow using RL Event Routing}
        \label{fig:opt-event-flow}
    \end{center}
\end{figure}

{\em Optimizing the receiving phase}, one has to distinguish between R and RL event routing.
In R event routing, all events are forwarded from event recipient $v_r$ directly to all (indirectly) following versions using $G_{v_r}$ instead of using other versions as intermediaries.
In RL event routing, events that do not reflect modifications to $v_r$'s version graph are forwarded from $v_r$ directly to current versions (as shown in Figure~\ref{fig:opt-event-flow}). 
%
If a version is offline when events are to be forwarded to it, event recipient $v_r$ buffers them until the version is back online.
Again, an event recipient's peer may go offline (although it should not or only rarely), thus the following two cases have to be dealt with.

\begin{enumerate}
\item Event recipient $v_r$ may be offline. If an event is to be forwarded to it from an event distributor, the latter buffers the event until $v_r$ is back online.

\item If event recipient $v_r$ goes online after being offline, it performs the following steps:
(1) it notifies the peers of subscribed documents' event distributors to receive buffered events, 
(2) it updates $G_{v_r}$ on the basis of events that reflect document flows which have been received during step 1 due to self-subscription (if $v_r \neq v_d$), and 
(3) it forwards events directly to (indirectly) following versions (in R routing) or directly to current versions only (in RL routing). In RL routing, events that reflect modifications to $v_r$'s version graph are delivered to all (indirectly) following versions using B or R routing (configured with the document, see below).
\end{enumerate}

If event distributor $v_d$ is offline while event recipient $v_r$ is online and both belong to the same document, $G_{v_r}$ may be outdated and thus events that are received by $v_r$ from subscribed documents are possibly sent to 
(a) versions that are no longer a current version, in which case the receiving version forwards it to its directly following versions, i.e., falls back to B event routing;
(b) versions that have been reallocated, in which case the receiving peer is responsible of forwarding the event to the reallocated version, or 
(c) versions that have been deleted, in which case $v_r$ is notified which sends the event to the (online) preceding version that is closest to the deleted version instead; that version in turn forwards the event to its directly following versions, i.e., falls back to B event routing.

For layer IM-2.2 to maintain version graph indices, events that reflect  modifications to the version graph have to be delivered to every version (indirectly following the event recipient) of the version graph. While this naturally happens when using B or R event routing, this is not the case with RL event routing.
Hence B event routing has to be employed for forwarding events in the sending phase and/or B or R event routing
%\footnote{in the following ``B/R routing'' is short for ``B and/or (B or R) routing''} in the receiving phase {\em in addition} to RL event routing.
Choosing B/R event routing in both phases makes event delivery more robust to offline event distributors and offline event recipients by keeping the version graph indices up to date irrespective of the two versions' online status. Thus a  fall back to B event routing in the receiving phase is less likely to occur. 
We expect B/R routing employed in both phases to result in less network traffic if the peers are more likely to be offline, however, this remains to be proved by experiments. 
Meanwhile it can be stated that it suffices to employ B/R event routing in either the sending or receiving phase.

The event routing chosen to deliver events is specified by configuration with the document. There, property {\sf tdf:useEventRouting} with a value out of \{{\sf B$|$R$|$RL}\} defines the event routing employed. If it is {\sf RL}, the two additional properties 
{\sf tdf:useInSendingPhase} and {\sf tdf:useInReceivingPhase} with a possible values of \{{\sf B$|$R}\} define the according routing algorithms to use in the sending and receiving phase, respectively, of which one must be specified.
%(a) property {\sf tdf:forVGIsUseEventRouting} with a value out of \{{\sf B}, {\sf R}\} defines which event routing shall be used for delivering events reflecting modifications to version graphs in the receiving phase (see above), and 
%(b) property {\sf tdf:forVGIsUsePhase} with a value out of \{{\sf S}, {\sf R}, {\sf SR}\} defines whether events reflecting modifications to version graphs shall be delivered in the sending phase (value {\sf S}, using B routing) and/or receiving phase (value {\sf RS}/{\sf R}, using the event routing defined by {\sf tdf:forVGIsUseEventRouting}).

Summarized, the optimized event routing model for event flows 
automatically makes event delivery more robust and reduce network traffic, while still being manually controllable by \cmd{relay} interactions. The optimized algorithms, however, assume that a document's event recipient and event distributor can exchange data with any (current) version (not an assumption in B event routing). A mixture of the two models, where events are forwarded to the most distant version of those with which data can be exchanged, would not be based on this assumption and may be the most appropriate one in a given setting. Note that such a mixed model does not have to be developed necessarily, but can be partly achieved manually by employing the optimized model and setting event distributors and event recipients accordingly. 



==> event-flows/event-flow.tex <==
% ############################################################
% # 

\subsection{Basic Event Routing (Layer IM-2.1B)}
\label{section:routing-model}

As shown in Figure~\ref{fig:ATDF.layers}, layer IM-2.1B provides for event routing by adding a layer on top of the base of layer of IM-2.

\begin{figure}[h]
    \begin{center}
        \includegraphics[scale=1.5]{event-flows/layers}
        \caption{Architectural Layers of ATDFs}
        \label{fig:ATDF.layers}
    \end{center}
\end{figure}

A document plays multiple publisher and subscriber roles during its lifetime, producing and consuming events. Since a document's current versions may be allocated at changing locations, events have to be routed from publishers to subscribers dynamically. 

A naive event routing algorithm would be to send an event from the version of a document in publisher role where the event occurs to all current versions of all subscribing documents. This would involve determining all target versions (a) either ad-hoc, i.e., by querying the P2P network using some discovery mechanism, (b) to store an index of all target versions with each current version of a document in publisher role, or (c) a mixture of both. While alternative (a) would result in high network traffic, alternative (b) would yield high complexity in maintaining the indices. The deficiency that all alternatives share is that a version is not notified of an event because it is off-line, not reachable due to the P2P overlay network topology or a firewall, or because of an out-dated index structure.

Instead, the presented event routing algorithm tries to find a balance between network traffic and complexity while guaranteeing event delivery to all subscribers. This is achieved by employing a form of centralization as in hybrid P2P systems such as FastTrack\footnote{\url{http://www.fasttrack.nu}} and \cite{Cast02JSAC}. 
Therefor, two central nodes are introduced for each document, namely two distinguished versions, the event distributor and event recipient (see later in this section). It is based on the following two assumptions.
%
First, there exists a network path between at least two distinguished versions of different documents so that data can be exchanged between the two documents via these versions. A network path may be defined explicitly, e.g., by a firewall configuration. 
%Thus a version of one document can use the two versions as intermediaries to exchange data with versions of the second document.
%
Second, data can be exchanged between two directly following versions of the same document.

The initial version of a document in publisher role is called the document's {\em event distributor}. It is responsible of distributing occurred events to event recipients of subscribed documents and thus has to maintain an index on them. 
If the event distributor is followed by other versions and an event occurs therein, the event is forwarded to the event distributor. This is done by forwarding the event to the respective preceding version until the event distributor is reached.
If a preceding version was offline when an event was to be forwarded to it, the peer that tried to forward the event buffered it until the version was back online.
In case of a merged version, which has $n$ preceding versions ($n>1$), a peer decides autonomously on the subset of them to which an event is forwarded (the number of the subset's members is defined by the peer's configuration parameter $\rho$). If $\rho > 1$ events are duplicated and have to be filtered out when the first common version is reached (which performed the branch). 
When an event is forwarded from the version where it occurred towards the event distributor it is said to be in the {\em sending phase}.

\begin{example}
\label{exmp:event-distributor}
After acceptance of the order by the supplier's distribution department, $v^*_{1}$ is proceeded at the storage department by $v^*_2$ as shown in Figure~\ref{fig:eventFlow}. Upon the order's shipment by the storage department, operation \op{ship} is invoked, causing an operation event to occur in $v^*_2$ at $l^*_{store}$, which is forwarded to the event distributor $v^*_1$ at $l^*_{distr}$.
Thereafter, $v^*_{2}$ is proceeded at the accounting department $l^*_{accnt}$ by $v^*_3$ where operation \op{bill} is invoked later on. Again, an operation event occurs which is forwarded via $v^*_2$ at $l^*_{store}$ to the event distributor $v^*_1$ at $l^*_{distr}$.
Both events are distributed to subscribing documents by $v^*_1$ at $l^*_{distr}$.
\end{example}

\begin{figure}[h]
    \begin{center}
        \includegraphics[scale=1.3]{event-flows/example-ef}
        \caption{Exemplary Event Flows}
        \label{fig:eventFlow}
    \end{center}
\end{figure}

The initial version of a document in subscriber role is called the document's {\em event recipient}. It receives events from event distributors of subscribed documents and is responsible of forwarding them to all current versions.
If the event recipient is followed by other versions, received events are forwarded to its successor version and offspring versions. This is recursively applied until all current versions are reached. By forwarding events to the successor version as well as to offspring versions, events are duplicated and have to be filtered out when versions are merged. Duplication by forwarding events to {\em all} following versions is necessary because a version cannot determine whether all its offspring versions are (indirectly) merged into a single version later on.
If a directly following version was offline when an event was to be forwarded to it, the peer that tried to forward the event buffered it until the version was back online. 
When an event is forwarded from the event recipient towards current versions it is said to be in the {\em receiving phase}.

\begin{example}
After shipment the procurement department's current version $v_2$ is proceeded by $v_3$ at the  accounting department $l_{accnt}$, which awaits the supplier's billing before booking and paying. The event representing the invocation of operation \op{bill} at $l^*_{accnt}$ in Example~\ref{exmp:event-distributor} is delivered to event recipient $v_1$ at $l_{proc}$ which forwards it to $v_{1.1.1}$, $v_{1.2.1}$, and $v_2$. The latter version filters out the same event it subsequently receives from $v_{1.1.1}$ and $v_{1.2.1}$. Finally, version $v_2$ forwards the event to $v_3$ at $l_{accnt}$. The event routing is shown in (a) of Figure~\ref{fig:eventFlow}.
\end{example}

% ############################################################
% # 

% \subsection{Controlling Event Flows}
% \label{section:control-event-flow}

Network traffic caused by event routing as described before can be reduced by {\em manually optimizing event flows}.
This is supported by interaction \cmd{relay} (see the Appendix for the interaction's definition). Because \cmd{relay} can modify a document's event distributor and event recipient, active peers provide for querying a version of whether it is the event distributor or event recipient.

First, network traffic can be reduced by {\em relaying event distribution} from $v_{i}$ to $v_{j}$, where the latter becomes the new event distributor.
This makes forwarding events that occur in versions (indirectly) following $v_{j}$ from $v_{j}$ to $v_{i}$ obsolete.
To relay event distribution from $v_{i}$ to $v_j$, every path (cf. Subsection~\ref{section:basic-model}) between every current version and $v_i$ must contain $v_j$. This ensures that events can be routed from current versions where they occur to the event distributor after relaying.

\begin{example}
Relaying event distribution from version $v^*_1$ to $v^*_3$ saves forwarding events occurring at $l^*_{accnt}$ via $l^*_{store}$ to $l^*_{distr}$. Events originating at $l^*_{accnt}$ thus flow directly via $l_{proc}$, $l_{op_1}$, and $l_{op_2}$ to $l_{accnt}$ as shown in (b) of Figure~\ref{fig:eventFlow}.
\end{example}

Second, network traffic can be reduced by {\em relaying event reception} from $v_i$ to $v_j$, where the latter becomes the new event recipient.
This makes forwarding events that occur in subscribed documents from $v_i$ to $v_j$ obsolete, because events are delivered from event distributors directly to $v_j$ instead of $v_i$.
%Initially, event reception can be relayed from the version at the subscribing document's permanent location to a directly following version at a temporary location. Thus events are delivered to the latter instead of the former by event distributors. Consequently, event reception can be relayed between two directly following versions at temporary locations. 
To relay event reception from $v_i$ to $v_j$, a path must exist from $v_j$ to every current version. This ensures that all current versions can be notified of newly occurred events after relaying.

%, meaning that an event distributor delivers events to version $v_{s'}$ allocated at a temporary location $s_{s'}$ instead delivering them to version $v_s$ allocated at permanent location $s_s$ as done originally. This frees $v_s$ from the responsibility to forward events to following version $v_{s'}$. Event reception can be relayed between two temporary locations, too.

\begin{example}
Relaying event reception from version $v_1$ to $v_3$ of document $d_{order}$ makes event distributor $v^*_3$ send occurred events directly to $v_3$, which saves forwarding events from $v_1$ via $v_2$, $v_{1.1.1}$, and $v_{1.2.1}$ to $v_3$ as shown in (c) of Figure~\ref{fig:eventFlow}.
\end{example}

%Finally, network traffic may be reduced by {\em relaying permanent location} of a document to another service. However, such an interaction may be connected to application semantics and has to be used with care. To relay permanent location from $l_i$ to $l_j$, the latter must host a version that acts as event distributor and event recipient of the document.



==> event-flows/implementation.tex <==
\subsection{Implementation}
\label{section:implementation}

We have implemented a proof-of-concept prototype using JXTA as our P2P platform. Regarding identifiers, PIDs are URNs in the {\sf jxta} namespace, DIDs and VIDs are UUIDs expressed as URNs. Thereby the prototype is independent of physical network addresses, i.e., peers and versions can be physically moved on a network without affecting their IDs. The resolution of URNs to network addresses is provided by JXTA. 

The prototype implements the presented two-layered model and routing algorithms. Because, among others, versions are published using so called advertisements, they can be dynamically discovered using JXTA's Peer Discovery Protocol. 
If during event forwarding towards the event distributor no preceding version is online, we implemented a fallback mechanism that dynamically tries to find another online version or the event distributor of the same document and forwards the event thereto. For event forwarding towards current versions a similar mechanism is implemented.

@@Implemented an SMTP-Filter so that e-mail can be used as user interface to active document flows; advantage: non-intrusive, transparent to user; send=checkout, receive=checkin; thereby making documents sent via e-mail traceable and enrich them with active behavior. 

==> event-flows/index.tex <==
The chapter describes the second layer of the two-layered extension to AXS. It provides for traceable document flows that are enriched with active behavior, abbreviated {\em ATDF}, and is also referred to as {\em layer IM-2}.

The chapter is organized as follows.
First, Section~\ref{section:ActiveExtensionForTDFs} describes the enrichment of TDFs with active behavior by employing AXS. Therefore, additional interactions on documents and version are introduced (see Subsection~\ref{section:active-interactions}) and a basic event routing algorithm is presented (see Subsection~\ref{section:routing-model}).
Second, Section~\ref{section:ATDF.optimization} presents event routing algorithms that use local indices of version graphs to optimize event routing.
Finally, Section~\ref{section:atdf.related-work} discusses related work.

\section{Enriching the Infrastructure Model}
\label{section:ActiveExtensionForTDFs}
\input{event-flows/active-extension}

\input{event-flows/event-flow}

\input{event-flows/event-flow-optimize}

\input{event-flows/related} 

==> event-flows/misc.tex <==


\subsection{Locating}

possibilities within the system
(1) local knowledge
(2) global knowledge: partial by registering document at some special (index) peer, which may maintain a log-document that subscribes the new one (i.e., event classes reflecting document flows thereof), so that a version graph of the new document is maintained at the index peer. Otherwise without subscription, at least one VID of one version has to be maintained by the index peer, so that this version can be queried about its knowledge of the version graph it is part of.


\subsection{misc}

@@wastebasket peer, sinnvoll?

pre-conditions of all interactions

motivation: @@an agent is aware of where in the document flow he is situated and which actions have been carried out already via the event history. This is not always the case for workflow systems.

dossier, connecting multiple documents together, when proceeding the dossier version, proceed all component versions as well. etc

@@checkin the metadatafile itself as a document and use it to synchronize annotations! 

==> event-flows/related.tex <==
\section{Related Work}
\label{section:atdf.related-work}

% \cite{Bail02WWW,Bail02CN,Boni02ICDE,Boni01bVLDBJ,Boni01aWWW,Schr01eComo}
% For defining active behavior for XML documents (layer 2) several approaches are available to choose from. Each of the approaches that apply active behavior to XML documents, from which  \cite{Schr01eComo} was chosen for reasons given in Section~\ref{section:introduction}, focusses on different aspects as follows: \cite{Boni01aWWW} presents how to push rules to an active service which is a server that hosts XML documents and executes active behavior, \cite{Boni02ICDE,Boni01bVLDBJ} show how to utilize existing languages such as XQuery to specify active behavior, \cite{Boni01Thesis} provides among others an execution model for such specified active behavior, \cite{Schr01eComo} presents how to define rules with XML schemas and to subscribe other documents to react to events that occur therein, and \cite{Bail02WWW,Bail02CN} propose a language to define active behavior and show how a set of ECA rules can be analyzed and optimized. Note that while \cite{Abite02VLDB} uses the notion of ``active XML'' it is not related to specifying active behavior.

The ATDF approach employs Active XML Schema (AXS) as an approach for active XML on top of the TDF approach. It was chosen because it provides the most comprehensive set of feature that are useful in a distributed environment. For brief disussions of these approaches see Subsection~\ref{section:IS.axs} and Subsection~\ref{section:IR.xmlview-xml}.

Regarding distributed active behavior related approaches focus on different aspects of distribution.
First, \cite{Chak99IEEE,Kris95TOSE} independently propose systems that support distributed event sources which are integrated by a central server. The server is responsible of event composition, condition evaluation, and rule execution.
% both propose a central server that is able to integrate events from various sources, detect composite events and execute rules. While the former is built upon CORBA for integration, the latter
Second, the idea first presented by \cite{Gatz98SIGMOD} to unbundle databases' active behavior into software components is applied to distributed environments by \cite{Cili01ICOP,Cili03CoopIS}. They propose among others distributed services for the tasks that \cite{Chak99IEEE,Kris95TOSE} assign to a central server. 
%Their event routing algorithms, detailed in \cite{Mueh02PhDThesis} differ from ours in that they use content-based addressing, i.e., use a filter on event's content as a subscription specification
% @@Moreover, \cite{Cili01ICOP,Cili03CoopIS} address event heterogeneity by proposing an event ontology
Different from all of these approaches we propose a P2P architecture and focus on issues when the data for which active behavior is defined for is distributed, i.e., dynamically allocated in a network.

% This also distinguishes our event routing algorithm from those presented in \cite{Mueh02PhDThesis} (which is connected to \cite{Cili01ICOP,Cili03CoopIS}) which operate in a broker architecture. When comparing clients with current versions (cf. Section~\ref{section:basic-model}) and brokers with event distributors and recipients (cf. Section~\ref{section:routing-model}), we focus on event routing between clients and brokers, while \cite{Mueh02PhDThesis} focusses on routing between brokers.

% The presented P2P model differs from existing P2P approaches because location is modelled explicitly. Of course, a layer that provides for location transparency could be employed on top of it, however, this does match the models intention which is to enable users to change documents' locations without affecting active behavior.

The presented event routing algorithm is tailored to the application, i.e., it uses version graphs to route events between versions. 
It cannot be compared to other algorithms, e.g., used by Gnutella and FastTrack, because they do not employ the publish/subscribe protocol and thus cannot ensure that messages are received by all recipients.
%A comparison with \cite{Mueh02PhDThesis} (which is employed by \cite{Cili01ICOP,Cili03CoopIS}) is also not possible, because the routing algorithms presented therein operate in an application-independent infrastructure in a broker architecture.
Comparing it to P2P approaches that use the publish/subscribe protocol,
%The presented approach introduces multiple centralized nodes for routing, two for each document, to map the publish/subscribe protocol to a hybrid P2P architecture. 
it is different from \cite{Yang2003CoopIS}, which uses a single centralized event server to handle subscriptions. However, while \cite{Cast02JSAC}'s underlying model uses DHTs and thus cannot be directly compared, it is similar in that it is a hybrid P2P model by using multiple central nodes (there, one for each topic).


==> kurzfassung.tex <==
% -*- TeX:DE -*-

\chapter*{Kurzfassung}
\vspace{-0.4cm}
% ä:Ã¤ ü:Ã¼ ö:Ã¶

Im Web sind zunehmend mehr Daten verfügbar, wobei Schätzungen eine Milliarde Dokumente im Jahr 2002 nennen. Es wird davon ausgegangen, dass die meisten dieser Dokumente im XML Format vorliegen, da zu erwarten ist, dass HTML von XML als Lingua franca des Webs abgelöst wird, z.B. in der Form von XHTML.

Ein verbreitetes {\em Problem} im Entwurf und der Wartung von Websites liegt darin, dass Webseiten sehr oft andere Daten replizieren oder aus anderen Daten abgeleitet werden. Diese anderen Daten, die auch als Basisdaten bezeichnet werden, sind für gewöhnlich nicht Bestandteil der replizierenden oder ableitenden Seite.
Zwei Eigenschaften von Websites zeichnen für dieses Problem verantwortlich. 
Erstens muss sich die Hypertext-Struktur einer Website nicht notwendigerweise mit dem darunterliegenden konzeptuellen Domänenmodell decken. Daher kann es notwendig sein, ein und dasselbe Datenelement auf mehreren Seiten darzustellen.
Zweitens wird der Inhalt vorgenerierter Seiten oft aus Legacy Systemen bezogen, wie relationalen Datenbanken. Webseiten replizieren in diesem Fall Datenelemente von Datenbanken.

Folglich werden Replikas und Ableitungen inkonsistent, wenn sich Basisdaten ändern, die in Webseiten oder relationalen Datenbanken gespeichert sind. Zum {\em Beispiel} zeigt eine vorgenerierte, ein Produkt anbietende Seite nach der Änderung des Preises in der Datenbank dieses zu einem falschen Preis an. %Oder, nachdem ein Diplomarbeitsthema an einen Studierenden vergeben wurde und dies auf der das Thema im Detail beschreibenden Seite geändert wurde, wird das Thema fälschlicherweise noch immer in der Liste der angebotenen Themen angeführt, fehlt in der Liste der bearbeiteten Themen und fehlt im Tätigkeitsbericht der betreuenden Person.

Die Dissertation bietet eine {\em Lösung} an, indem ein kombinierter Ansatz zum Erhalt der Konsistenz jener Webseiten vorgeschlagen wird, die
(i) Daten aus relationalen Datenbanken replizieren, oder
(ii) Daten aus Webseiten replizieren bzw. sich aus ihnen ableiten.
Werden Basisdaten geändert, wird die Änderung sofort zu betroffenen Webseiten weitergeleitet. Dort wird deren Wartung inkrementell vollzogen, indem nur die von der Änderung betroffenen Teile modifiziert werden, anstatt die Seite komplett von neuem zu generieren.

Der vorgeschlagene Ansatz bietet so konsistente und aktuelle Seiten zu jeder Zeit.
Er ist u.a. effizient durch die Anwendung inkrementeller Seiten-Wartungstechniken,
generisch durch den Erhalt der Konsistenz in XML Daten im Allgemeinen und flexibel durch das Reagieren auf Änderungen in Webseiten anderer Unternehmen. 

==> metaschema/approaches.tex <==
\section{Approaches}
\label{section:approaches}

%[shorten] Each of the four approaches that can be used to implement a tailored metaschema has its own idiosyncratic structure which directly affects its ranking regarding the evaluation criteria presented in Section~\ref{section:criteria}. In this section we describe the four approaches as well as rank them regarding the evaluation criteria.

This section describes four approaches to implementing a tailored metaschema and ranks them with respect to the evaluation criteria presented in Section~\ref{section:criteria}. 





==> metaschema/comparison.tex <==
\section{Comparison}
\label{section:comparison}

When comparing the approaches' characteristics summarized in Table~\ref{tab:PSA-Characteristics}, it gets evident that there is a {\em tradeoff} between semantic expressiveness and schema interoperability. 
The Proprietary Schema approach defines new concepts at M2 not defined by XML Schema and thus imposes proprietary schemas at M1, resulting in high expressiveness but low interoperability. 
The Side by Side Approach tries to overcome this by defining a transformation from new concepts to XML Schema concepts at M2 and applying it to proprietary schemas at M1. This increases interoperability, however, at the cost of locality of change. 
The Framework approach goes one step further by expressing new concepts by XML Schema concepts at M1, having positive effects on interoperability and locality of change, but negative effects on expressiveness. 
Finally, the Specialized XML Schema approach directly extends XML Schema with the new concepts at M2. It suffers from the lack of support by existing XML Schema validators and the constraints of the underlying XML Schema.

\begin{table}
\begin{center}
\caption{Characteristics of the Presented Approaches}
\label{tab:PSA-Characteristics}
   \begin{tabular}[h]{p{4cm}p{0.6cm}p{0.6cm}p{0.6cm}p{0.6cm}}
   \parbox[b][2.5cm]{5cm}{Criteria} & 
      \begin{rotate}{65}\parbox[b]{2.5cm}{Proprietary Schema}\end{rotate} & 
      \begin{rotate}{65}\parbox[b]{2.5cm}{Side by Side}\end{rotate} & 
      \begin{rotate}{65}\parbox[b]{2.5cm}{Framework}\end{rotate} & 
      \begin{rotate}{65}\parbox[b]{2.5cm}{Specialized\\XML Schema}\end{rotate}  \\
   \hline \hline
   Semantic expressiveness & high & high & low & med. \\
   Schema interoperability & low & med. & high & high$^{\dagger}$ \\
   Locality of change & high & low & med. & med. \\
   \hline
      \multicolumn{5}{r}{\scriptsize $^{\dagger}$\parbox[t]{7.5cm}{Assuming standard XML validators provide  for a plug-able XML Schema}} \\
   \end{tabular}
\end{center}
\end{table} 

Since there is no single best approach, one has to choose the most appropriate one based on given requirements. In case schemas will change often, locality of change is the primary criterion with the Proprietary Schema approach being favorable. In case instance documents have to be shared with other partners, schema interoperability is the primary criterion with the Proprietary Schema Approach falling behind. In practice it may be beneficial to use a mixed approach (for an example see Section~\ref{section:EmployingAMixedApproachForAXS}).

\section{Related Work}
\label{section:metaschema.related-work}

Examples for approaches employing the {\it Proprietary Schema approach} are RDF %[shorten]\cite{W3C1999RDF} 
and JavaBeans Persistence \cite{Sun02JSR57}. 
The RDF standard defines RDF's tailored metaschema and a syntax of RDF instances as XML by an EBNF grammar. This grammar can be seen as a declarative specification of $\tau_0$. In addition, the RDF Schema (RDFS) standard %[shorten]\cite{W3C2003aRDFS} 
defines a proprietary schema language for RDF. 
Going beyond XML, JavaBeans Persistence provides for serialization of JavaBean objects as XML documents. It realizes $\tau_0$ by a dedicated Java class. Here, the Java language constitutes the tailored metaschema.
%the Java class {\tt java.beans.\-XML\-En\-coder}.

Among approaches following the {\it Side by Side approach} are \cite{Klei2000ECAI,Micro01ADO,OMG2003XMI2,Rahm01VLDBJ}. \cite{Klei2000ECAI} describes transforming OIL \cite{Horr2000} ontologies to XML schemas by textually describing $\tau_1$ that transforms OIL concepts to XML Schema concepts. 
Independent of XML, Microsoft's ADO.NET DataSet \cite{Micro01ADO} implements among others a generic mapping between the relational model (constituting the tailored metaschema) and XML. It allows to read relational data and to write XML data with its XML schema and vice versa, thus implementing $\tau_0$, $\tau_1$, and their inverse.
The Side by Side approach has been also extensively explored in \cite{Rahm01VLDBJ} recently, yielding an abstract algebra for model mapping \cite{Bern00SIGMOD} (the notion of ``model'' in \cite{Bern00SIGMOD} corresponds to ``schema'' in our approach).
OMG's XMI \cite{OMG2003XMI2} is distantly related, because it does not exactly fit the side-by-side approach's structure. However, it has in common that XMI defines a schema transformation, but of metaschemas (i.e., instance of MOF \cite{MOF02}) into XML Schemas. Thus the transformation takes place at M2 instead of M1 and the transformation function, which could be named $\tau_2$, is defined at M3. The intention of XMI is for example to transform the UML metamodel into an XML Schema, and UML models into XML documents. Aligning XMI's intention with the side-by-side approach, the resulting XML document of the former could be seen as the proprietary schema of the latter.

%, only one layer higher (M3,M2,M1), so when transformed one layer down it corresponds to the sbs-approach?

The {\it Framework approach} has not been employed in the XML field yet. We suspect that a major reason for not employing it is that frameworks usually evolve from simple XML schemas instead of being created from scratch by implementing a tailored metaschema.
%...More often simply the mechanisms provided by XML Schema and application needs foster framework development such as XHTML Modularization \cite{W3C2002bXHTMLMod}. 
Going beyond XML, an example of fostering the Framework approach is UML with its extension mechanisms \cite{Rumb99aUML}. Thus, instead of extending the UML metaschema at M2 (called metamodel in UML), the extension mechanisms provide a means to customize UML at M1. Extension mechanisms are the main concepts to build reusable frameworks, called profiles in UML. Another example of providing a new semantic concept at M1 is the role pattern \cite{Baeu97CACM,Kapp98Mod}. For example, it has been implemented in Smalltalk in terms of a predefined framework \cite{Gott96TOIS}.

The {\it Specialized XML Schema approach}, as the Framework approach, has not been employed in the XML field yet. A major reason could be not wanting to lose interoperability.
%
However, tailoring metaschemas is well known in the non-XML literature. So-called open data models have been proposed in the past (e.g., \cite{Klas95,Mano93}), which consist of a few built-in concepts but which can be extended by additional modeling concepts at M2 for specific application needs.



==> metaschema/criteria.tex <==
\section{Evaluation Criteria}
\label{section:criteria}

This section presents criteria to determine the quality of the different approaches.
These quality criteria, which we have identified to be relevant in the narrow context of implementing tailored metaschemas, are related to quality factors proposed in literature \cite{Boeh76,ISO9126}
%[shorten] ,McCa80
to facilitate a better understanding of their implications. This is only done informally since it is not the focus of this chapter.

{\it Semantic expressiveness} describes how much semantics is expressed formally and concisely by a schema. Since semantics is defined by the tailored metaschema, a schema expressed therein is most expressive. When using XML Schema instead, semantics of the tailored metaschema need to be mapped to XML Schema. Because usually not all semantics can be mapped, schemas expressed in XML Schema are less expressive. 
The more semantics is explicit in a schema, the better the schema can be verified against an explicit metaschema such that errors can be detected at design time. Semantic expressiveness influences quality factors such as understandability, maintainability, testability, and reusability.

{\it Schema interoperability} in general describes the ability of a system to exchange schemas with other systems and interpret them. Interoperability also affects design time of a system in that it allows to reuse schema components from interoperable schemas and to reuse software components implemented for interoperable schemas and metaschemas. In the case of AXS, schema interoperability describes the ability of standard XML software to process schemas that have been created following each of the presented approaches. Thus it directly affects the extent of reusing standard XML software when writing applications that process such schemas. This criteria influences quality factors such as interoperability, flexibility, and portability.

{\it Locality of change} describes the self-containedness of a schema such that a change in one schema component does not require subsequent changes in dependent schema components in the same or other schemas. It is negatively affected by redundantly modelled schema components (i.e., components that model the same circumstance by different concepts) and non-atomic schema components (i.e., a circumstance is modelled by several dependent components). Locality of change is influenced by two aspects: First by the schema's environment (i.e., the employed metaschema and its imposed usage), and second, by the design of a given schema. Because the second aspect is application specific and thus independent of the presented approaches, we focus on the first aspect. Locality of change influences quality factors such as understandability, maintainability, and integrity. 

==> metaschema/framework-approach.tex <==
\subsection{Framework Approach}
\label{section:FrameworkApproach}

This approach uses only an XML schema that expresses all circumstances formerly modelled by the proprietary schema as shown on the left of Figure~\ref{fig:framework-approach}. Thus it eliminates the need for proprietary schema {\sf s}, transformation $\tau_1$, and synchronization of {\sf s} with {\sf s'}.

%[shorten] Given the previous approaches' drawbacks, i.e., either having no XML schema or needing to keep two schemas synchronized, an approach would be preferable that uses only an XML schema that expresses all circumstances formerly modelled by the proprietary schema. This is provided by the Framework approach, eliminating the need for proprietary schema {\sf s} and schema transformation $\tau_1$ including the synchronization of {\sf s} with {\sf s'}.

\begin{figure}[h]
    \begin{center}
      \includegraphics[scale=1.3]{metaschema/framewor}
      \caption{Framework Approach}
      \label{fig:framework-approach}
    \end{center}
\end{figure}

Since intensional aspects are orthogonal to XML Schema, they can be expressed easily using XML Schema extension mechanisms (annotations and foreign attributes). Expressing extensional aspects is more complicated as they must be expressed solely with concepts provided by XML Schema.

%When expressing all circumstances solely by an XML schema, intensional and extensional aspects have to be treated differently. Intensional aspects, which are {\it orthogonal} to XML Schema, can be expressed easily by using XML Schema extension mechanisms, namely annotations and foreign attributes. 
%Expressing extensional aspects is more complicated as they cannot be expressed with concepts from a tailored metaschema must be expressed solely with concepts provided by XML Schema. Furthermore, in order to facilitate code reuse across applications, XML schema designers must follow well-defined conventions when expressing extensional aspects.

The framework concept as known from object-oriented programming \cite{John97CACM} can help in this situation. A framework is a means to provide a base schema common to all applications, along with conventions for its adaption and usage in the design of particular schemas. 
XML Schema provides a set of concepts that can be employed in framework design, such as abstract types, type derivation, abstract elements, and substitution groups (see \cite{Mali02aIBM} for a brief overview). 
Therefore an XML Schema framework comprises a set of reusable and/or specializable elements and types, which form the base schema, and a set of informal conventions describing their reuse and specialization.

\begin{example}
\label{example:framework}
The Active XML Schema framework below defines the structure of event classes which are represented by {\sf actf:eventClass} elements that are of abstract type {\sf actf:TEventClass}. Moreover, abstract type {\sf actf:TEventType} describes events, which comprise an identifier (attribute {\sf id}), occurrence time (element {\sf occurrenceTime}), and status (attribute {\sf status}). 
%
Type {\sf actf:TEventType} is directly or indirectly extended by specialized event types which are provided by the framework for all kinds of events (e.g., {\sf actf:TOperationEvtTp} for operation events and {\sf actf:TImportedEvtTp} for imported events). 
%
Finally, in addition to event types, reusable event classes are provided by the framework (e.g., {\sf actf:TEvtCs\_ImportedEvtTp} is a special event class having {\sf event} elements of type {\sf actf:TImportedEvtTp}, a specialized {\sf actf:TEventType}).

  {\sf \footnotesize
  \begin{tabbing}
  \quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \kill
  \rule{\textwidth-1pc}{0.2mm} \\
  {\itshape (M1) XML Schema framework with target namespace actf:} \\
  {\tt 01}\>\>$<$!{\tt --} \textit{Abstract base event type and class} {\tt --}$>$ \\
  {\tt 02}\>\>$<$xs:element name=``\textbf{eventClass}'' type=``actf:TEventClass"/$>$ \\
  {\tt 03}\>\>$<$xs:complexType name=``\textbf{TEventClass}'' abstract=``true"/$>$ \\
  {\tt 04}\>\>$<$xs:complexType name=``\textbf{TEventType}'' abstract=``true"$>$ \\
  {\tt 05}\>\>\>$<$xs:sequence$>$ \\
  {\tt 06}\>\>\>\>$<$xs:element name=``occurrenceTime" type=``actf:TTimestamp"/$>$ \\
  {\tt 07}\>\>\>$<$/xs:sequence$>$ \\
  {\tt 08}\>\>\>$<$xs:attribute name=``id" type=``xs:ID" ../$>$ \\
  {\tt 09}\>\>\>$<$xs:attribute name=``status" type=``actf:TEvtStatus" ..$>$ \\
  {\tt 10}\>\>$<$/xs:complexType$>$ \\  
  %
  {\tt 11}\>\>$<$!{\tt --} \textit{Event type and class for operation events} {\tt --}$>$ \\
  {\tt 12}\>\>$<$xs:complexType name=``\textbf{TOperationEvtTp}" abstract=``true"$>$ .. \\
  {\tt 13}\>\>\>$<$xs:extension base=``actf:TEventType"$>$$<$xs:sequence$>$ \\
  {\tt 14}\>\>\>\>$<$xs:element name=``return" nillable=``true"$>$ .. $<$/xs:element$>$ \\
  {\tt 15}\>\>\>\>$<$xs:element name=``diff" nillable=``true" minOccurs=``0"$>$ .. $<$/xs:element$>$ \\
  {\tt 16}\>\>\>$<$/xs:sequence$>$$<$/xs:extension$>$ .. \\
  {\tt 17}\>\>$<$/xs:complexType$>$ \\
  {\tt 18}\>\>$<$xs:complexType name=``\textbf{TEvtCs\_OperationEvtTp}''$>$ .. \\
  {\tt 19}\>\>\>$<$xs:extension base=``actf:TEventClass"$>$$<$xs:sequence$>$ \\
  {\tt 20}\>\>\>\>$<$xs:element name=``\textbf{event}'' type=``actf:TOperationEvtTp" ../$>$ \\
  {\tt 21}\>\>\>$<$/xs:sequence$>$$<$/xs:extension$>$ .. \\
  {\tt 22}\>\>$<$/xs:complexType$>$ \\
  %
  {\tt 23}\>\>$<$!{\tt --} \textit{Event type and class for imported events} {\tt --}$>$ \\
  {\tt 24}\>\>$<$xs:complexType name=``\textbf{TImportedEvtTp}'' abstract=``true"$>$ .. \\
  {\tt 25}\>\>\>$<$xs:extension base=``actf:TEventType"$><$xs:sequence$>$ \\
  {\tt 26}\>\>\>\>$<$xs:element name=``\textbf{remoteEvent}" type=``actf:TEventType"/$>$ \\
  {\tt 27}\>\>\>$<$/xs:sequence$>$ .. $<$/xs:extension$>$ .. \\
  {\tt 28}\>\>$<$/xs:complexType$>$ \\
  {\tt 29}\>\>$<$xs:complexType name=``\textbf{TEvtCs\_ImportedEvtTp}''$>$ .. \\
  {\tt 30}\>\>\>$<$xs:extension base=``actf:TEventClass"$>$$<$xs:sequence$>$ \\
  {\tt 31}\>\>\>\>$<$xs:element name=``\textbf{event}" type=``actf:TImportedEvtTp" ../$>$ \\
  {\tt 32}\>\>\>$<$/xs:sequence$>$$<$/xs:extension$>$ .. \\
  {\tt 33}\>\>$<$/xs:complexType$>$ \\
  \rule{\textwidth-1pc}{0.2mm}
  \end{tabbing}} 
 
\end{example}

%[martin] Developing an XML schema based on a framework involves specialization of abstract types, useage of predefined types and elements, provisioning of default values for attributes, etc. ... The mechanisms upon which the framework is built provide rules on how application schemas must be designed, e.g., abstract types must be specialized, abstract elements can only be substituted by elements of substitutable type, etc.

To some extent, conventions defining the reuse and specialization of schema components provided by an XML Schema framework can be enforced by mechanisms of XML Schema. 
For example, an abstract type must be specialized before it can be used, or an abstract substitution group's head has to be substituted by an element of an appropriate type. 
Unfortunately, in many cases these mechanisms are not  sufficient to enforce a correct usage of the framework. Therefore, schema designers must know and follow informal conventions regarding the use of framework components.

\begin{example}
Modelling the exemplary schema based on the XML framework requires the definition of the following (as shown below).
First, event type {\sf j:TExecAnnounceEvtTp\_Imported} is defined for imported events, which is done by extending event type {\sf actf:TImportedEvtTp}. Since element {\sf actf:remoteEvent} cannot be refined by the exemplary schema because it is not in the framework's namespace, an annotation is provided that indicates that elements representing remote events shall be of type {\sf j:TExecAnnounceEvtTp} in instance documents.
%
Second, a corresponding event class (element {\sf j:jobSite.announce}) is defined by making it part of the substitution group headed by {\sf actf:eventClass}. 
The type of the event class's {\sf actf:event} elements is defined in an annotation as {\sf j:TExecAnnounceEvtTp\_Imported}, due to the same reasons as with the event type for imported events.
Proxy {\sf u:jobSite}, which is an intensional aspect, is defined within an annotation. 
%
Note that the use of the annotation as well as the definition of parallel type hierarchies comprising event types and event classes are informal conventions, i.e., not enforceable by the XML Schema framework.

\noindent
\parbox{1cm}{
  {\sf \footnotesize
  \begin{tabbing}
  \quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \kill
  \rule{\textwidth-1pc}{0.2mm} \\
  {\itshape (M1) Exemplary XML schema with target namespace u:} \\
  {\tt 01}\>\>$<$!{\tt --} \textit{Imported event type} {\tt --}$>$ \\
  {\tt 02}\>\>$<$xs:complexType name=``\textbf{TExecAnnounceEvtTp\_Imported}''$>$ .. \\
  {\tt 03}\>\>\>$<$xs:extension base=``actf:TImportedEvtTp"$>$ \\
  {\tt 04}\>\>\>\>$<$xs:annotation$>$$<$xs:appinfo$>$ \\ 
  {\tt 05}\>\>\>\>\>$<$actm:remoteEvtTp=``j:TExecAnnounceEvtTp''/$>$ .. \\
  {\tt 06}\>\>\>\>$</$xs:annotation$>$$<$/xs:appinfo$>$ \\ 
  {\tt 07}\>\>\>$<$/xs:extension$>$ .. \\
  {\tt 08}\>\>$<$/xs:complexType$>$ \\
  {\tt 09}\>\>$<$!{\tt --} \textit{Imported event class} {\tt--}$>$ \\
  {\tt 10}\>\>$<$xs:element name=``\textbf{jobSite.announce}" \\
  {\tt }\>\>\>\>type=``actf:TEvtCs\_ImportedEvtTp" substitutionGroup=``actf:eventClass"$>$ \\
  {\tt 11}\>\>\>$<$xs:annotation$>$$<$xs:appinfo$>$ \\ 
  {\tt 12}\>\>\>\>$<$actm:proxy name=``jobSite'' forDocType=``j:JobAnnounce'' type=``single''$/>$ \\
  {\tt 13}\>\>\>\>$<$actm:hasMemberType=``u:TExecAnnounceEvtTp\_Imported''/$>$ .. \\
  {\tt 14}\>\>\>$<$/xs:appinfo$>$$<$/xs:annotation$>$ .. \\
  {\tt 15}\>\>$<$/xs:element$>$ \\
  \rule{\textwidth-1pc}{0.2mm}
  \end{tabbing}}
}
\end{example}

Regarding the characteristics of the framework approach, most notably is the lack of {\it semantic expressiveness} of extensional aspects. This is exemplified by comparing the import of an event class by the proprietary schema shown in Example~\ref{example:prop-extensional-aspects} with the above schema. Furthermore, informal conventions that must be followed when using a framework severely impact semantic expressiveness.
%Moreover, processing an XML schema that uses a framework requires tracing element types back to framework types in order to determine their semantics, therefore implementing such software is a difficult task.
%
On the positive side, {\it schema interoperability} is high since schemas (and frameworks) are expressed solely in XML Schema. 
%[shorten] Thus standard XML software can be used to process schemas. In particular, a high schema interoperability opens the possibility to reuse schema design tools, a feature certainly needed when using XML Schema frameworks. 
%[martin] Thus the framework provides extensible and reusable components that can also be used by others.
%
{\it Locality of change} is medium since the framework may impose modifications of multiple schema components in order to achieve the modification of a single circumstance.
%while a schema transformation $\tau_1$ is not necessary, 
%Due to the informal conventions, {\it verifiability} is medium. Intensional aspects and ... can be verified / enforced, though.

%==$>$ generell: extensionale aspekte mit hohem impedance mismatch sind im framework-ansatz schwer zu behandeln

%??? framework nicht immer ohne $\tau_1$ möglich ??? e.g. TOperationEvent: spez. muss op-signatur entsprechen... - geht, wenn diese in XSD definiert ist - was sie sein müsste, weil sie ja einen extensionalen aspekt hat !! $<$-- spricht das für die schema integratability? oder geht das genauso beim prop-schema (sofern es XML ist...) 

==> metaschema/implementing-dexa.tex <==
The chapter discusses the realization of the metaschema of the Active XML Schema (AXS) approach, which was presented in Chapter~\ref{chapter:ActiveXMLSchema}.
%
As described in Section~\ref{section:activeExtensionOfXMLSchema}, %in order to enrich XML with event driven, active behavior, 
AXS defines active behavior within XML schemas along metadata, and stores traces of active behavior such as occurred events within XML documents along data.
The semantic expressiveness of XML Schema, the schema language recommended by the W3C, however, is not sufficient to define the active semantics of Active XML Schema concepts. 
The contribution of this chapter is to identify, explore, and evaluate approaches to implementing AXS with XML Schema, discussing the trade-off between semantic expressiveness and interoperability. 
Assuming that AXS may be seen as representative for tailored schema languages, the findings of this chapter can be applied for arbitrary tailored schema languages.

The chapter is organized as follows. After giving a brief overview of the problem in Section~\ref{section:activexmlintro}, Section~\ref{section:criteria} defines criteria by which the approaches are evaluated, which are presented in Section~\ref{section:approaches}. Subsequently, the four approaches are ranked according to the criteria. Section~\ref{section:comparison} summarizes the approaches by directly comparing them to each other.
For a better understanding of the presented approaches, 
Section~\ref{section:metaschema.related-work} discusses examples from theory and practice. 
Finally, Section~\ref{section:EmployingAMixedApproachForAXS} gives an in-depth example of applying a mixed approach for realizing AXS.

\input{metaschema/introduction}

\input{metaschema/criteria}

\input{metaschema/approaches}
\input{metaschema/propschema-approach}
\input{metaschema/sidebyside-approach}
\input{metaschema/framework-approach}
\input{metaschema/specxmlschema-approach}

\input{metaschema/comparison}

\input{metaschema/realizingaxs}




==> metaschema/introduction.tex <==
\section{Introduction}
\label{section:activexmlintro}

Tailored schema languages define domain concepts thus semantics once and for all across schemas. In relational databases for example, the schema language defines concepts such as tables and foreign keys, constituting modelling primitives for database schemas. 
Applications exhibiting event driven, active behavior are another example where the use of a dedicated schema language is favorable. Such a tailored schema language defines the semantics of active concepts such as event-condition-action (ECA) rules and event types independent of individual application schemas.

As the usage of XML increases, the need for tailored XML schema languages, which go beyond the semantic expressiveness of XML Schema, arises.
%[shorten] \cite{W3C2001XMLSchema1,W3C2001XMLSchema2}, arises. 
This goes in parallel with the emerging practice to define an XML syntax both for schemas and instances (e.g., as RDF does). %[shorten] \cite{W3C1999RDF,W3C2003aRDFS} does).

For instance, the Active XML Schema (AXS) approach provides an XML syntax both for schemas and instances. Its schema language\footnote{For the purpose of readability, we use the term metaschema instead of schema language throughout the rest of the chapter. If we talk about a schema expressed in XML Schema, we concisely call it XML schema.} allows to define circumstances having {\it intensional aspects} and/or {\it extensional aspects}. While the former refers to circumstances that only affect a schema, such as ECA rules, the latter refers to circumstances that only affect instances of a schema, such as the structure of occurred events.

Using XML for schemas and instances instead of using other data formats is beneficial with respect to {\it interoperability}, {\it openness}, and {\it integration}. This means that schemas and instances described with XML syntax are accessible under various platforms and environments, they can be extended by employing XML namespaces, %[shorten]\cite{W3C1999NS}, 
and they can be integrated with other XML standards such as  XLink, %[shorten]\cite{W3C2001XLink}, 
XSLT,
%[shorten]\cite{W3C1999XSLT}, 
and RDF. 
%[shorten] However, defining XML syntaxes for both schemas and instances is not advantageous at first, since it adds an extra layer of complexity when defining metaschemas that needs to be handled properly.

The contribution of this chapter is to identify, explore, and evaluate approaches to implementing tailored metaschemas with XML Schema. In particular, four approaches with distinct characteristics are presented. They are explored and applied to Active XML Schema, giving insight into their respective implications. Furthermore, the approaches are evaluated with respect to criteria that have been identified to be relevant for the quality of a tailored metaschema's implementation.

Since Active XML Schema comprises concepts that have intensional and extensional aspects, it can be assumed to be a representative for tailored metaschemas. Thus the chapter generalizes statements about Active XML Schema to statements about tailored metaschemas. However, keep in mind that the findings presented in this chapter, except for the approaches and evaluation criteria themselves, are based on experiences in implementing the metaschema of Active XML Schema.

The running example is described in Example~\ref{example:metaschema.jobagency}, which summarizes Examples~\ref{example:axs.job-agency},
\ref{example:axs.ec-announce}, and
\ref{example:axs.import-scenario} from
Chapter~\ref{chapter:ActiveXMLSchema}.

\begin{example}
\label{example:metaschema.jobagency}
A job agency provides an Active XML schema defining active document type {\sf j:JobAnnounce} and a document {\sf academicJobs.xml} having that type, which comprises a list of current job offers. 
%[shorten] (cf. Figure~\ref{fig:exImExportAndRules} which uses an extended UML \cite{Rumb99aUML} notation\footnote{The operation section of classes is tagged by ``{\sf O}'', the newly introduced event class section is tagged by``{\sf E}'', the exported event class section by ``{\sf $\uparrow$}'', the imported event class section by ``{\sf $\downarrow$}'', and the rule section by ``{\sf R}''.}). 
A new job offer is announced by an invocation of operation {\sf announce(j:Job)}, which is defined by the active document type. It adds new job offer {\sf j} at the end of the list. 
%To provide others access to newly announced jobs via an event class, the job agency exports event class {\sf announce}. 
A university's science faculty posts, as a courtesy to its staff and students, relevant job offers supplied by the job agency at its document {\sf science.xml} of active document type {\sf u:Faculty}. The latter imports event class {\sf announce}, using proxy {\sf jobSite} to refer to the document from which the remote event class is imported. The proxy's value is bound in instance {\sf science.xml} to document {\sf academicJobs.xml}. Announced job offers are now locally available within a faculty's page in the form of events contained in the imported event class.
\end{example}

%\begin{figure}[h]
%   \begin{center}
%      \includegraphics[width=5cm]{activexmlintro.eps}
%      \caption{Export and Import of Event Classes and Rules}
%      \label{fig:exImExportAndRules}
%   \end{center}
%\end{figure}

%The metaschema of Active XML Schemas, which comprises the active artifacts presented in this section, is used as the tailored metaschema to analyze the applicability and implications of each of the implementation approaches. It is shown how parts of Example~\ref{example:jobagency} are implemented to highlight idiosyncrasies of each approach. 

==> metaschema/propschema-approach.tex <==
\subsection{Proprietary Schema Approach} 
\label{section:PSA}

This approach expresses schemas directly in terms of the tailored meta\-schema, constituting the most ``natural'' approach with respect to schema design.
As shown on the left of Figure~\ref{fig:proprietary-schema-approach}, schema {\sf s} (an XML document) is created by instantiating tailored meta\-schema {\sf m} (e.g., an XML schema). Instance data in turn is created by proprietarily instantiating schema {\sf s}.

\begin{figure}[h]
    \begin{center}
      \includegraphics[scale=1.3]{metaschema/propschem}
      \caption{Proprietary Schema Approach}
      \label{fig:proprietary-schema-approach}
    \end{center}
\end{figure}

For intensional aspects, i.e., aspects that apply for all instances but have no corresponding materialization at the instance level, it is not necessary to consider an XML syntax for M0.

\begin{example}
\label{exmp:prop1}
  %ECA rules are of intensional nature, t
  The tailored meta\-schema and the exemplary proprietary schema below show how rules are defined and expressed by element {\sf actm:rule}. A rule is identified by its name and is defined upon an event class (attributes {\sf name} and {\sf definedOn}), it comprises a condition and an action (elements {\sf actm:condition} and {\sf actm:action}). Since ECA rules only have intensional aspects, no XML syntax needs to be considered for M0.
%While events may occur during the execution of a rule thus materializing in the instance document, a rule execution itself does not materialize in the instance.

  \begin{minipage}[h]{\textwidth}
  {\sf \footnotesize
  \begin{tabbing}
  \quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \kill
  \rule{\textwidth-1pc}{0.2mm} \\
  {\itshape (M2) Tailored metaschema with target namespace actm:} \\
  {\tt 01}\>\>$<$xs:element name=``\textbf{rule}'' ..$>$ .. \\
  %$<$xs:complexType$>$ \\
  {\tt 02}\>\>\>$<$xs:sequence$>$ \\
  {\tt 03}\>\>\>\>$<$xs:element name=``\textbf{condition}'' ../$>$ \\
  {\tt 04}\>\>\>\>$<$xs:element name=``\textbf{action}'' ../$>$ \\
  {\tt 05}\>\>\>$<$/xs:sequence$>$ \\
  {\tt 06}\>\>\>$<$xs:attribute name=``name'' type=``xs:QName" ../$>$ .. \\
  {\tt 07}\>\>\>$<$xs:attribute name=``definedOn'' type=``xs:QName'' ../$>$ .. \\
  {\tt 08}\>\>$<$/xs:element$>$ \\
  \rule{\textwidth-1pc}{0.1mm} \\
  {\itshape (M1) Exemplary proprietary schema:} \\
  {\tt 09}\>\>$<$\textbf{actm:rule} \textbf{definedOn}=``u:jobSite.announce'' name=``announceJobRule" ..$>$ \\
  {\tt 10}\>\>\>$<$\textbf{actm:condition}$>$..$<$/actm:condition$>$ \\
  {\tt 11}\>\>\>$<$\textbf{actm:action}$>$..$<$/actm:action$>$ \\
  {\tt 12}\>\>$<$/actm:rule$>$ \\
  \rule{\textwidth-1pc}{0.2mm}
  \end{tabbing}}
  \end{minipage}
\end{example}

%Since schema {\sf s} is simply an XML document containing arbitrary markup, instances are always proprietary because naturally no standardized instantiation of a proprietary schema can exist. @@Thus an application that deals with instances cannot employ XML as its internal data model but has to use a proprietary one. To export 

For extensional aspects it is necessary to define so-called {\it instance transformation function} $\tau_0$: $I$$\rightarrow${\it XML}. It defines how a proprietary instance is transformed into an XML document. Moreover an inverse function $\tau_0^{-1}$ must exist to transform an XML document back into a proprietary instance. Note that $\tau_0$ is defined at M2, i.e., independent of a particular schema. Therefore it can be reused across applications.

\begin{example}
\label{example:prop-extensional-aspects}
  The tailored meta\-schema below defines the import of an event class by element {\sf actm:imported\-Event\-Class}. The exemplary proprietary schema imports event class {\sf announce} from a remote document represented by proxy {\sf u:jobSite}. 
Finally, the imported event class and events contained therein materialize at the instance level.
%\footnote{To represent an event class an equally named element is used opposite to \cite{Schr01eComo}, where element {\sf eventClass} was used for presentational purposes.}
  
  {\noindent
  {\sf \footnotesize
  \begin{minipage}[h]{\textwidth}
  \begin{tabbing}
  \quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \kill
  \rule{\textwidth-1pc}{0.2mm} \\
  {\itshape (M2) Tailored metaschema with target namespace actm:} \\
  {\tt 01}\>\>$<$xs:element name=``\textbf{importedEventClass}" ..$>$ \\
  {\tt 02}\>\>\>$<$xs:complexType$>$ \\
  {\tt 03}\>\>\>\>$<$xs:attribute name=``name" type=``xs:QName" ../$>$ \\
  {\tt 04}\>\>\>\>$<$xs:attribute name=``hasMemberType" type=``xs:QName" ../$>$ ..\\
  {\tt 05}\>\>\>\>$<$xs:attribute name=``proxy" type=``xs:QName" ../$>$ \\
  {\tt 06}\>\>\>\>$<$xs:attribute name=``remoteEvtCs" type=``xs:QName'' ../$>$ \\
  {\tt 07}\>\>\>$<$/xs:complexType$>$ \\
  {\tt 08}\>\>$<$/xs:element$>$ \\
  \rule{\textwidth-1pc}{0.1mm} \\
  %
  {\itshape (M1) Exemplary proprietary schema:} \\
  {\tt 09}\>\>$<$\textbf{actm:importedEventClass} name=``jobSite.announce" \\
  {\tt 10}\>\>\>proxy=``u:jobSite'' remoteEvtCs=``j:announce" .. /$>$ \\
  \rule{\textwidth-1pc}{0.1mm} \\
  %
  {\itshape (M0) Exemplary instance:} \\
  {\tt 11}\>\>$<$\textbf{jobSite.announce}$>$ \\
  {\tt 12}\>\>\>$<$\textbf{actf:event} id=``e19" ..$>$ .. \\
  {\tt 13}\>\>\>\>$<$atcf:deliveryTime pt=``2003-03-01T12:14.00.07" ../$>$ \\
  {\tt 14}\>\>\>\>$<$\textbf{actf:remoteEvent} id=``r47'' ..$>$ .. \\
  {\tt 15}\>\>\>\>\>$<$actf:occurrenceTime pt=``2003-03-01T12:13:14.15" ../$>$ \\
  {\tt 16}\>\>\>\>$<$/actf:remoteEvent$>$ \\
  {\tt 17}\>\>\>$<$/actf:event$>$ \\
  {\tt 18}\>\>\>$<$\textbf{actf:event} id=``e20'' ..$>$ .. $<$/event$>$ ..\\
  {\tt 19}\>\>$<$/jobSite.announce$>$\\
  \rule{\textwidth-1pc}{0.2mm}
  \end{tabbing}
  \end{minipage}
  }}

\end{example}

{\it Semantic expressiveness} is high because using a tailored meta\-schema makes all semantics explicit at the schema level. 
%
However, since these schemas are expressed in a proprietary format, {\it schema interoperability} is low because standard XML software cannot interpret the proprietary schema. 
This also affects implementation aspects, since standard XML software cannot be reused to validate instance documents against the proprietary schema. 
%
{\it Locality of change} is high, because the tailored metaschema does not impose redundant or non-atomic schema components. 

==> metaschema/realizingaxs.tex <==
\section{Employing a Mixed Approach for AXS}
\label{section:EmployingAMixedApproachForAXS}

When implementing Active XML Schema we decided to follow a mixed approach, mixing Side by Side and Framework approach. We employed the Side by Side approach to provide maximum semantic expressiveness for human modelers. Extensional aspects of proprietary schemas are transformed to XML schemas adhering to a dedicated framework by an XSLT stylesheet representing $\tau_1$. 
Thus we are fully interoperable and able to reuse standard XML software. 
Employing both approaches in combination minimizes the required transformation functionality that has to be provided by $\tau_1$. 
The mixed approach is shown in Figure~\ref{fig:RealizingActiveXMLSchema}.
Since Active XML schemas are assumed not to change often, low locality of change is not considered a problem.

In the following the different components of AXS's implementation and its use in the context of the chapter's running example are shown. AXS's implementation comprises its tailored metaschema, the {\em Active XML Metaschema} {\sf m}, and its XML Schema framework, the {\em Active XML Framework} {\sf f}. 
The namespace prefixes that are used for them are {\sf actm}\footnote{denoting \url{http://big.tuwien.ac.at/axs/metaschema/1.0}} and {\sf actf}\footnote{denoting \url{http://big.tuwien.ac.at/axs/framework/1.0}} respectively.
The exemplary use of {\sf m} and {\sf f} for representing a rule and the import of an event class are shown by a proprietary schema {\sf s} which is an instance of {\sf m}, and an XML schema {\sf s'} resulting from a transformation of {\sf s} to an instance of {\sf f}.

\begin{figure}[h]
    \begin{center}
      \includegraphics[scale=1.3]{metaschema/realizingaxs}
      \caption{Realizing Active XML Schema using a Mixed Approach}
      \label{fig:RealizingActiveXMLSchema}
    \end{center}
\end{figure}

First, the Active XML Metaschema for rules is shown below, forming a part of metaschema {\sf m}. Here, the metaschema for rules, which is depicted in Figure~\ref{fig:uml-metamodel-rule} as an UML diagram, is expressed as an XML schema.
The tailored metaschema has already been sketched in Example~\ref{exmp:prop1}.
%
A rule comprises a condition and an action, is described by a name and a priority, and is defined on an event class.

\medskip
{\noindent \begin{minipage}[h]{\textwidth}
{\sf \footnotesize
\begin{tabbing}
\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \kill
\rule{\textwidth-1pc}{0.2mm} \\
{\itshape (M2) Active XML Metaschema for rules (with target namespace actm):} \\
$<$xs:element name=``\textbf{rule}"$>$ \\
\>$<$xs:complexType$>$ \\
\>\>$<$xs:sequence$>$ \\
\>\>\>$<$xs:element name=``\textbf{condition}" type=``actm:NativeCode" minOccurs=``0"/$>$ \\
\>\>\>$<$xs:element name=``\textbf{action}" type=``actm:NativeCode"/$>$ \\
\>\>$<$/xs:sequence$>$ \\
\>\>$<$xs:attribute name=``name" type=``xs:QName" use=``required"/$>$ \\
\>\>$<$xs:attribute name=``priority" type=``xs:integer" use=``optional"/$>$ \\
\>\>$<$xs:attribute name=``definedOn" type=``xs:QName" use=``required"/$>$ \\
\>$<$/xs:complexType$>$ \\
$<$/xs:element$>$ \\
\rule{\textwidth-1pc}{0.2mm}
\end{tabbing}}\end{minipage}}
\bigskip

Second, the exemplary use of the above metaschema for defining a rule is shown below, forming a part of proprietary schema {\sf s}.
Again, the schema has already been sketched in Example~\ref{exmp:prop1}. Here, it shows the complete rule introduced in Example~\ref{example:rules} and shown in Figure~\ref{fig:exImExportAndRules}.
All unprefixed elements are in the namespace of the Active XML Metaschema, the condition and action are expressed using XSLT. Imported event class {\sf u:jobSite.announce} on which the rule is defined on, is described later in this section.
The {\sf actm:invokeOperation} element is an XSLT extension element that is used to invoke an operation defined by AXS. 
Bindings {\sf \$evt} represents the event that triggered the rule, 
{\sf \$cond} represents the value resulting from the condition's evaluation, and {\sf \$staticDoc} represents the contents of the ``static'' XML document.

\medskip
{\noindent 
%\begin{minipage}[h]{\textwidth}
{\sf \footnotesize
\begin{tabbing}
\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \kill
\rule{\textwidth-1pc}{0.2mm} \\
{\itshape (M1) Proprietary schema defining rule announceJobRule (with target namespace u):} \\
$<$\textbf{rule} name=``\textbf{announceJobRule}" definedOn=``u:jobSite.announce" \\
\>xmlns=``http://big.tuwien.ac.at/axs/metaschema/1.0''$>$ \\
\>$<$\textbf{condition} lang=``http://www.w3.org/1999/XSL/Transform"$>$ \\
\>\>$<$xsl:value-of select=``\$evt//j:job[j:field=\$staticDoc/u:fieldOfInterest]"/$>$ \\
\>$<$/condition$>$ \\
%http://big.tuwien.ac.at/axs/languages/xslt-1.0-extended
\>$<$\textbf{action} lang=``http://www.w3.org/1999/XSL/Transform"$>$ \\
\>\>$<$invokeOperation name=``postJob"$>$ \\
\>\>\>$<$parameter name=``job"$>$ \\
\>\>\>\>$<$xsl:value-of select=``\$cond"/$>$ \\
\>\>\>$<$/parameter$>$ \\
\>\>$<$/invokeOperation$>$ \\
\>$<$/action$>$ \\
$<$/rule$>$ \\
\rule{\textwidth-1pc}{0.2mm}
\end{tabbing}}
%\end{minipage}}
\bigskip

Third, the Active XML Metaschema for event types is shown below, forming a part of metaschema {\sf m}. 
Here, the metaschema for event types, which is depicted in Figure~\ref{fig:uml-metamodel-evts} and Figure~\ref{fig:uml-metamodel-ixe} as UML diagrams, is expressed as an XML schema.
This part of the tailored metaschema has not been sketched in this chapter yet.

\medskip
{\noindent 
%\begin{minipage}[h]{\textwidth}
{\sf \footnotesize
\begin{tabbing}
\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \kill
\rule{\textwidth-1pc}{0.2mm} \\
{\itshape (M2) Active XML Metaschema for event types (with target namespace actm):} \\
$<$!{\tt --} Base event type {\tt --}$>$ \\
$<$xs:element name=``\textbf{eventType}" type=``actm:EventType"/$>$ \\
$<$xs:complexType name=``\textbf{EventType}" abstract=``true"$>$ \\
\>$<$xs:attribute name=``name" type=``xs:QName" use=``required"/$>$ \\
$<$/xs:complexType$>$ \\
$<$!{\tt --} Operation event type {\tt --}$>$ \\
$<$xs:complexType name=``\textbf{OperationEvtTp}"$>$ \\
\>$<$xs:complexContent$>$ \\
\>\>$<$xs:extension base=``actm:EventType"$>$ \\
\>\>\>$<$xs:sequence$>$ \\
\>\>\>\>$<$xs:element ref=``actm:operationRef"/$>$ \\
\>\>\>$<$/xs:sequence$>$ \\
\>\>\>$<$xs:attribute name=``timeSpec" type=``actm:TmSpec" use=``required"/$>$ \\
\>\>$<$/xs:extension$>$ \\
\>$<$/xs:complexContent$>$ \\
$<$/xs:complexType$>$ \\
$<$!{\tt --} Imported event type {\tt --}$>$ \\
$<$xs:complexType name=``\textbf{ImportedEvtTp}"$>$ \\
\>$<$xs:complexContent$>$ \\
\>\>$<$xs:extension base=``actm:EventType"$>$ \\
\>\>\>$<$xs:attribute name=``remoteEvtTp" type=``xs:QName" use=``required"/$>$ \\
\>\>$<$/xs:extension$>$ \\
\>$<$/xs:complexContent$>$ \\
$<$/xs:complexType$>$ \\
\rule{\textwidth-1pc}{0.2mm}
\end{tabbing}}
%\end{minipage}
}
\bigskip

Fourth, the exemplary use of the above metaschema for defining an operation event type is shown below, forming a part of proprietary schema {\sf s}.
The schema has not been sketched in this chapter yet.
It defines operation event type {\sf j:TExec\-Announce\-Evt\-Tp} for events that are signalled after the execution of operation {\sf announce(j:Job)} of interface {\sf j:JobAnnounce}.

\medskip
{\noindent 
\begin{minipage}[h]{\textwidth}
{\sf \footnotesize
\begin{tabbing}
\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \kill
\rule{\textwidth-1pc}{0.2mm} \\  
{\itshape (M1) Proprietary schema defining event type TExecAnnounceEvtTp} (with target \\ 
\>\>{\itshape namespace j):} \\
$<$\textbf{eventType} name=``\textbf{TExecAnnounceEvtTp}" timeSpec=``after" \\
\>xsi:type=``actm:OperationEvtTp" \\ \>xmlns=``http://big.tuwien.ac.at/axs/metaschema/1.0''$>$ \\
\>$<$operationRef interfaceNm=``j:JobAnnounce" operationNm=``announce"$>$ \\
\>\>$<$parameter type=``j:Job"/$>$ \\
\>$<$/operationRef$>$ \\
$<$/eventType$>$ \\
\rule{\textwidth-1pc}{0.2mm}
\end{tabbing}}
\end{minipage}}
\bigskip

Fifth, the Active XML Metaschema for event classes is shown below, forming a part of metaschema {\sf m}. 
Here, the metaschema for event classes, which is depicted in Figure~\ref{fig:uml-metamodel-evts} and Figure~\ref{fig:uml-metamodel-ixe} as UML diagrams, is expressed as an XML schema.
The tailored metaschema has already been sketched in Example~\ref{example:prop-extensional-aspects}.

\medskip
{\noindent 
%\begin{minipage}[h]{\textwidth}
{\sf \footnotesize
\begin{tabbing}
\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \kill
\rule{\textwidth-1pc}{0.2mm} \\
{\itshape (M2) Active XML Metaschema for event classes (with target namespace actm):} \\
$<$!{\tt --} Base event class {\tt --}$>$ \\
$<$xs:element name=``\textbf{eventClass}" type=``actm:EventClass"/$>$ \\
$<$xs:complexType name=``EventClass"$>$ \\
\>$<$xs:attribute name=``name" type=``xs:QName" use=``required"/$>$ \\
\>$<$xs:attribute name=``exported" type=``xs:boolean" use=``required"/$>$ \\
\>$<$xs:attribute name=``hasMemberType" type=``xs:QName" use=``required"/$>$ \\
$<$/xs:complexType$>$ \\
$<$!{\tt --} Proxy {\tt --}$>$ \\
$<$xs:element name=``\textbf{proxy}"$>$ \\
\>$<$xs:complexType$>$ \\
\>\>$<$xs:attribute name=``name" type=``xs:QName" use=``required"/$>$ \\
\>\>$<$xs:attribute name=``forDocType" type=``xs:Name" use=``required"/$>$ \\
\>\>$<$xs:attribute name=``type" use=``required" type=``actm:ProxyTp"/$>$ \\
\>$<$/xs:complexType$>$ \\
$<$/xs:element$>$ \\
$<$!{\tt --} Imported event class {\tt --}$>$ \\
$<$xs:element name=``\textbf{importedEventClass}" type=``actm:ImportedEvtCs" \\
\>substitutionGroup=``actm:eventClass"/$>$ \\
$<$xs:complexType name=``ImportedEvtCs"$>$ \\
\>$<$xs:complexContent$>$ \\
\>\>$<$xs:extension base=``actm:EventClass"$>$ \\
\>\>\>$<$xs:sequence$>$ \\
\>\>\>\>$<$xs:element name=``filterExpr" type=``actm:NativeCode" \\ \>\>\>\>\>minOccurs=``0" maxOccurs=``1"/$>$ \\
\>\>\>$<$/xs:sequence$>$ \\
\>\>\>$<$xs:attribute name=``proxy" type=``xs:QName" use=``required"/$>$ \\
\>\>\>$<$xs:attribute name=``remoteEvtCs" type=``xs:QName" use=``required"/$>$ \\
\>\>$<$/xs:extension$>$ \\
\>$<$/xs:complexContent$>$ \\
$<$/xs:complexType$>$ \\
\rule{\textwidth-1pc}{0.2mm}
\end{tabbing}}
%\end{minipage}
}
\bigskip

Sixth, the exemplary use of the above metaschema for defining an imported event type and an imported event class is shown below, forming a part of proprietary schema {\sf s}.
The schema has already been sketched in Example~\ref{example:prop-extensional-aspects}.
It defines remote event type {\sf j:TExec\-Announce\-Evt\-Tp\_Imported} for wrapping events of operation event {\sf j:TExecAnnounceEvtTp}. Proxy {\sf u:jobSite} is used in importing remote event class {\sf j:announce} as imported event class {\sf u:jobSite.announce}.

\medskip
{\noindent
\begin{minipage}[h]{\textwidth}
{\sf \footnotesize
\begin{tabbing}
\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \kill
\rule{\textwidth-1pc}{0.2mm} \\
{\itshape (M1) Proprietary schema defining an imported event type and event class (with target} \\
\>\>{\itshape namespace u):} \\
$<$actm:\textbf{eventType} name=``\textbf{TExecAnnounceEvtTp\_Imported}" \\ \>remoteEvtTp=``j:TExecAnnounceEvtTp" xsi:type=``actm:ImportedEvtTp"/$>$ \\
$<$actm:\textbf{proxy} name=``\textbf{jobSite}" forDocType=``j:JobAnnounce" type=``single"/$>$ \\
$<$actm:\textbf{importedEventClass} name=``\textbf{jobSite.announce}" exported=``false" \\
\>proxy=``u:jobSite" remoteEvtCs=``j:announce" \\ \>hasMemberType=``u:TExecAnnounceEvtTp\_Imported"/$>$ \\
\rule{\textwidth-1pc}{0.2mm}
\end{tabbing}}\end{minipage}}
\bigskip

Seventh, the Active XML Framework for event types is shown below, forming a part of framework {\sf f}.
The framework has already been sketched in Example~\ref{example:framework}. Here, the complete definitions of the abstract base event type {\sf actf:TEventType} and the abstract operation event type {\sf actf:TOperationEvtTp} are shown, where the latter is derived from the former.
These types are part of the event type hierarchy at the schema layer (M1) mentioned in Section~\ref{section:event-types-and-classes}.

\medskip
{\noindent
%\begin{minipage}[h]{\textwidth}
{\sf \footnotesize
\begin{tabbing}
\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \kill
\rule{\textwidth-1pc}{0.2mm} \\
{\itshape (M1) Active XML Framework for event types (with target namespace actf):} \\
$<$xs:element name=``\textbf{event}" type=``actf:TEventType"/$>$ \\
$<$xs:complexType name=``\textbf{TEventType}" abstract=``true"$>$ \\
\>$<$xs:sequence$>$ \\
\>\>$<$xs:element name=``occurrenceTime" type=``actf:TTimestamp"/$>$ \\
\>$<$/xs:sequence$>$ \\
\>$<$xs:attribute name=``id" type=``xs:NMTOKEN" use=``required"/$>$ \\
\>$<$xs:attribute name=``status" type=``actf:TEvtStatus" use=``optional"/$>$ \\
$<$/xs:complexType$>$ \\
$<$xs:complexType name=``\textbf{TOperationEvtTp}" abstract=``true"$>$ \\
\>$<$xs:complexContent$>$ \\
\>\>$<$xs:extension base=``actf:TEventType"$>$ \\
\>\>\>$<$xs:sequence$>$ \\
\>\>\>\>$<$xs:element name=``return" nillable=``true"$>$ \\
\>\>\>\>\>$<$xs:complexType mixed=``true"$>$ \\
\>\>\>\>\>\>$<$xs:sequence$>$ \\
\>\>\>\>\>\>\>$<$xs:any namespace=``\#\#any" processContents=``lax"/$>$ \\
\>\>\>\>\>\>$<$/xs:sequence$>$ \\
\>\>\>\>\>$<$/xs:complexType$>$ \\
\>\>\>\>$<$/xs:element$>$ \\
\>\>\>\>$<$xs:element name=``diff" nillable=``true" minOccurs=``0"$>$ \\ 
\>\>\>\>\>$<$xs:complexType mixed=``true"$>$ \\
\>\>\>\>\>\>$<$xs:sequence$>$ \\
\>\>\>\>\>\>\>$<$xs:any namespace=``\#\#any" processContents=``lax"/$>$ \\
\>\>\>\>\>\>$<$/xs:sequence$>$ \\
\>\>\>\>\>$<$/xs:complexType$>$ \\
\>\>\>\>$<$/xs:element$>$ \\
\>\>\>$<$/xs:sequence$>$ \\
\>\>$<$/xs:extension$>$ \\
\>$<$/xs:complexContent$>$ \\
$<$/xs:complexType$>$ \\
\rule{\textwidth-1pc}{0.2mm}
\end{tabbing}}
%\end{minipage}
}
\bigskip

Eighth, XML schema {\sf s'} as the result of transforming the part of proprietary schema {\sf s} that defines an operation event type (cf. fourth), is shown below. It defines how the extensional aspects of events are represented at the instance layer (M0).

\medskip
{\noindent
\begin{minipage}[h]{\textwidth}
{\sf \footnotesize
\begin{tabbing}
\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \kill
\rule{\textwidth-1pc}{0.2mm} \\
{\itshape (M1) XML schema for operation event type TExecAnnounceEvtTp (with target} \\
\>\>{\itshape namespace j):} \\
$<$xs:complexType name=``\textbf{TExecAnnounceEvtTp}"$>$ \\
\>$<$xs:complexContent$>$ \\
\>\>$<$xs:extension base=``\textbf{actf:TOperationEvtTp}"$>$ \\
\>\>\>$<$xs:sequence$>$ \\
\>\>\>\>$<$xs:element name=``job" type=``j:Job"/$>$ \\
\>\>\>$<$/xs:sequence$>$ \\
\>\>$<$/xs:extension$>$ \\
\>$<$/xs:complexContent$>$ \\
$<$/xs:complexType$>$ \\
\rule{\textwidth-1pc}{0.2mm}
\end{tabbing}}\end{minipage}}
\bigskip

Ninth, the Active XML Framework for imported event types and imported event classes is shown below, forming a part of framework {\sf f}.
%
The framework has already been sketched in Example~\ref{example:framework}. Here, the complete definitions of the abstract imported event type {\sf actf:TImportedEvtTp} and abstract imported event class {\sf actf:TEvtCs\_ImportedEvtTp} are shown. As one can see, the event class stores events of the imported event type, i.e., its member type is the imported event type.

\medskip
{\noindent
\begin{minipage}[h]{\textwidth}
{\sf \footnotesize
\begin{tabbing}
\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \kill
\rule{\textwidth-1pc}{0.2mm} \\
{\itshape (M1) Active XML Framework for imported event types and classes (with target} \\
\>\>{\itshape namespace actf):} \\
$<$!{\tt --} Imported event type {\tt --}$>$ \\
$<$xs:complexType name=``\textbf{TImportedEvtTp}" abstract=``true"$>$ \\
\>$<$xs:complexContent$>$ \\
\>\>$<$xs:extension base=``actf:TEventType"$>$ \\
\>\>\>$<$xs:sequence$>$ \\
\>\>\>\>$<$xs:element name=``publicationTime" type=``actf:TTimestamp"/$>$ \\
\>\>\>\>$<$xs:element name=``deliveryTime" type=``actf:TTimestamp"/$>$ \\
\>\>\>\>$<$xs:element name=``\textbf{remoteEvent}" type=``actf:TEventType"/$>$ \\
\>\>\>$<$/xs:sequence$>$ \\
\>\>$<$/xs:extension$>$ \\
\>$<$/xs:complexContent$>$ \\
$<$/xs:complexType$>$ \\
$<$!{\tt --} Imported event class {\tt --}$>$ \\
$<$xs:element name=``\textbf{eventClass}" type=``actf:TEventClass" abstract=``true"/$>$ \\
$<$xs:complexType name=``\textbf{TEvtCs\_ImportedEvtTp}"$>$ \\
\>$<$xs:complexContent$>$ \\
\>\>$<$xs:extension base=``actf:TEventClass"$>$ \\
\>\>\>$<$xs:sequence$>$ \\
\>\>\>\>$<$xs:element name=``event" type=``actf:TImportedEvtTp" minOccurs=``0" \\
\>\>\>\>\>maxOccurs=``unbounded"/$>$ \\
\>\>\>$<$/xs:sequence$>$ \\
\>\>$<$/xs:extension$>$ \\
\>$<$/xs:complexContent$>$ \\
$<$/xs:complexType$>$ \\
\rule{\textwidth-1pc}{0.2mm}
\end{tabbing}}\end{minipage}}
\bigskip

Tenth, XML schema {\sf s'} as the result of transforming the part of proprietary schema {\sf s} that defines an imported event type and imported event class (cf. sixth), is shown below. It defines how the extensional aspects of imported events and imported event classes are represented at the instance layer (M0).

\medskip
{\noindent
\begin{minipage}[h]{\textwidth}
{\sf \footnotesize
\begin{tabbing}
\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \kill
\rule{\textwidth-1pc}{0.2mm} \\
{\itshape (M1) XML schema for an imported event type and class (with target namespace u):} \\
$<$xs:complexType name=``\textbf{TExecAnnounceEvtTp\_Imported}"$>$ \\
\>$<$xs:complexContent$>$ \\
\>\>$<$xs:extension base=``\textbf{actf:TImportedEvtTp}"/$>$ \\
\>$<$/xs:complexContent$>$ \\
$<$/xs:complexType$>$ \\
$<$xs:element name=``\textbf{jobSite.announce}" type=``actf:TEvtCs\_ImportedEvtTp" \\
\>substitutionGroup=``actf:eventClass"/$>$ \\
\rule{\textwidth-1pc}{0.2mm}
\end{tabbing}}\end{minipage}}
\bigskip 

==> metaschema/sidebyside-approach.tex <==
\subsection{Side by Side Approach}

This approach is similar to the Proprietary Schema approach in that it uses an explicit tailored metaschema to define schemas. However, an XML schema is provided in addition, which does not replace the proprietary one but stands side by side to it. Likewise, instance transformation function $\tau_0$ is still used to serialize instances as XML.

The transformation of a proprietary schema into an XML schema is defined at M2 by so-called {\it schema transformation function} $\tau_1$$:$ $S$$\rightarrow${\it XSD} and applied at M1 as depicted on the right of Figure~\ref{fig:side-by-side-approach}. 
Function $\tau_1$ can be derived from $\tau_0$, since the latter defines the structure of XML documents implicitly. While $\tau_0$ is used at runtime, i.e., when documents are processed, $\tau_1$ is used at design time, i.e., when schemas are created. Because only extensional aspects of the proprietary schema are transformed to an XML schema, $\tau_1$ is {\it partial}.

\begin{figure}[h]
    \begin{center}
      \includegraphics[scale=1.3]{metaschema/sidebysi}
      \caption{Side by Side Approach}
      \label{fig:side-by-side-approach}
    \end{center}
\end{figure}

\begin{example}
\label{example:SbSA}
The result of transforming extensional aspects of proprietary schema {\sf s} (cf. Example~\ref{example:prop-extensional-aspects}) to XML schema {\sf s'} by $\tau_1$ is shown below. It defines the imported event class as element {\sf u:jobSite.announce}, which contains a sequence of {\sf u:event} elements, each representing an imported event and in turn containing the wrapped remote event as element {\sf u:remoteEvent}.

  {\sf \footnotesize
  \begin{tabbing}
  \quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \kill
  \rule{\textwidth-1pc}{0.2mm} \\
  {\itshape (M1) Exemplary XML schema with target namespace u:} \\
  {\tt 01}\>\>$<$xs:element name=``\textbf{jobSite.announce}'' actm:eventClass=``jobSite.announce''$>$ \\ 
  {\tt 02}\>\>\>$<$xs:complexType$><$xs:sequence$>$ \\
%  \>\>\>$<$!{\tt --} \textit{the imported event} {\tt --}$>$ \\
  {\tt 03}\>\>\>\>$<$xs:element name=``\textbf{event}" ..$>$ \\
  % actm:artifact=``importedEvent"$>$ \\
  {\tt 04}\>\>\>\>\>$<$xs:complexType$>$$<$xs:sequence$>$ \\
  {\tt 05}\>\>\>\>\>\>$<$xs:element name=``\textbf{remoteEvent}" ..$>$ .. $<$/xs:element$>$ \\
  %\>\>\>\>\>\>actm:artifact=``remoteEvent"$>$ ..\\
  {\tt 06}\>\>\>\>\>$<$/xs:sequence$>$$<$/xs:complexType$>$ \\
  {\tt 07}\>\>\>\>\>$<$xs:attribute name=``id" type=``xs:ID'' ../$>$ \\
  {\tt 08}\>\>\>\>\>$<$xs:attribute name=``deliveryTime'' ../$>$ \\
  {\tt 09}\>\>\>\>\>$<$xs:attribute name=``publicationTime'' ../$>$ \\
  {\tt 10}\>\>\>\>\>$<$xs:attribute name=``deliveryTime'' ../$>$ \\
  {\tt 11}\>\>\>\>$<$/xs:element$>$ \\
  {\tt 12}\>\>\>$<$/xs:sequence$>$$<$/xs:complexType$>$ \\
  {\tt 13}\>\>$<$/xs:element$>$ \\
  \rule{\textwidth-1pc}{0.2mm}
  \end{tabbing}} 
\end{example}

Still using a tailored metaschema to model schemas results in high {\it semantic expressiveness}. But in contrast to the Proprietary Schema Approach, this approach provides an XML schema for extensional aspects, resulting in higher {\it schema interoperability}.
Thus standard XML software can be used to validate instance documents at the cost of implementing $\tau_1$ to transform schemas. 
Implementation of applications is supported by providing explicit links from components in {\sf s'} to components in {\sf s} (cf. attribute {\sf actm:eventClass} in Example~\ref{example:SbSA}).
%
Having two schemas expressing the same circumstances redundantly by components in terms of different metaschemas makes it necessary to keep them synchronized. Thus {\it locality of change} is low. 


==> metaschema/specxmlschema-approach.tex <==
\subsection{Specialized XML Schema Approach}

%This approach extends XML Schema with new concepts of the tailored metaschema as shown in Figure~\ref{fig:specialized-schema-approach}. To relate new concepts to XML Schema concepts, mechanisms provided by XML Schema itself are used, which is possible because XML Schema itself is defined by an XML schema, which in turn assumes XML Schema at M3. Thus plenty of possibilities exist to relate concepts, such as element composition and type derivation.

This approach extends XML Schema with new concepts of the tailored metaschema as shown in Figure~\ref{fig:specialized-schema-approach} opposed to the framework approach, which expresses new concepts of the tailored metaschema by XML Schema concepts. 
To relate new concepts to XML Schema concepts the mechanisms provided by XML Schema itself are used, because XML Schema at M2 is defined by an XML schema, (cf. \cite{W3C2001XMLSchema1}), which in turn assumes XML Schema at M3 (as one can see, XML Schema is meta-circularly defined \cite{Maes87OOPSLA}). Thus plenty of possibilities exist to relate concepts, such as element composition, type composition, or type derivation.  Also redefinition as shown in \cite{Prov02aXML.com} is an option. Note, however, while \cite{Prov02aXML.com} focusses on restricting XML Schema, this approach focusses on extending it.

\begin{figure}[h]
    \begin{center}
      \includegraphics[scale=1.3]{metaschema/specxmls}
      \caption{Specialized XML Schema Approach}
      \label{fig:specialized-schema-approach}
    \end{center}
\end{figure}

Depending on whether XML Schema is to be extended by intensional or extensional aspects, different procedures are followed. 
An extension with intensional aspects is simply a matter of adding new concepts to XML Schema without the need to relate them to existing concepts.
On the contrary, extensional aspects {\it must} be defined as specializations of existing concepts such as elements and attributes, in order to inherit the extensional semantics of those concepts.
%[shorten] Note that 
Intensional aspects thus have no standard meaning, i.e., they can be safely ignored by standard XML Schema validators.

This approach has the advantage that an XML Schema validator can interpret specialized XML schemas, because it is possible to 
derive the basic meaning of a schema component of a specialized concept from the XML Schema concept it is based on. Or in different terms, it is possible to 
perform a {\it downcast} according to the principle of type substitutability. Unfortunately, standard XML Schema validators currently do not provide for a plug-able XML Schema necessary for a downcast.
%[shorten], i.e., for a dynamically changeable metaschema, 

\begin{example}
In XML Schema, group {\sf xs:schemaTop} defines the content of element {\sf xs:schema}, the document element of every XML schema. The group defines a choice of elements {\sf xs:element}, {\sf xs:attribute}, and others. 
It is redefined\footnote{The redefinition of {\sf xs:schemaTop} is a group redefinition that contains a reference to itself. Thus, it is semantically equivalent to a derivation by extension, being applied to an element group instead of a complex type.} by the specialized XML Schema to include elements {\sf actm:rule} and {\sf actm:import\-Event\-Class}. 
%
Because a rule has only intensional aspects, element {\sf actm:rule} can be declared by referencing the respective element declaration of the tailored metaschema depicted in Example~\ref{exmp:prop1}. 
%
Because an imported event class has extensional aspects, element {\sf actm:imported\-Event\-Class} is indirectly derived from {\sf xs:topLevelElement} (via {\sf xs:actm.EventSequence}), the type of a global element declaration in XML Schema.
%[false] \footnote{An intermediary dummy type is involved between {\sf actm:TEvent\-Sequence} and {\sf xs:top\-Le\-vel\-Ele\-ment} to solve namespace issues but is left out for presentational reasons.}
The two schema documents with different namespaces shown below form the specialized XML schema.

  {\sf \footnotesize
  \begin{tabbing} 
  \quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \kill
  \rule{\textwidth-1pc}{0.2mm} \\
  {\itshape (M2) Specialized XML Schema with targetNamespace xs:} \\
  {\tt 01}\>\>$<$xs:redefine schemaLocation=``XMLSchema.xsd"$>$ \\
  {\tt 02}\>\>\>$<$xs:group name=``\textbf{schemaTop}''$>$$<$xs:choice$>$ \\
  {\tt 03}\>\>\>\>$<$xs:group ref=``xs:schemaTop"/$>$ \\
  {\tt 04}\>\>\>\>$<$xs:element ref=``\textbf{actm:rule}/$>$ \\
  {\tt 05}\>\>\>\>$<$xs:element ref=``\textbf{actm:importedEventClass}''/$>$ .. \\
  {\tt 06}\>\>\>$<$/xs:choice$>$$<$/xs:group$>$ \\
  {\tt 07}\>\>$<$/xs:redefine$>$ \\
  %
  {\tt 08}\>\>$<$xs:complexType name=``\textbf{actm.EventSequence}''$>$ ..  \\
  %\>$<$xs:complexContent$>$ \\
  {\tt 09}\>\>\>$<$xs:restriction base=``\textbf{xs:topLevelElement}''$>$ .. $<$/xs:restriction$>$ \\
  {\tt 10}\>\>$<$/xs:complexType$>$ \\

  \rule{\textwidth-1pc}{0.1mm} \\
  {\itshape (M2) Specialized XML Schema with targetNamespace actm:}  \\
  {\tt 01}\>\>$<$xs:element name=``\textbf{importedEventClass}''$>$ ..\\
  %\>$<$xs:complexContent$>$ \\
  {\tt 02}\>\>\>$<$xs:extension base=``\textbf{xs:actm.EventSequence}'$>$ .. \\
  {\tt 03}\>\>\>\>$<$xs:attribute name=``proxy" type=``xs:QName" use=``required"/$>$ \\
  {\tt 04}\>\>\>\>$<$xs:attribute name=``remoteEvtCsName" type=``xs:QName" use=``required"/$>$ \\
  {\tt 05}\>\>\>\>$<$xs:attribute name=``exported" type=``xs:boolean" use=``required"/$>$ \\
  {\tt 06}\>\>\>$<$/xs:extension$>$ \\
  {\tt 07}\>\>$<$/xs:element$>$ \\
  \rule{\textwidth-1pc}{0.2mm}
  \end{tabbing}}
\end{example}

On the negative side, the power of a downcast is very limited compared to an explicitly defined schema transformation $\tau_1$. In particular, a specialized concept can not arbitrarily modify extensional semantics of its base concept. For instance, the extensional semantics of a specialized element is always limited to that of exactly one element. 
Therefore it is not possible to define a particular composition of elements by means of one specialized element.

%\begin{example} ... exemplary schema: intensional aspects equal to the proprietary schema from 4.1 whereas extensional aspects essentially looks like the XML schema from 4.2 except that some more readable names (xs:importEventClass instead of xs:element) can be used - but because of the limits of downcast the overall structure of schema components remains the same (therefore mainly presentational effects) \end{example}

Overall {\it semantic expressiveness} is medium, whereby the semantic expressiveness of intensional and extensional aspects differ. It is high for intensional aspects because they are expressed in terms of their unconstrained metaschema. It is medium for extensional aspects, because their metaschema is constrained by the concepts of XML Schema.
%
If standard XML Schema validators provide for a plug-able XML Schema, {\it schema interoperability} will be high since they can interpret specialized XML Schemas. Unfortunately, in practice this is not yet the case causing low interoperability.
%Implementation complexity is low since no schema transformation function needs to be defined and, in theory, standard validators can be reused. The latter can be validated against the specialized XML Schema language, thus {\it verifiability} is high.
%
Concerning {\it locality of change} it is advantageous that only one metaschema is employed. However, one concept of the tailored metaschema is possibly expressed by several concepts of XML Schema, producing several dependent schema components. Therefore locality of change is medium.


==> problem.tex <==
\section{Problem Statement}
\label{section:IM.Problem}

Now having the definition of ``consistency of data on the Web'' at hand, we can break down the problem of maintaining consistency of data on the Web into the following three parts, each one being dealt with in a separate subsection.

\subsection{Consistency between Relational Databases and the Web}
\label{section:IM.Problem.1}

When pre-generating Web pages from relational databases, it has to be decided on how to model Web pages, how to model the database, and how to map between the two, having far-reaching consequences.
First, the expressivity of the models and the mapping determines the kind of Web pages that can be modelled. Moreover, the models determine the kind of mappings that can be designed.
Second, the kind of mapping determines the maintainability of a Web site in terms of the amount of manual action that needs to be performed upon a modification in the database to adjust the mapping.
Third, the models and the mapping determine possible consistency techniques, varying in their update granularity and kind of consistency they can provide.
%
All of these aspects in pre-generating Web pages and their consequences are discussed in the following.

The {\em database} can be modelled either {\em instance-based} or {\em class-based}. This addresses the possibility to modularly design the chunks of data that represent the content of Web pages. A simple approach will allow to define such chunks individually only, i.e., being instance-based. An approach should employ a class-based technique, generating the corresponding instances automatically. This will reduce the complexity of underlying database queries and simplify mapping knowledge and its maintenance in terms of easily determining ``dirty'' pages, i.e., pages that contain out-dated content.

Also {\em Web pages} can be modelled either {\em instance-based} or {\em class-based}. Instance-based refers to modelling every single page by its own, while class-based refers to modelling only classes of Web pages. A class of Web pages (short a ``page class'') comprises a set of pages that share the same structural, navigational, and presentational features, just like the extent of a class in an object-oriented database collects objects of the same kind.
An approach should support class-based models, because they again simplify mapping knowledge and its maintenance. In addition, an approach may also support instance-based models, however, this is less important.

Possibilities to define the {\em mapping knowledge} between the database and Web pages can be distinguished along two dimensions.
First, the mapping may be {\em implicit}, e.g., defined within database queries for determining the content of a page, or {\em explicit}, e.g., in the form of metadata. Explicit mapping knowledge facilitates the maintenance of and reasoning about it.
Second, following the models for databases and Web pages, mappings may be {\em instance-based}, mapping database instances to Web pages, or {\em class-based}, mapping database classes to page classes. Class-based mappings result in the least amount of mapping knowledge, minimized design and maintenance costs, and lowest coupling between the database and Web pages.

%Naturally, when pages are pre-generated, the issue of efficiently keeping their content synchronized with the database arises. 

The maintained {\em consistency} between Web pages and database content can be {\em weak} or {\em strong}.
Under weak consistency Web pages may contain out-dated content, while strong consistency ensures up-to-date content on Web pages.
Weak consistency is usually solved by periodically polling for database updates and carrying out re-generation of affected pages in case of detected updates. If an implicit mapping knowledge is used it is likely that only weak consistency can be maintained (e.g., as in \cite{Yago00VLDB}). Maintenance of weak consistency is also said to be ``pull-based''.
%
Strong consistency mechanisms ensure immediate updates of Web pages upon a database modification. The mechanism usually exploits explicit mapping knowledge to determine the pages that need to be modified. Strong consistency is usually ``push-based'', pushing database modifications to dirty pages.
%
If only one kind of consistency is supported by an approach, strong consistency is obviously more important.
%
With either consistency, special attention needs to be drawn to update all affected pages upon a single database modification and that those changes become visible to users at once, so that the Web pages are consistent among themselves. This is also referred to as {\em multiple view consistency} in the literature \cite{Zhuge1997ICDE}.

Web pages can be modified to be up-to-date with different {\em update granularities}.
%
First, a dirty page can be re-generated from scratch by ``pulling'' the page's content from the database and generating a new page replacing the dirty one. This involves execution of many unnecessary queries and maintenance by {\em completely} re-generating Web pages that contain for their largest part unchanged content, resulting in high maintenance costs.
Second, a dirty Web page can be modified {\em incrementally} by only updating the ``dirty'' part of it. This is likely to reduce maintenance cost, because no unnecessary data needs to be read from the database.

Summarizing, the {\bf problem} in maintaining consistency between relational databases and the Web lies in (i) designing the languages for modelling relational databases and Web pages, so that (ii) a mapping that is easy to maintain can be designed, i.e., an explicit and class-based mapping, which (iii) allows to design a mechanism that at least provides for strong consistency with incremental update granularity.

% ############################################################

\subsection{Consistency within Data on the Web}
\label{section:intro.problem.axs}

%Sharing content is the key success factor of the Web, recently facilitated by XML \cite{W3C1998XML}, which supports among others the exchange of information between e-business partners. XML standards and frameworks for e-business, such as ebXML cite{ebXML03a} or BizTalk \cite{BizTalk} further foster the exchange by providing for interoperability.

Data on the Web can be {\em change-dependent} on other data in different organizational settings.
The base data, i.e., the data depended on may 
reside within the same Web page, or on other Web pages
% (then being referred to as ``remote data'') 
within the same business or on Web pages of another business. 
If base data does not reside within the same Web page, it is referred to as ``remote data''.
If other businesses are involved, they may be cooperating, i.e., agreeing and supporting replication or derivation of data, or not cooperating, being neutral or hostile to others replicating or deriving data from theirs. 
Intuitively, the organizational setting that is to be supported by an approach influences its technical realization. The thesis' focus is on base data within the same business or in cooperating businesses, while also allowing the integration of data from hostile businesses.

Various {\em examples} for change-dependencies in different organizational settings come to mind.
Within the same business, an employee's data, e.g., his/her phone number or job title is often replicated on several Web pages.
Across businesses, a travel agency selling trips that use a certain accommodation may want to raise the price of the trips if the price for an overnight stay in that accommodation rises.
Or, an author or reader of a book may be interested when a review is added at Amazon, a university department may want to publish job offers at its Web site provided by a job agency that could be interesting to its students, or a citation index like CiteSeer\footnote{\url{http://citeseer.nj.nec.com}} may want to derive its citations directly from publication announcements made at universities' Web sites.
An example for a possibly hostile derivation is Geizhals\footnote{\url{http://www.geizhals.at}}, a service that collects and compares offers of different businesses for the same product.

{\em Reasons} for change dependencies are manifold. Technically, the intent is 
to adapt data according to remote data,
to have data replicated or derived from remote data available in a new context, or 
to combine and/or compare remote data locally.
%
More concrete, it can be used for example 
to add value by presenting remote data in a new context, like publishing relevant job offers at a department's Web site;
to provide a preview of linked content or an annotated link;
to provide a navigation context in order not to get lost in hyperspace;
to promote remote data by presenting it on several pages; and finally
to add value by combining and/or comparing remote data, e.g., comparing products.

To achieve consistency, storing data in a relational database and using approaches for maintaining consistency between the database and Web pages is often not a viable option.
This would only be viable in the organizational setting of a single business, and even there it may not be easy to negotiate and run a shared database.
Moreover, there exists content for which it is not reasonable to store it in a database. For such Web-only content, i.e., content in Web pages that is not drawn from underlying databases, a light-weight Web-based solution to Web content management would be a better alternative. This should not replace but complement database functionality.

Additional kinds of change dependencies exist to the ones on data in other Web pages.
First, data may be {\em change-dependent on time}. An approach should support for adapting Web pages to points and periods in time, e.g., for automatic adding of up-to-date content or removing out-dated content. For example, an announced job offer on a department's Web site is to be removed after the application deadline is over.
%
Second, data may also be {\em change-dependent on data in legacy systems} such as relational databases or workflow systems. This resembles the functionality of data-intensive Web sites as far as data in relational databases is concerned. Nevertheless, a uniform interface to maintain consistency to arbitrary legacy systems is desirable.
%
And third, data may be {\em change-dependent on a Web page's history}, i.e., on previous states of a page. For example, a department publishes jobs announced by a job agency, which may announce a job multiple times, only if the department has not published the job before.

%@Interoperability between different applications used by different e-business partners for maintaining content can be reached by defining an XML layer on top of those applications. Thereby content residing for example in databases or workflow systems can be easily exchanged with partners. 

Based on the above considerations and the properties of the Web, four desired characteristics can be derived that an approach for maintaining consistency of data on the Web should feature.
First, change dependencies between Web pages are usually characterized by autonomous control over participating pages, since they often belong to autonomous businesses. Thus, businesses being involved in replication or derivation of data must not be constrained in their {\em autonomy} in how they store and manipulate pages in any way.
%
Second, ideally there exists {\em low coupling} between the systems that maintain consistency, so that one business is not (vitally) affected by actions another business undertakes, such as adding/removing a Web page or going offline for some period.
%
Third, the possibility to {\em integrate legacy systems} in a uniform way should be supported to adapt Web pages according to, e.g., data residing in relational databases or workflow systems.
%
Fourth, the approach should be {\em general} so that it can be applied to manage data in any of the three design dimensions of content, hypertext, and presentation. %Since data in any of the dimensions is XML data this should not be hard to achieve.

Summarizing, the {\bf problem} in maintaining consistency within data on the Web lies in designing an approach supporting change dependencies on data in Web pages, on data in legacy systems, on time, and on Web pages'  histories.  
It should 
(i) preserve businesses' autonomy in managing their Web site, 
(ii) result in a low coupling between systems holding dependent data, 
(iii) provide a uniform interface to legacy systems, and 
(iv) maintain consistency in all design dimensions of Web pages, namely content, hypertext, and presentation.
As with consistency between relational databases and the Web, such an approach should provide at least for strong consistency with incremental update granularity.

\subsection{Consistency in Document Flows on the Web}
\label{section:intro.problem.dataflow}

This subsection uses an extended notion of data on the Web, as described at the end of Subsection~\ref{section:IM.DataOtW}.
Thus, when talking of an approach herein that shall maintain consistency of data on the Web, it is referred to data in the refined sense.
%an extended approach is meant that enriches the original approach addressed so far which maintains consistency of data in the original sense.

Web pages often change their location, i.e., their URL over time, a property of Web pages not considered in this thesis yet. 
An approach providing for consistency of data on the Web, however, should consider this property, which is supported by the following observations.
First, every person who is using the Web regularly will admit that she is often confronted with ``404 Not Found'' or similar due to links to pages whose locations have been modified.
Second, there are prominent calls to refrain from modifying URLs of Web pages or at least to handle them properly \cite{Bern98W3C,W3C2003TAG1}.
Third, URI schemes have been proposed to hide changing locations of pages by providing for location-independent identifiers that can be translated to location-dependent identifiers (for an overview see \cite{W3C2001URI-Clarif,Werf1999a}). Examples are URNs \cite{IETF1997URN} and DOIs \cite{doi.org}.

Looking at XML documents in general instead of Web pages, it can be observed that in certain situations XML documents also change their location over time.
Thereby they form {\em physical} document flows between nodes in the network, being externally observable.
This is different from many systems that seem to support such flows, which, however, in fact only provide for {\em virtual} document flows. They allocate documents permanently at a central repository and provide access from varying nodes, e.g., a workflow engine usually stores workflow data in a central repository, causing the workflow data to flow only virtually between nodes, i.e., clerks' desks.
Contrarily, on the Web there is a physical document flow where documents are moved physically from node to node. 
%To be able to refer to XML data that is physically moved it may have an explicit identifier, in which case the data is generally referred to as a document.
%A dataflow comprising documents is referred to as {\em document flow} throughout the thesis, being either a physical document flow or a virtual document flow. 
%Naturally, only physical document flows need to be dealt with by an extended approach, since 
Note that documents participating in virtual document flows do not change their location and that consistency management is thus already covered by dealing with the problems in the previous two subsections.

Today, physical document flows take place via the Web in business transactions and personal ad-hoc data exchange.
First, rather recently, in the area of Web services, approaches such as BPEL \cite{Bpel2004v11} and ebXML \cite{ebXML03a} provide for the specification of business transactions between businesses.
In the realm of a business transaction XML documents such as a purchase order and an invoice are exchanged.
%While the approaches do not consider documents but only services as first-class objects, thus supporting only dataflows, they can easily be extended to support document flows. Dealing with documents and thus being able to maintain consistency between them can prove useful as shown in the running example in Section~\ref{section:active-TDFs}.
% Following the paradigm of procedural programming, this led to the discussion known as the SOAP vs. REST \cite{Field2000Diss} debate (e.g., cf. \cite{Pres2002XML.com}).
%@XML's interoperable syntax fosters the exchange of (e.g., purchase order) documents between applications within and across businesses which lead to standards such as ebXML cite{ebXML03a}, BPEL \cite{Bpel2004v11}, and SOAP \cite{W3C2003SOAP}.
%
Second, since the advent of the Web, ad-hoc data exchange between individuals has become a daily routine. 
%Unfortunately, there are a lot of situations where documents are exchanged without preserving any metadata except for the document's file name.  
The data exchange is carried out by handing over documents in situations where people want to exchange documents but cannot rely on the same information infrastructure, e.g., because they are working for different businesses. Instead, they use emails with attachments, instant messaging, or filesharing applications such as FTP.

Physical document flows have the following {\em advantages} over virtual document flows:
First, they provide for {\em lower coupling} because participants do not rely on a central repository which is a possible central point of failure and which is usually difficult to provide when documents flow across business' boundaries.
% or b) service types offered by others.
Second, they provide for {\em higher mobility} in manipulating documents going hand in hand with emerging mobile computing devices, assuming that the functionality otherwise provided by the central repository, such as active behavior and versioning, is available locally at each involved node of the document flow.
Third, they provide for {\em higher autonomy} by allowing to implement security aspects such as authentification and authorization locally where documents are stored.
%or b) leaving open which action to perform upon receipt of a document (as opposed to service invocation).
Fourth, lower coupling and higher autonomy result in {\em higher flexibility} in whether and how a document flow takes place, thus providing among others for spontaneous ad-hoc document flows.

A peer-to-peer (P2P) infrastructure is a pre-requisite for supporting physical document flows. Thus an approach for physical document flows has the {\em disadvantages} connected to P2P infrastructures, which are the following. 
Above all, global properties are hard to guarantee in P2P systems, such as global availability of shared data and globally constrained access to data according to security policies. 
It is also difficult to maintain a globally consistent state in P2P systems, a topic distributed consistency protocols are aiming at.
Therefore, a P2P system is usually more complex to design and implement and has to deal with several challenges connected with P2P systems, such as maintaining network control, guaranteeing network security, and avoiding freeloaders (see \cite{Scho2003CACM}).
Thus, if the extended approach is not the approach of choice in a given setting, one may switch to virtual document flows instead. However, if physical document flows are to be used, a P2P infrastructure cannot be circumvented.

An approach that maintains consistency of data on the Web should be capable of maintaining consistency of data participating in document flows.
As such it should provide consistency {\em across and agnostic to document flows}, where ``across'' addresses consistency between documents of which at least one participates in a document flow, and ``agnostic'' means that it should be possible to access a document transparently of whether it participates in a document flow or not, referred to as {\em document flow transparency}.
Examples are consistency between Web pages irrespective of changes to the page's URLs and consistency between XML documents irrespective of their participation in document flows.
%Moreover, an approach should provide for consistency {\em within} a document flow. This assumes that a document leaves traces when participating in a document flow, in the sense that nodes store the latest version of the document stored on them. Then it may be desired to maintain consistency among a document's versions.

%?? example of a computer hardware retailer, has prices in his advertising brochures, and a note that the daily prices may differ. 

Summarizing, the {\bf problem} in maintaining consistency in document flows on the Web lies in designing a P2P infrastructure that preserves the properties of the original approach for providing autonomy, low coupling, and strong consistency with incremental update granularity in spite of the extension. Additionally, the extended approach must provide access to documents transparently of whether they participate in document flows or not. 

==> smwp/smwp_benchmark.tex <==
This subsection presents a benchmark comparing the SWMP approach with triggered pull-based maintenance (cf., e.g., \cite{Sind98WebDB}). The benchmark description is preceded by a brief description of the SMWP prototype.

\subsection{Overview of the SMWP Prototype}

We implemented a prototype of the SMWP approach on top of Oracle9i DBS for storing and maintaining data in fragment classes as well as metadata describing frag-mentation schemas and page schemas. The prototype provides a generic framework in that it can be used with arbitrary relations, fragmentation schemas, and page schemas. Currently pages are stored in the file system, however the modular architecture allows to change the page storage system, e.g., using an XML database. Generated pages can be viewed with an arbitrary Web-browser that is capable of formatting XML documents by the means of CSS \cite{W3C1998CSS2} or XSLT \cite{W3C1999XSLT}. Processing XML is carried out by Java, which is loaded into and executed inside the DBS, and based solely on SAX \cite{Meggi00aXMLDev} in order to minimize memory needs, which lead to performance problems when using DOM \cite{W3C2004DOM3Core} in an earlier prototype. Employed tools are Oracle's XDK \cite{OracleXDK} (its XML parser and XSQL) and Apache's Xalan \cite{ApacheXalan}, which is used for serializing documents from SAX event streams, because to the best of our knowledge XDK does not support this functionality. A modular architecture allows to change the employed XML tools to more efficient ones as they become available. The prototype is available on the Web\footnote{at \url{http://www.dke.jku.at/smwp/}} for download.

Pages of a page class $P$$<$$K$$>$ are pre-generated as follows: By reading the page content schema (e.g., Figure~7 in \cite{Schr02aIS}) the foundation fragment class $F$$<$$K$$>$ as well as the other mapped fragment classes are determined. For each fragment $f$$<$$k$$>$ of the foundation fragment class a page p<k> is generated. The content of a page is generated by read-ing the fragments through SQL queries and transforming the queries' results into an XML document (e.g., see Figure 10 for a sample document) according to the Page Content DTD (see Figure~9 in \cite{Schr02aIS}). 

Active behavior for maintaining fragment classes and page classes as described by the algorithms in Subsection~\ref{IncrementalDD} is implemented using PL/SQL database triggers which propagate a modification of a fragment class to dependent fragment classes and affected page classes. An incremental modification of a page that is affected by a fragment modification is carried out by a SAX filter. The affected page is parsed by a SAX parser, which generates events for each recognized XML element. The filter listens to the event stream and passes events to Xalan's SAX Serializer \cite{ApacheXalan}, which constructs an XML document from its incoming event stream. If an event concerns an element that is to be modified, the filter modifies the event before passing it on. The original page is replaced with the newly constructed one after parsing, thus reflecting the fragment modification.

For benchmarking the triggered pull-based approach, we extended the prototype by a simple mechanism that invalidates ``dirty'' web pages by inspecting modifications on relations.

\subsection{Benchmark Architecture}

The benchmark setting consisted of 28 fragment classes, 10 page classes (each com-prising up to 7 fragment classes), and 19,600 pages with page sizes between 2kB and 500kB. The Oracle database operates on an Ultra-60 machine (UltraSPARC-II 360MHz processor, 512MB of RAM) running Solaris 7. 

The architecture of our benchmark is depicted in Figure~\ref{fig:smwp.benchmark-architecture}. A modification of a relation in the database (i.e., inserting, updating, or deleting a tuple) causes corresponding modifications of affected pages. We benchmarked three approaches for maintaining pre-generated web pages (cf. \cite{Schr02aIS}, Section~4.3):

\begin{enumerate}
\item[(1)] Pre-generation of web pages, using for maintenance
    \begin{enumerate}
    \item[a)] incremental push-based data delivery via fragments (``core SMWP'')
    \item[b)] a mixed approach in which triggers initiate complete re-generation of ``dirty'' web pages by pulling data from fragments (referred to as ``triggered pull of fragments'')
    \end{enumerate}

\item[(2)] triggered pull-based data delivery with complete regeneration of ``dirty'' web pages from base relations like \cite{Chal00INFOCOM}, \cite{Labr00SIGMOD}, and \cite{Sind98WebDB}. We have chosen to benchmark this approach with respect to SMWP, represented by options (1) a) and b). We did not benchmark the ``on the fly generation'' approach mentioned in \cite{Schr02aIS} (Section~4.3), because its running time equals that one of the triggered pull-based approach. Both approaches differ only in whether page generation is triggered by a modification of a fragment or by a user's request respectively.
\end{enumerate}
 
\begin{figure}
    \begin{center}
        %Figure 23
        \includegraphics[scale=1.2]{smwp/benchmark_architecture}
        \caption{Benchmark Architecture}
        \label{fig:smwp.benchmark-architecture}
    \end{center}
\end{figure}

For comparing the running time of the different page maintenance approaches we are interested mainly in maintenance time $t_m$\footnote{An additional lower index put in brackets is used to distinguish between different maintenance approaches: ``push'' for incremental push-based, ``mix'' for mixed, and ``pull'' for triggered pull-based maintenance, e.g. $t_{m(pull)}$ or $t_{m(mixed)}$.}, which denotes the time needed for modifying affected pages once a base relation has been modified. Dependent on the employed maintenance approach, tm comprises the time needed for maintaining fragments (not effective in the case of triggered pull-based maintenance), the time needed for retrieving data from the database (not effective in the case of incremental push-based maintenance), and the time needed to modify affected pages accordingly. As $t_m$ does not include update time of relations, the benchmark times of the triggered pull-based approach basically coincide with the times needed for on the fly generation of a web page. 

\subsection{Benchmark Goal and Expectations}

The goal of the benchmark was to compare the maintenance time of the core SMWP approach against other page maintenance approaches. We expected the core SMWP approach to outperform triggered pull-based maintenance or on the fly generation, as incremental propagation of changes to web pages via fragments does not involve complex queries and complete re-constructions of web pages. This expectation was nourished by Sindoni, who determined page generation to be the main cost factor in his approach, and Yagoub et al. \cite{Yago00VLDB}, who experienced that retrieving web page content from the database takes up to 90\% of the maintenance time.

The rationale behind considering the mixed approach was as follows: On the one hand, queries retrieving web page content are very simple (they just select all tuples from the according fragments) reducing query time compared to the triggered pull-based approach. On the other hand, parsing existing web pages for incremental modification might be more costly than simply re-generating the page from its fragments. 

\subsection{Benchmark Results}

Figure~\ref{fig:smwp.benchmark-maint-time} presents total maintenance times for a single page class with pages of different size . The page content schema of this page class is composed of 7 fragment classes which we experienced to be a typical number of fragment classes according to the common design rule ``seven plus or minus two''.
To achieve representative results, each measurement point depicts the average of the maintenance times of a single page due to repeated changes to a base relation. Similar measurements with other page classes have been undertaken and show similar results: The graph (interpolation line) for incremental push-based maintenance re-mains identical, but the graphs for mixed and triggered pull-based maintenance vary in offset and gradient, although they never meet. Due to these variations, the intersection point of the graphs for incremental push-based and mixed maintenance varies between 5kB and 50kB, while the graphs for the triggered pull-based and the incremental push-based approach never meet.
 
\begin{figure}
        %Figure 24
    \begin{center}
    \includegraphics[width=11cm]{smwp/t_all}
    \caption{Maintenance Time}
    \label{fig:smwp.benchmark-maint-time} 
    \end{center}
\end{figure}

Further measurements have shown that with decreasing database cache hit ratio the graphs for mixed and triggered pull-based maintenance increase in offset and gradient. Also, the intersection point between the graphs of their maintenance times moves, with respect to the graphs in Figure~\ref{fig:smwp.benchmark-maint-time}, towards larger page sizes (such as 250kB) with increased database load.

The benchmark results carried out for a single page class met our expectations. The incremental push-based (core SMWP) approach generally outperformed the other approaches. In the case of large web pages and high database cache hit ratios the mixed approach may be the better choice, because parsing a larger page by SAX can take longer than re-generating the page from fragments.

The advantage of incremental push-based and, also, mixed maintenance over triggered pull-based maintenance increases when more than one page is affected by a modification of a relation, since fragments need to be only modified once. With each additional affected page the graph for triggered pull-based maintenance moves, with respect to the graphs in Figure\ref{fig:smwp.benchmark-maint-time}, further up the y-axis than the graphs of the other approaches do.

A major goal of the SMWP approach was to come up with a declarative design architecture that simplifies the mapping between database entities and web pages and, thus, reduces design and maintenance complexity of pre-generated web pages. The competitive performance further justifies the use of the core SMWP approach. Should a particular application face performance problems with the core SMWP approach, one can flexibly switch to other page generation options as described in \cite{Schr02aIS} (Section~4.3). 

==> smwp/smwp_frag-schema.tex <==
Off-the-shelf relational database technology is used to store fragments and pages as instances of fragment classes and page classes respectively. Because the number of fragments will be typically large with each fragment being relatively small, we do not realize each fragment but all fragments of one fragment class by a single relation. To be able to determine the fragment a tuple is contained in, fragment parameters are stored as part of the tuple. Thus a fragment is read by selecting tuples that have the fragment's parameter values.

It is crucial to determine well-suited techniques for realizing fragment classes. Database {\it views} would be a reasonable option, because primary and derived fragment classes build views over their fragmentation and derivation base classes. Unfortunately, triggers, which would have to be used to incrementally propagate updates on fragments to web pages, cannot be defined on views in major database products (such as Oracle or Microsoft SQL Server). However, some products allow to define triggers on a variation of views, known as {\it materialized views}. But they present another drawback: an incremental update mechanism (i.e., only the affected tuple is updated) for materialized views that join master tables is not provided but only a complete update mechanism (i.e., re-constructing the materialized view from scratch). Again, this prevents from incremental update propagation to web pages.

%[http://download-west.oracle.com/otndoc/oracle9i/901_doc/server.901/a87499/repmview.htm#53762] To be fast refreshed, the defining query for a materialized view must observe certain restrictions. If you require a materialized view whose defining query is more general and cannot observe the restrictions, then the materialized view is complex and cannot be fast refreshed. [..] Specifically, a materialized view is considered complex when the defining query of the materialized view contains: [..] Joins other than those in a subquery; For example, the following statement creates a complex materialized view: CREATE MATERIALIZED VIEW hr.emp_join_dep AS SELECT last_name FROM hr.employees@orc1.world e, hr.departments@orc1.world d WHERE e.department_id = d.department_id;

Therefore we have chosen to realize fragment classes by relations and associated update mechanisms between dependent fragment classes. Fragments $f$$<$$l$$>$ of fragment class $F$$<$$L$$>$ are stored in a single, so called {\it content relation}, named $FC\_F\_L$ after the fragment class it represents. Application relations are the starting point for newly defined fragment classes in that they serve as content relations of fragmentation base classes.
%For clarity of presentation, synonym $FC\_F$ is defined for each application relation $F$ (i.e., root fragment class $F$$<>$).
In order to be able to use uniform prefixes (i.e., ``FC\_'') for names of root fragment classes (which are application relations) and other fragment classes, synonym $FC\_F$ is defined for each application relation $F$ representing root fragment class $F$$<>$.

\begin{example}
Figure~\ref{RelationArchitecture} depicts the realization of the wine shop's fragmentation schema (cf. Figure~\ref{ParameterizedFragmentation}). For the three application relations synonyms {\sf FC\_Wines}, {\sf FC\_Wineries}, and {\sf FC\_Regions} are defined to uniformly treat them like content relations {\sf FC\_Prem\-Wineries\_region}, {\sf FC\_Prem\-Wines\_region}, and {\sf FC\_Regions\_id}, which store the respective fragment class' tuples.
\end{example}

To provide for independence of fragmentation from fragment class' current contents, meta data about fragmentation is stored separately from content relations. For each content relation $FC\_F\_L$ holding tuples of fragments, {\it fragmentation relation} $FR\_F\_L$ stores the domain of parameters $L$. In that way fragments that currently do not comprise any tuples are supported as well. Such a fragment will be listed with its parameter values in $FR\_F\_L$ but will posses no tuples in $FC\_F\_L$.

\begin{example}
Figure~\ref{RelationArchitecture} depicts fragmentation relations {\sf FR\_Prem\-Wineries\_region}, {\sf FR\_Prem\-Wines\_region}, and {\sf FR\_Regions\_id}, which store the respective fragment's parameters. To better motivate the use of fragmentation relations, imagine region {\sf saha} in which no premium wineries are located. If no fragmentation relation had been used, fragments of fragment class {\sf PremWineries$<$region$>$} would have been determined by content relation {\sf FC\_\-PremWineries\_\-region}. Because no premium winery is located in region {\sf saha}, the content relation would not contain tuples having {\sf saha} as the value of attribute {\sf region}. Thus fragment {\sf premWineries$<$saha$>$} and page {\sf premWines$<$saha$>$} would not have existed. On the other hand, by storing the parameter's domain in fragmentation relation {\sf FR\_PremWineries\_region}, a tuple with the value {\sf saha} exists therein independent of content relation {\sf FC\_\-Prem\_\-Wineries}, and thus fragment {\sf premWineries$<$saha$>$} and page {\sf premWines$<$saha$>$} exist. This prevents a user who follows the link from page {\sf region$<$saha$>$} to page class {\sf PremWines$<$region$>$} to experience a HTTP 404 (Not Found) error or similar.
%Page {\sf premWines$<$saha$>$} would not have existed because without fragmentation relations, actual fragmentation would have been determined by means of the primary fragment class, which would not have contained wineries located in that region.
\end{example}

As described in Subsection~\ref{SDLDbDesign}, a parameter is re-usable by defining it on a root fragment class and independent of the fragment class' contents by using a reference relation to store the values of the parameter's domain. An application relation may serve as a reference relation (e.g., see Example~\ref{CreateParameter} and Example~\ref{UseReferenceRelation2}), otherwise a reference relation is created (e.g., see Example~\ref{CreateReferenceRelation}). In either case, the reference relation for parameter $P$ defined upon root fragment class $F$$<>$ is named $RV\_F\_P$ (via a synonym if an application relation is used as a reference relation).

\begin{example}
Figure~\ref{RelationArchitecture} depicts reference relations {\sf RV\_Wineries\_region} and {\sf RV\_Regions\_id}, which store the values of the domains of parameters {\sf region} and {\sf id} (both reference relations being a synonym for application relation {\sf Regions}).
\end{example}

\begin{sidewaysfigure}
    \begin{center}
        \includegraphics[scale=1.3]{\smwpdir figure-3}
        \caption{Realization of a Fragmentation Schema}
        \label{RelationArchitecture}
    \end{center}
\end{sidewaysfigure}

In the following subsections we describe how fragmentation schemas are realized by content, fragmentation, and reference relations in detail.

% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%
% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~

\subsection{Parameters}
\label{RealizingParameters}

Pre-requisite for the definition of a parameter $P$ upon root fragment class $F$$<>$ with content relation $FC\_F(X)$ is that $P$$\in$$X$. If $P$ is the primary key of $FC\_F$, the latter can be used as the parameter's reference relation, which stores the parameter's domain. Otherwise, to achieve independence of parameter $P$'s domain from contents held by $FC\_F$, another application relation can be used as the reference relation, where $P$$\in$$X$ must reference the primary key attribute of this relation.

\begin{example}
   In the definition of parameter {\sf region} upon root fragment class {\sf Wineries$<>$}, application relation {\sf Regions} is used as reference relation (cf.\ Example~\ref{CreateParameter}), because {\sf region} is an attribute of {\sf FC\_Wineries} and attribute {\sf region} references primary key attribute {\sf id} of relation {\sf Regions}. The parameter's domain is defined by primary key attribute values $\pi_{id}(${\sf FC\_Regions}$)$. In order to treat reference relations uniformly, synonym {\sf RV\_Wineries\_region} is defined for relation {\sf Regions}. If analogously to {\sf Prem\-Wineries$<$region$>$} (cf.\ Example~\ref{CreatePrimaryFC}) fragment class {\sf StdWineries$<$region$>$} was defined upon fragmentation base class {\sf Wineries$<>$} using tuple selection predicate {\sf category=``standard''}, the parameter definition of {\sf region} would be re-used.
\end{example}

If no application relation can be used as a reference relation, a reference relation has to be created. Such a reference relation is named $RV\_F\_P$, has schema $P$, and is initialized with current values from the content relation of the root fragment class (i.e., with $\pi_P(FC\_F)$). Furthermore, a foreign key constraint is defined on attribute $P$$\in$$X$, referencing the newly created relation.

\begin{example}
\label{RealizingCreatedReferenceRelation}
   Reference relation {\sf RV\_Regions\_state} would be created for parameter {\sf state}, which was introduced in Example~\ref{CreateReferenceRelation} for illustrative purposes.
\end{example}

% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%
% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~

\subsection{Primary Fragment Classes}
\label{RealizingPrimaryFragmentClasses}

When primary fragment class {\it G$<$KL$>$} is defined upon fragmentation base class {\it F$<$L$>$} a new content relation and a new fragmentation relation are created. They are initialized with tuples from the content and fragmentation relation of the fragmentation base class and with tuples from reference relations.

In the definition of a primary fragment class a fragment selection predicate  $p_F$ and a tuple selection predicate $p_T$ can be used to narrow the set of fragments and tuples therein that are taken over from the fragmentation base class. For accurate presentation we introduce the notion of selection predicate $p$, which is defined as $p$$=$$p_F$$\wedge$$p_T$.

New content relation $FC\_G\_KL(X)$ then stores all fragments of the primary fragment class. It holds tuples from $FC\_F\_L(X)$ for which selection predicate $p$ applies. Its primary key attributes equal the ones of the content relation of the fragmentation base class.

\begin{example}
   Content relation {\sf FC\_Prem\-Wineries\_region} realizes primary fragment class {\sf Prem\-Wineries$<$region$>$} (which is created as shown in Example~\ref{CreatePrimaryFC}). It holds tuples from {\sf FC\_Wineries} for which tuple selection predicate {\sf category=``premium''} applies. A fragment is retrieved by selecting all wineries of a certain region, e.g., fragment {\sf Prem\-Wineries\_rioj} is retrieved by evaluating $\sigma_{region=``rioj"}(${\sf FC\_Prem\-Wineries\_region}$)$. Attribute {\sf id} is the primary key attribute of both of the aforementioned content relations.
\end{example}

New fragmentation relation $FR\_G\_KL(KL)$ stores the domain of the fragment class' parameters $KL$, $dom(KL)$=$dom(K)$$\times$$dom(L)$, and thus defines the fragments. For each parameter value the fragment selection predicate $p_F$ must apply. Because $dom(K)$=$\prod_{i=1}^{|K|}K_i$ is defined by a reference relation $RV\_E\_K_i$ for each parameter $K_i$$\in$$K$ (with primary key attribute $\phi_{RV\_E\_K_i}$\footnote{In the following expression $\phi_R$ is used to denote the primary key attributes of relation $R$.}) and $dom(L)$ is defined by $FR\_F\_L$, data held by $FR\_G\_KL$ is defined by $dom(KL)$=$\{t \in ((\prod_{i=1}^{|K|}\pi_{\phi_{RV\_E\_K_i}}(RV\_E\_K_i)) \times FR\_F\_L) | p_F(t)\}$.

\begin{example}
   Fragmentation relation {\sf FR\_Prem\-Wineries\_region(region)} defines the fragments of {\sf Prem\-Wineries$<$region$>$}. Its data is defined by {\sf RV\_\-Wineries\_\-region} only, because the fragmentation base class is a root fragment class and no parameters other than {\sf region} are introduced. All primary key attribute values from {\sf RV\_\-Wineries\_\-region} are taken over to {\sf FR\_Prem\-Wineries\_region} because no fragment selection predicate is defined.
\end{example}

To ensure data consistency, foreign key constraints are defined on both the content relation, referencing the fragmentation relation, and the fragmentation relation, referencing fragmentation and reference relations it depends on.

% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%
% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~

\subsection{Derived Fragment Classes}

When derived fragment class {\it G$<$KL$>$} is defined upon fragmentation base class {\it F$<$L$>$} and derivation base class {\it H$<$K$>$}, a new content relation and a new fragmentation relation are created. The content relation is initialized with tuples from the content relation of the fragmentation base class, while the fragmentation relation is initialized with tuples from the fragmentation relations of both the fragmentation and derivation base class.

New content relation $FC\_G\_KL(Z)$ stores all fragments of the derived fragment class. It holds tuples from $FC\_F\_L(X)$ that join with tuples from $FC\_H\_K(Y)$, where the join is defined by an equi-join $FC\_F\_L[J_F$=$J_H]FC\_H\_K$. Derived fragmentation is employed whenever fragmentation by properties of attributes $X$ of $FC\_F\_L$ is not possible, i.e., $K$$\cap$$X$=$\emptyset$. To store additional parameters $K$, $FC\_F\_L$'s schema $X$ is extended by $K$, i.e., $Z$=$X$$\cup$$K$. A tuple $t$$\in$$FC\_F\_L$ may qualify for several derived fragments (i.e., it may join with multiple tuples $s$$\in$$FC\_H\_K$). Therefore tuple $t$ from the fragmentation base class results in set $V$ of tuples in the derived fragment class, where $V$=$\pi_Z(t[J_F$=$J_H]FC\_H\_K)$. Consequently the primary key attributes of $FC\_G\_KL$ consist of the primary key attributes of $FC\_F\_L$ extended by $K$.

\begin{example}
   Content relation {\sf FC\_Prem\-Wines\_\-region} of derived fragment class {\sf Prem\-Wines\-$<$region$>$} (which is created as shown in Example~\ref{CreateDerivedFC}) contains tuples from the fragmentation base's content relation {\sf FC\_Wines} that join with the derivation base's content relation {\sf FC\_Prem\-Wineries\_region} on {\sf FC\_Wine[\-producedBy=id]FC\_Prem\-Wineries\-\_region}. The schema of {\sf FC\_Prem\-Wines\_region} comprises attribute {\sf region} additionally to attributes from {\sf FC\_Wines}, its primary key attributes comprise attributes {\sf id} and {\sf region}.
\end{example}

New fragmentation relation $FR\_G\_KL(KL)$ stores the domain of parameter set $KL$, $dom(KL)$=\-$dom(K)$$\times$$\-dom(L)$. Because $dom(L)$ is defined by $FR\_F\_L$ and $dom(K)$ by $FR\_H\_K$, data held by $FR\_G\_KL$ is defined by $dom(KL)$=$\-FR\_F\_L$$\times$\-$FR\_H\_K$.

\begin{example}
   Fragmentation relation {\sf FR\_Prem\-Wines\_region} defines the fragments of {\sf Prem\-Wines\-$<$region$>$}. Its data is defined by {\sf FR\_Prem\-Wineries\_region} only, because the fragmentation base class is not parameterized.
\end{example}

To ensure data consistency, foreign key constraints are defined on both the content relation, referencing the fragmentation relation, and the fragmentation relation, referencing the fragmentation relations of the fragmentation and derivation base.

%First, foreign key constraints are defined on $K$$\in$$FR\_G\_KL$, referencing $FR\_H\_K(K)$, and $L$$\in$$FR\_G\_KL$, referencing $FR\_F\_L(L)$. Second, as for data relations of primary fragment classes, a foreign key is defined on attributes $KL$$\in$$FC\_G\_KL$, referencing $FR\_G\_KL$. This foreign key constraint replaces defined ones on $L$$\in$$FC\_F\_L$ (remember that $K$$\cap$$X=\emptyset$), while foreign key constraints defined on $(X$$\setminus$$L)$$\in$$FC\_F\_L$ are identically defined on $FC\_G\_KL$.

The presented realization of fragment classes is not optimal with respect to disk space because it stores fragment class' contents redundantly. However, unlike main memory, disk capacity is usually not a limiting resource that must be managed wisely \cite{Labr00SIGMOD,Rabi02a}. Nevertheless, optimizations of disk space usage are possible at the expense of processing time. E.g., one possibility is not to store complete tuples in content relations but only their primary key attributes and attributes representing parameters, and to construct fragments by joining such tuples with the appropriate application relation. The employed configuration has to be determined when deploying the SMWP approach, either being optimized with respect to disk space usage or processing time.

% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%
% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~

\subsection{Storing Page Classes}

When page class $P$$<$$K$$>$ is defined upon foundation fragment class {\it F$<$L$>$}, its pages are pre-generated and stored inside the database in attributes of type CLOB. Pages are pre-generated as follows: for each fragment {\it f$<$l$>$} of the foundation fragment class, a page {\it p$<$k$>$} is generated (the mapping between parameter names $l$ and $k$ is specified with the definition of a page class, e.g., see Example~\ref{UseParameterMap}). Furthermore, all fragments that are mapped to a page are read through SQL queries from the content relations of mapped fragment classes and transformed to XML, using a simple generic mapping (cf. \cite{Schr02aIS,Schr01aADC}).

\begin{example}
A page of page class {\sf PremWines$<$region$>$} is pre-generated for each fragment of its foundation fragment class {\sf PremWineries$<$region$>$} and stored inside the database. For each page mapped fragments are read from content relations representing fragment classes. The fragments and tuples contained therein are transformed to XML, forming the page's content. An exemplary tuple contained in fragment {\sf premWineries$<$rioj$>$} is shown below.

\begin{tabbing}
\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \kill
$<$fragment id=``premWineries\&lt;rioj$>$'' ..$>$ \\
\>$<$tuple ..$>$ \\
\>\>$<$attribute name=``id''$>$4$<$/attribute$>$ \\
\>\>$<$attribute name=``name''$>$Finca Allende$<$/attribute$>$ \\
\>\>$<$attribute name=``region''$>$rioj$<$/attribute$>$ .. \\
\>$<$/tuple$>$ .. \\
$<$/fragment$>$
\end{tabbing}
\end{example}



==> smwp/smwp_incremental-dd.tex <==
Once fragments and pages have been created, later fragment modifications need to be propagated to dependent fragment classes and affected page classes to modify their data accordingly. 
A fragment class is dependent on another fragment class if the former contains a tuple of the latter as a replica or if a tuple's membership in the former depends on the existence of a ``joining'' tuple in the latter (i.e., in the derivation base class). Furthermore, by mapping fragment classes to page classes, modifications on fragments need to be propagated to affected pages (i.e., those pages that contain the tuple serialized as XML).

In this section, we show how the algorithms presented in \cite{Schr02aIS,Schr01aADC} at the conceptual level for the maintenance of fragments' content can be implemented in a relational database setting by database triggers maintaining content relations. In addition we also present triggers for the maintenance of fragment relations. These triggers are extenders (in terms of \cite{Ceri00}) since they are generated automatically according to declaratively defined fragment classes to maintain their contents according to modifications of application relations.

With respect to the different kinds of relations that realize fragment classes and parameters, different kinds of triggers are distinguished as follows. {\it Content triggers} are defined on content relations to propagate modifications on fragments' content. {\it Serialization triggers} deal with update propagation from modified fragment classes to affected pages. They are defined on both content and fragmentation relations of fragment classes that are mapped to page classes. {\it Fragmentation triggers} are defined on both reference and fragmentation relations to propagate modifications on parameters and fragments to dependent fragmentation relations.

To provide for easy definition and maintenance of triggers, they are modularly designed in that each trigger propagates updates to a single dependent relation only. Such a relation is either a content or fragmentation relation of a fragment class that is defined upon the fragment class of the updated content relation (via its fragmentation or derivation base).
The benefits of this approach are as follows: 
(a) triggers are easily created by using a template, thus a small set of algorithm templates can be used irrespective of an actual fragmentation schema,
%(b) triggers as instantiations of algorithm templates perform better than triggers that use a generic algorithm (alternatively to a template), which would need to query meta data at runtime to determine dependent relations,
(b) triggers are easily added or deleted in case of new fragment classes are created or existing fragment classes are deleted.

Furthermore, to be able to use the same algorithm templates for fragmentation triggers on reference and fragmentation relations, their algorithms abstract from differences in structure and usage between reference and fragmentation relations.

To avoid a fragmentation schema's realization to influence legacy applications, newly created reference relations (such as {\sf RV\_Regions\_state}, cf. Example~\ref{RealizingCreatedReferenceRelation}) need particular attention. With the creation of a reference relation, a foreign key constraint is introduced on the according application relation referencing the reference relation to ensure data consistency. This brings up the problem of foreign key violations when legacy applications modify the application relation. Therefore, with the definition of a parameter that creates a new reference relation, a {\it synchronization trigger} is created on the application relation that keeps the contents of the reference relation synchronized.

\begin{sidewaysfigure}
    \begin{center}
        \includegraphics[scale=1.3]{\smwpdir figure-4}
        \caption{Realization of Incremental Push-Based Data Delivery}
        \label{TriggerArchitecture}
    \end{center}
\end{sidewaysfigure}

In short, modifications on content, fragmentation, and parameters are propagated incrementally by database triggers to maintain actual fragmentation and web pages. For each primary fragment class one content trigger (on the fragmentation base class' content relation) and several fragmentation triggers (one on the fragmentation base class' fragmentation relation and one on each introduced parameter's reference relation) propagate modifications. For each derived fragment class two content triggers (one on each of the fragmentation and derivation base class' content relation) and two fragmentation triggers (one on each of the fragmentation and derivation base class' fragmentation relation) propagate modifications. To maintain web pages according to database modifications, two serialization triggers are created (one on the fragment class' content relation and one on its fragmentation relation) for each fragment class that is mapped to at least one page class. They propagate modifications to affected pages. 

\begin{example}
    Figure~\ref{TriggerArchitecture} depicts the realization of incremental push-based data delivery of the wine shop's fragmentation and page content schema by content, fragmentation and serialization triggers.
\end{example}

% ############################################################
%
% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~

\subsection{Maintaining Primary Fragment Classes}
\label{PropOfModToPrimaryFCs}

With the definition of primary fragment class {\it G$<$KL$>$} upon fragmentation base class {\it F$<$L$>$}, using selection predicate $p$, and parameters $KL$, which are defined upon root fragment class {\it E$<>$}, a new content trigger on $FC\_F\_L$, a new fragmentation trigger on $FR\_F\_L$, and a new fragmentation trigger on $RV\_E\_K_i$ for each  $K_i$$\in$$K$ are created as described in the following.

\subsubsection{Content Trigger}
\label{PrimaryCT}

First, a content trigger is created on the content relation of the fragmentation base class (i.e., on $FC\_F\_L$) to propagate modifications thereon to the content relation of the primary fragment class (i.e., $FC\_G\_KL$), considering the selection predicate. Its algorithm template is described in this section.

Algorithm templates are depicted by pseudo-code mixed with SQL statements throughout the chapter. 
For better readability placeholders and variables are denoted in italics.
While placeholders are replaced by actual values when the template is instantiated to implement a trigger, %(i.e., at compile time)
actual values of variables are determined at run time. Variables $old$ and $new$ are used in all templates. They are bound to the old and new tuple values as defined by SQL and are thus called bindings. For a concise presentation of the templates, we make use of the following abbreviations: 
(a) $X$=$Y$ is used to test two sets of attributes $X$ and $Y$ that both comprise the same attributes $a_1..a_n$ for equality of their respective attribute values (i.e., to test whether $X.a_1$=$Y.a_1$$\wedge$$..$$\wedge$$X.a_n$=$Y.a_n$),
(b) analogously the same applies for testing inequality by $X$$\neq$$Y$, 
(c) in SQL Update statements ``UPDATE ... SET $X$=$Y$'' is used to set attributes $X.a_1$=$Y.a_1 .. X.a_n$=$Y.a_n$, and 
(d) whenever a variable that comprises a set of attributes (e.g., binding $new$) is used without further specification of attributes it refers to all attributes (e.g., $new$ refers to $new.a_1,..,new.a_n$). 

The algorithm template for content triggers for primary fragment classes distinguishes the following three cases:
(a) If a tuple is inserted (line \lnnum{4}) and the tuple selection predicate applies ($X'$ denotes $X$$\setminus$$KL$) as well as the fragment selection predicate applies (lines \lnnum{5}), the tuple is inserted into the primary fragment class (line \lnnum{6}). 
(b) If a tuple is updated (line \lnnum{7}), selection predicates for the old (line \lnnum{8}) and new tuple (line \lnnum{9}) are determined. If both the old and new tuple qualify for fragments of the primary fragment class (line \lnnum{10}), the affected tuple is either updated if the fragment it is contained in remains identical (lines \lnnum{11} and \lnnum{12)}, or deleted and inserted if the fragment changes (lines \lnnum{13} to \lnnum{15}). If the tuple does not qualify for any fragment of the primary fragment class any longer, it is deleted (lines \lnnum{16} and \lnnum{17}). Vice versa, if the tuple newly qualifies for a fragment, it is inserted (lines \lnnum{18} and \lnnum{19}). 
(c) If a tuple is deleted (\lnnum{20}) and it qualified for a fragment of the primary fragment class (line \lnnum{21}), it is deleted therefrom as well (line \lnnum{22}).

%\begin{alg}
\begin{tabbing}
\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \kill
%\lnnum{1}\>TRIGGER {\sf CT\_}{\it FC\_F\_L}{\sf -To-}{\it FC\_G\_KL} \\
\lnnum{1}\>TRIGGER {\sf CT\_FragBaseToPrimaryFC-}{\it FC\_G\_KL} \\
\lnnum{2}\>AFTER INSERT OR UPDATE OR DELETE ON $FC\_F\_L$ \\
\lnnum{3}\>FOR EACH ROW \\
%
\lnnum{4}\>\>\keyw{if} INSERTING \\
\lnnum{5}\>\>\>\keyw{if} $p_T(new.X')$ AND p$_F($new.$KL)$ \\
\lnnum{6}\>\>\>\>INSERT INTO $FC\_G\_KL$ VALUES $new$; \\
%
\lnnum{7}\>\>\keyw{if} UPDATING \\
\lnnum{8}\>\>\>$p_{old}$:=$p_T(old.X')$ AND $p_F(old.KL)$; \\
\lnnum{9}\>\>\>$p_{new}$:=$p_T(new.X')$ AND $p_F(new.KL)$; \\
\lnnum{10}\>\>\>\keyw{if} $p_{old}$ AND  $p_{new}$ \\
\lnnum{11}\>\>\>\>\keyw{if} $old.K$=$new.K$ \\ 
\lnnum{12}\>\>\>\>\>UPDATE $FC\_G\_KL$ AS G SET G.$X$=$new.X$ \\
          \>\>\>\>\>\>WHERE G.$\phi_G$=$old.\phi_G$; \\
\lnnum{13}\>\>\>\>\keyw{if} $old.K$$\neq$$new.K$ \\
\lnnum{14}\>\>\>\>\>DELETE FROM $FC\_G\_KL$ AS G WHERE G.$\phi_G$=$old.\phi_G$; \\
\lnnum{15}\>\>\>\>\>INSERT INTO $FC\_G\_KL$ VALUES $new$; \\
%
\lnnum{16}\>\>\>\keyw{if} $p_{old}$ AND NOT $p_{new}$ \\
\lnnum{17}\>\>\>\>DELETE FROM $FC\_G\_KL$ AS G WHERE G.$\phi_G$=$old.\phi_G$; \\
%
\lnnum{18}\>\>\>\keyw{if} NOT $p_{old}$ AND $p_{new}$ \\
\lnnum{19}\>\>\>\>INSERT INTO $FC\_G\_KL$ VALUES $new$; \\
%
\lnnum{20}\>\>\keyw{if} DELETING \\
\lnnum{21}\>\>\>\keyw{if} $p_T(old.X')$ AND $p_F(old.KL)$ \\
\lnnum{22}\>\>\>\>DELETE FROM $FC\_G\_KL$ AS G WHERE G.$\phi_G$=$old.\phi_G$;
\end{tabbing}
%\end{alg}

\begin{example}
   With the definition of primary fragment class {\sf Prem\-Wineries$<$region$>$}, which is defined upon fragmentation base class {\sf Prem\-Wineries$<>$}, a content trigger is created on {\sf FC\_Wineries} to propagate modifications to {\sf FC\_Prem\-Wineries\_region}. 
\end{example}

\subsubsection{Fragmentation Trigger}
\label{PrimaryFT}

Second, a fragmentation trigger is created on each relation $S_i$$\in$$S$, where $S$ is the set of reference and fragmentation relations, $FR\_G\_KL$ depends on. $S$ comprises reference relations $RV\_E\_K_i$ for each parameter $K_i$$\in$$K$ and fragmentation relation $FR\_F\_L$ if {\it $|$L$|$$>$$0$}. By abstracting from differences in structure and usage between reference and fragmentation relations, the same algorithm template is used for fragmentation triggers on reference relations as well as fragmentation triggers on fragmentation relations.

In the following the algorithm template for fragmentation triggers for primary fragment classes is described. Insert, Update, and Delete SQL Statements on reference and fragmentation relations reflect creation, modification, and deletion of fragments, activating fragmentation triggers. Such a trigger is created on each relation $S_i$$\in$$S$. Variable $S'$, which is used in the template, is defined by $S$$\setminus$$S_i$. In case of fragment modification or deletion (line \lnnum{4}), fragments of the primary fragment class that show corresponding parameter values are deleted (line \lnnum{5}). In case of fragment modification or creation (line \lnnum{6}), 
%relations $FR\_G\_KL$ depends on other than $R_0$ are determined (line \lnnum{7}), and 
new fragments are determined by building the cartesian product of the new parameter value by the domains of the remaining parameters and inserted if the fragment selection predicate applies (line \lnnum{7}). Note that the modification of a fragment's parameters causes the creation and deletion of fragments.

%{\sf \footnotesize 
\begin{tabbing}
\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \kill
%\lnnum{1}\>TRIGGER {\sf FT\_}$S_i${\sf -To-}{\it FR\_G\_KL} \\
\lnnum{1}\>TRIGGER {\sf FT\_FragBase-$S_i$-ToPrimaryFC-}{\it FR\_G\_KL} \\
\lnnum{2}\>BEFORE INSERT OR UPDATE OR DELETE ON $S_i$ \\
\lnnum{3}\>FOR EACH ROW \\
%
\lnnum{4}\>\>\keyw{if} UPDATING OR DELETING \\
\lnnum{5}\>\>\>DELETE FROM $FR\_G\_KL$ WHERE $\phi_{S_i}$=$old.\phi_{S_i}$; \\
%
\lnnum{6}\>\>\keyw{if} UPDATING OR INSERTING \\
%\lnnum{7}\>\>\>$S'=\{R_i | R_i \in S: R_i \neq R_0\}$ \\
\lnnum{7}\>\>\>INSERT INTO $FR\_G\_KL$ \\
\>\>\>\>(SELECT $new.\phi_{S_i}$, $S'_1.\phi_{S'_1}$, .., $S'_n.\phi_{S'_n}$ FROM $S'_1$, .., $S'_n$ \\
\>\>\>\>\>WHERE $p_F$($new.\phi_{S_i}$, $S'_1.\phi_{S'_1}$, .., $S'_n.\phi_{S'_n}$));
\end{tabbing}
%}

\begin{example}
   Fragmentation relation {\sf FR\_Prem\-Wineries\_region} of primary fragment class {\sf Prem\-Wineries\-$<$region$>$} depends on reference relation {\sf RV\_\-Wineries\_\-region} (i.e., application relation {\sf Regions}) only. It does not depend on any fragmentation relation, because its fragmentation base class {\sf Wineries$<>$} is not parameterized.
   Therefore, a fragmentation trigger is created on {\sf RV\_\-Wineries\_\-region} only to propagate modifications to the domain of parameter {\sf region}.
\end{example}

% ############################################################
% #
% #
% ############################################################

\subsection{Maintaining Derived Fragment Classes}

With the definition of derived fragment class {\it G$<$KL$>$} upon fragmentation base class {\it F$<$L$>$} and derivation base class {\it H$<$K$>$}, a new content trigger on $FC\_F\_L$, a new content trigger on $FC\_H\_K$, a new fragmentation trigger on $FR\_F\_L$, and a new fragmentation trigger on $FR\_H\_K$ are created as described in the following.

\subsubsection{Content Triggers}
\label{DerivedCT}

Because the derived fragment class is defined upon, and thus dependent on, its fragmentation and derivation base class, a content trigger is created on $FC\_F\_L(X)$ and $FC\_H\_K(Y)$ to propagate modifications to $FC\_G\_KL(Z)$ (where $Z$$=$$X$$\cup$$K$). While the fragmentation base class provides contents to be held by the derived fragment class, the derivation base class defines how this data is to be further partitioned. Due to these different roles, content triggers on $FC\_F\_L$ and $FC\_H\_K$ have different algorithms.

First, the algorithm template for the content trigger that is created on the content relation of the fragmentation base class is described in the following. It distinguishes the following three cases:
(a) If a tuple is inserted (line \lnnum{4}) it is inserted into all fragments of the derived fragment class it qualifies for as well (line \lnnum{5}).
(b) If a tuple is updated (line \lnnum{6}) and the join attribute values did not change (line \lnnum{7}), tuples of the derived fragment class can be updated as well (line \lnnum{8}). If the join attribute values changed (line \lnnum{9}), fragments the tuple qualifies for change as well. Thus it is deleted from fragments it is contained in but no longer qualifies for (line \lnnum{10}), updated in fragments it is contained in and still qualifies for (line \lnnum{11}), and inserted into fragments it newly qualifies for (line \lnnum{12}). Remember that $old.L$ and $new.L$ never differ, because updates to $L$ would have been translated to according delete and insert statements by another trigger before (cf. Section~\ref{PrimaryCT}).
(c) If a tuple is deleted (line \lnnum{13}) it is deleted from all fragments of the derived fragment class it is contained in (line \lnnum{14}).

%{\sf \footnotesize
\begin{tabbing}
\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \kill
%\lnnum{1}\>TRIGGER {\sf CT\_}{\it FC\_F\_L}{\sf -To-}{\it FC\_G\_KL} \\
\lnnum{1}\>TRIGGER {\sf CT\_FragBaseToDerivedFC-}{\it FC\_G\_KL} \\
\lnnum{2}\>AFTER INSERT OR UPDATE OR DELETE ON $FC\_F\_L$ AS F \\
\lnnum{3}\>FOR EACH ROW \\
%
\lnnum{4}\>\>\keyw{if} INSERTING \\
\lnnum{5}\>\>\>INSERT INTO $FC\_G\_KL$ \\
\>\>\>\>(SELECT DISTINCT $new$, H.$K$ FROM $FC\_H\_K$ AS H \\
\>\>\>\>\>WHERE H.$J_H$=$new.J_F$); \\
%
\lnnum{6}\>\>\keyw{if} UPDATING \\
\lnnum{7}\>\>\>\keyw{if} $old.J_F$=$new.J_F$ \\
\lnnum{8}\>\>\>\>UPDATE $FC\_G\_KL$ AS G SET G.$X$=$new.X$ \\
\>\>\>\>\>WHERE G.$\phi_F$=$old.\phi_F$; \\
\lnnum{9}\>\>\>\keyw{if} $old.J_F$$\neq$$new.J_F$ \\
\lnnum{10}\>\>\>\>DELETE FROM $FC\_G\_KL$ AS G \\
\>\>\>\>\>WHERE G.$\phi_F$=$old.\phi_F$ AND G.$K$ NOT IN ( \\
\>\>\>\>\>\>SELECT $K$ FROM $FC\_H\_K$ WHERE $J_H$=$new.J_F$); \\
\lnnum{11}\>\>\>\>UPDATE $FC\_G\_KL$ AS G SET G.$X$=$new.X$ \\
\>\>\>\>\>WHERE G.$\phi_F$=$old.\phi_F$; \\
\lnnum{12}\>\>\>\>INSERT INTO $FC\_G\_KL$ \\
\>\>\>\>\>(SELECT DISTINCT $new$, $H.K$ FROM $FC\_H\_K$ AS H \\
\>\>\>\>\>\>WHERE H.$J_H$=$new.J_F$ AND NOT EXISTS ( \\
\>\>\>\>\>\>\>SELECT * FROM $FC\_G\_KL$ AS G \\
\>\>\>\>\>\>\>\>WHERE G.$\phi_F$=$new.\phi_F$ AND G.$K$=H.$K$)); \\
%
\lnnum{13}\>\>\keyw{if} DELETING \\
\lnnum{14}\>\>\>DELETE FROM $FC\_G\_KL$ AS G \\
\>\>\>\>WHERE G.$\phi_F$=$old.\phi_F$;
\end{tabbing}
%}

\begin{example}
   A content trigger is created on {\sf FC\_Wines} to propagate modifications thereon to {\sf FC\_Prem\-Wines\_region} of derived fragment class {\sf Prem\-Wines$<$region$>$} with fragmentation base {\sf Wines$<>$} and derivation base {\sf Prem\-Wineries$<$region$>$}. For example, the insertion of a new wine $w$ into {\sf FC\_Wines} entails the insertion of tuple $v$$=$$\pi_Z(t[${\sf producedBy$=$id$]$FC\_\-Wineries\_\-region}$)$ into {\sf FC\_Prem\-Wines\_region(Z)}, thus enriching the new wine with information about the region it is produced in.
\end{example}

Second, the algorithm template for the content trigger that is created on the content relation of the derivation base class is described in the following. It needs to detect upon a tuple modification whether another tuple contained in the same fragment has the same join attribute values as the tuple being modified. If not, tuples from the fragmentation base do no longer qualify for the derived fragment class and have to be removed. Thus this trigger needs to access bindings {\it old} and {\it new} as well as the content relation it is defined upon. However, while the bindings can only be accessed from row-level triggers (created as ``FOR EACH ROW''), the content relation can only be accessed from statement-level triggers (created as ``FOR EACH STATEMENT''), because for a row-level trigger the content relation is mutating and thus not accessible. Since a trigger can be either row-level or statement-level but not both, this problem needs to be solved specifically to SMWP.

%It is split up into two triggers that conceptually constitute one content trigger to circumvent the problem of not being able to read {\it mutating relations}, which would have occurred if only one trigger had been used.  Because all fragments of a fragment class are collected in one content relation, this relation is mutating from the viewpoint of a trigger that is triggered upon a tuple modification. 

The solution to the problem of mutating content relations is the following: 
(a) The content trigger is defined as a statement-level trigger (opposite to the other two content triggers {\sf CT\_FragBaseToPrimaryFC-}{\it $FC\_G\_KL$} and {\sf CT\_FragBaseToDerivedFC-}{\it $FC\_G\_KL$}) to be able to query the content relation,
(b) To achieve that the content trigger is triggered once for each modified tuple (i.e., to be able to use statement-level triggers instead of row-level triggers), all content triggers use cursors to modify several tuples by issuing a single SQL statement for each tuple being modified (and not a single SQL statement to modify several tuples as used in their algorithm templates for presentational purposes) and root fragment classes cannot be used as derivation base classes,
(c) An auxiliary trigger is used to make the bindings available to the content trigger. It is a row-level trigger that is triggered before a tuple modification and stores the bindings in an auxiliary relation, named {\sf SMWP\_Worktrace} (which is in NF$^2$). By these means the content trigger can read bindings $old$ and $new$ from {\sf SMWP\_Worktrace} as well as the modified content relation $FC\_H\_K$.

The algorithm template of the auxiliary trigger, which is triggered before each row is shown below. It inserts the following data into {\sf SMWP\_Worktrace}: the name of the derived fragment class to distinguish between potentially several derived fragment classes that have {\it H$<$K$>$} as derivation base class (needed by algorithm template {\sf CT\_DerivBaseToDerivedFC-}{\it FC\_G\_KL}, see later in this section) and bindings $old$ and $new$ where applicable.

%{\sf \footnotesize
\begin{tabbing}
\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \kill
%\lnnum{1}\>TRIGGER {\sf AT\_}{\it FC\_H\_K}{\sf -To-}{\it FC\_G\_KL} \\
\lnnum{1}\>TRIGGER {\sf AT\_DerivBaseToDerivedFC-}$FC\_G\_KL$ \\
\lnnum{2}\>BEFORE INSERT OR UPDATE OR DELETE ON $FC\_H\_K$ \\
\lnnum{3}\>FOR EACH ROW \\
%
\lnnum{4}\>\>\keyw{if} INSERTING \\
\lnnum{5}\>\>\>INSERT INTO {\sf SMWP\_Worktrace(fcName,old,new)} \\
\>\>\>\>VALUES (``$FC\_G\_KL$'', NULL, $new$); \\
\lnnum{6}\>\>\keyw{if} UPDATING \\ 
\lnnum{7}\>\>\>INSERT INTO {\sf SMWP\_Worktrace(fcName,old,new)} \\
\>\>\>\>VALUES (``$FC\_G\_KL$'', $old$, $new$); \\
\lnnum{8}\>\>\keyw{if} DELETING \\
\lnnum{9}\>\>\>INSERT INTO {\sf SMWP\_Worktrace(fcName,old,new)} \\
\>\>\>\>VALUES (``$FC\_G\_KL$'', $old$, NULL);
\end{tabbing}

The algorithm template of the content trigger, which is triggered after each statement, is shown below. Before performing any action, bindings $old$ and $new$ are read from {\sf SMWP\_Worktrace} where applicable (lines \lnnum{5}, \lnnum{10}, and \lnnum{19}). The algorithm distinguishes the following three cases:
(a) If a tuple is inserted into the derivation base (line \lnnum{4}) and no other tuple with the same join attribute values already exists in the same fragment (lines \lnnum{6}, \lnnum{7}), the tuples from the fragmentation base that additionally qualify for the derived fragment class are determined and inserted (line \lnnum{8}). 
(b) If a tuple is updated (line \lnnum{9}) and the values of the join attributes have changed (line \lnnum{11}), tuples from the fragmentation base may no longer or may newly qualify for fragments of the derived fragment class. In case no other tuple with the same join attribute values as the old ones exists in the same fragment (line \lnnum{12}, \lnnum{13}), the tuples that do no longer qualify are determined and deleted (line \lnnum{14}). In case no other tuple with the same join attribute values as the new ones existed in the same fragment before (lines \lnnum{15}, \lnnum{16}), tuples that additionally qualify are determined and inserted (line \lnnum{17}). Remember that $old.K$ and $new.K$ never differ, because updates to $K$ would have been translated to according delete and insert statements by another trigger before (cf. Section~\ref{PrimaryCT} and earlier in this section).
(c) If a tuple is deleted (line \lnnum{18}) and no other tuple with the same join attribute values exists in the same fragment (lines \lnnum{20}, \lnnum{21}), tuples from the fragmentation base do no longer qualify for fragments of the derived fragment class and are thus deleted (line \lnnum{22}).
Finally, temporary buffered bindings $old$ and $new$ are removed from relation {\sf SMWP\_Worktrace} (line \lnnum{23}).

%{\sf \footnotesize
\begin{tabbing}
\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \kill
%\lnnum{1}\>TRIGGER {\sf CT\_}{\it FC\_H\_K}{\sf -To-}{\it FC\_G\_KL} \\
\lnnum{1}\>TRIGGER {\sf CT\_DerivBaseToDerivedFC-}{\it FC\_G\_KL} \\
\lnnum{2}\>AFTER INSERT OR UPDATE OR DELETE ON $FC\_H\_K$ \\
\lnnum{3}\>FOR EACH STATEMENT \\
%
\lnnum{4}\>\>\keyw{if} INSERTING \\
\lnnum{5}\>\>\>SELECT {\sf new} INTO $new$ FROM {\sf SMWP\_Worktrace} \\
\>\>\>\>WHERE {\sf fcName}=``$FC\_H\_K$''; \\
\lnnum{6}\>\>\>SELECT COUNT(*) INTO $count^i$ FROM $FC\_H\_K$ AS H \\
\>\>\>\>WHERE H.$\phi_H$$\neq$$new.\phi_{H}$ AND H.$J_H$=$new.J_H$ AND H.$K$=$new.K$; \\
\lnnum{7}\>\>\>\keyw{if} $count^i$=0 \\
\lnnum{8}\>\>\>\>INSERT INTO $FC\_G\_KL$ \\
\>\>\>\>\>(SELECT *, $new.K$ FROM $FC\_F\_L$ WHERE $J_F$=$new.J_H$); \\
% 
\lnnum{9}\>\>\keyw{if} UPDATING \\
\lnnum{10}\>\>\>SELECT {\sf old}, {\sf new} INTO $old$, $new$ FROM {\sf SMWP\_Worktrace} \\
\>\>\>\>WHERE {\sf fcName}=``$FC\_H\_K$''; \\
\lnnum{11}\>\>\>\keyw{if} $old.J_H$$\neq$$new.J_H$ \\
%
\lnnum{12}\>\>\>\>SELECT COUNT(*) INTO $count^u_1$ FROM $FC\_H\_K$ AS H \\
\>\>\>\>\>WHERE H.$\phi_H$$\neq$$old.\phi_{H}$ AND H.$J_H$=$old.J_H$ AND H.$K$=$old.K$; \\
\lnnum{13}\>\>\>\>\keyw{if} $count^u_1$=0 \\
\lnnum{14}\>\>\>\>\>DELETE FROM $FC\_G\_KL$ \\
\>\>\>\>\>\>WHERE $K$=$old.K$ AND $J_F$=$old.J_H$; \\
%
\lnnum{15}\>\>\>\>SELECT COUNT(*) INTO $count^u_2$ FROM $FC\_H\_K$ AS H \\
\>\>\>\>\>WHERE H.$\phi_H$$\neq$$new.\phi_{H}$ AND H.$J_H$=$new.J_H$ AND H.$K$=$new.K$; \\
\lnnum{16}\>\>\>\>\keyw{if} $count^u_2$=0 \\
\lnnum{17}\>\>\>\>\>INSERT INTO $FC\_G\_KL$ \\
\>\>\>\>\>\>(SELECT *, $new.K$ FROM $FC\_F\_L$ WHERE $J_F$=$new.J_H$); \\
%
\lnnum{18}\>\>\keyw{if} DELETING \\
\lnnum{19}\>\>\>SELECT {\sf old} INTO $old$ FROM {\sf SMWP\_Worktrace} \\
\>\>\>\>WHERE {\sf fcName}=``$FC\_H\_K$''; \\
\lnnum{20}\>\>\>SELECT COUNT(*) INTO $count^d$ FROM $FC\_H\_K$ AS H \\
\>\>\>\>WHERE H.$\phi_H$$\neq$$old.\phi_{H}$ AND H.$J_H$=$old.J_H$ AND H.$K$=$old.K$; \\
\lnnum{21}\>\>\>\keyw{if} $count^d$=0 \\
\lnnum{22}\>\>\>\>DELETE FROM $FC\_G\_KL$ \\
\>\>\>\>\>WHERE $K$=$old.K$ AND $J_F$=$old.J_H$; \\
%
\lnnum{23}\>\>DELETE FROM {\sf SMWP\_Worktrace} WHERE {\sf fcName}=``$FC\_G\_KL$'';
\end{tabbing}
%}

\begin{example}
   To propagate modifications on {\sf PremWineries$<$region$>$} to derived fragment class {\sf PremWines$<$region$>$}, an auxiliary trigger and a content trigger are created on {\sf FC\_PremWineries\_region}. While the auxiliary trigger is triggered before each row and insert bindings $old$ and $new$ into relation {\sf SMWP\_Worktrace}, the content trigger is triggered after each statement and accesses content relation {\sf FC\_PremWineries\_region} and auxiliary relation {\sf SMWP\_Worktrace}.
\end{example}

% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~

\subsubsection{Fragmentation Triggers}
\label{DerivedFT}

Furthermore, one fragmentation trigger is created on the fragmentation relations of the fragmentation base class (i.e., $FR\_F\_L$ if $|${\it L}$|$$>$$0$) and one on the derivation base class (i.e., $FR\_H\_K$). These triggers propagate creations and deletions of fragments to $FR\_G\_KL$. They do not propagate modifications of fragments, because fragmentation triggers on reference relations (cf. the algorithm in Subsection~\ref{PrimaryFT}) translate updates on reference relations to equivalent creations and deletions of fragments as soon as they occur. Notice that derived fragment classes do not depend on any reference relation, because they do not introduce new parameters.

The algorithm template for fragmentation triggers for derived fragment classes is described in the following. It differs from the one presented in Subsection~\ref{PrimaryFT} in that $|S|$$\leq$$2$, because $S$ comprises $FR\_H\_K$ and possibly $FR\_F\_L$ only, and in that it does not need to treat updates to fragmentation relations for the reasons mentioned before. 
A fragmentation trigger is created on each relation $S_i$$\in$$S$. Variable $S'$, which is used in the template, is defined by $S$$\setminus$$S_i$ and may be empty.
The algorithm template distinguishes the following two cases: (a) If a fragment is deleted (line \lnnum{4}), fragments of the derived fragment class that have corresponding parameter values are deleted (line \lnnum{5}).
(b) If a fragment is created (line \lnnum{6}), new parameter values are determined by forming the cartesian product of the new parameter value by the domain of the other parameters and fragments are created (line \lnnum{7}).

%{\sf \footnotesize 
\begin{tabbing}
\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \kill
%\lnnum{1}\>TRIGGER {\sf FT\_}$S_i${\sf -To-}{\it FR\_G\_KL} \\
\lnnum{1}\>TRIGGER {\sf FT\_Frag/DerivBase-$S_i$-ToDerivedFC-}{\it FR\_G\_KL} \\
\lnnum{2}\>BEFORE INSERT OR DELETE ON $S_i$ \\
\lnnum{3}\>FOR EACH ROW \\
\lnnum{4}\>\>\keyw{if} DELETING \\
\lnnum{5}\>\>\>DELETE FROM $FR\_G\_KL$ \\
\>\>\>\>WHERE $\phi_{S_i}$=$old.\phi_{S_i}$; \\
\lnnum{6}\>\>\keyw{if} INSERTING \\
\lnnum{7}\>\>\>INSERT INTO $FR\_G\_KL$ \\
\>\>\>\>(SELECT $new.\phi_{S_i}$, $S'.\phi_{S'_1}$ FROM $S'_1$); 
\end{tabbing}
%}

\begin{example}
   Fragmentation relation {\sf FR\_Prem\-Wines\_region} of derived fragment class {\sf Prem\-Wines$<$region$>$} depends on fragmentation relation {\sf FR\_Prem\-Wineries\_region} of the derivation base class only, because fragmentation base class {\sf Wines$<>$} is not parameterized. Therefore the only fragmentation trigger created is the one on {\sf FR\_Prem\-Wineries\_region} to propagate modifications thereon to {\sf FR\_Prem\-Wines\_region}.
\end{example}

% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%
% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~

\subsection{Maintaining Page Classes}

Pre-generated pages contain contents drawn from a database and have therefore to be synchronized with it. For automatic synchronization, modifications to fragment's contents are propagated to pages, entailing equivalent modifications on XML serializations of tuples. Analogously modifications to fragmentation are propagated to pages, entailing equivalent modifications of XML serializations of fragments as well as the creation and deletion of pages.

A {\it fragmentation serialization-trigger} translates creations and deletions of fragments to equivalent operations on pages. It is created on fragmentation relation $FR\_F\_L$ if {\it F$<$L$>$} is mapped to at least one page class. Such a trigger iterates over all page classes the modified fragment class is mapped to. If the modified fragment class is the current page class' foundation fragment class, a page is either created (comprising existing empty fragments of mapped fragment classes) or deleted. Otherwise all existing pages the fragment is mapped to are determined by comparing parameter values, taking parameter maps (e.g., cf. Example~\ref{UseParameterMap}) into account, and a fragment is added (if not yet existent) or deleted thereon.
%by using {\sf L'} representing parameters {\sf L} in terms of {\sf K}. 

%{\sf \footnotesize \begin{tabbing}
%\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \kill
%TRIGGER {\it ST-FragmentationToPage-FR\_F\_L} \\
%AFTER INSERT OR DELETE ON $FR\_F\_L$ \\
%\lnnum{1}\>\>\keyw{for each} P$<$K$>$ $\in \mu($F$<$L$>)$ \\
%\lnnum{2}\>\>\>\keyw{if} INSERTING \\
%\lnnum{3}\>\>\>\>\keyw{if} F$<$L$>$ = $\beta($P$<$K$>)$ \\
%\lnnum{4}\>\>\>\>\>createXMLPage(P$<$K$>$, $new$) \\
%\lnnum{5}\>\>\>\>\keyw{else} \\
%\lnnum{6}\>\>\>\>\>\keyw{for each} k $\in$ dom(K) such that $\pi_{L'}($k$)$=$new$ \\
%\lnnum{7}\>\>\>\>\>\>createXMLFragment(P$<$K$>$, k, F$<$L$>$, $new$) \\
%\lnnum{8}\>\>\>\keyw{else if} DELETING \\
%\lnnum{9}\>\>\>\>\keyw{if} F$<$L$>$ = $\beta($P$<$K$>)$ \\
%\lnnum{10}\>\>\>\>\>deleteXMLPage(P$<$K$>$, $old$) \\
%\lnnum{11}\>\>\>\>\keyw{else} \\
%\lnnum{12}\>\>\>\>\>\keyw{for each} k $\in$ dom(K) such that $\pi_{L'}($k$)$=$old$ \\
%\lnnum{13}\>\>\>\>\>\>deleteXMLFragment(P$<$K$>$, k, F$<$L$>$, $old$)
%\end{tabbing}}

Besides modifications to fragmentation also modifications to fragments' content have to be propagated to pages. 
A tuple insert, update, or delete entails the according modification of affected pages. A {\it content serialization-trigger} is created on content relation $FC\_F\_L$ if {\it F$<$L$>$} is mapped to at least one page class. It propagates modifications to fragment's contents to affected pages. Because the logic of both serialization triggers basically corresponds to the algorithms presented in \cite{Schr02aIS}, the interested reader is referred to there for their algorithms.

\begin{example}
    A fragmentation serialization-trigger is created on {\sf FR\_Prem\-Wineries\_region} to propagate modifications on fragmentation to pages. Since fragment class {\sf Prem\-Wineries\-$<$region$>$} is the foundation fragment class of page class {\sf Prem\-Wines\-$<$region$>$}, pages are created or deleted whenever a tuple is inserted into or deleted from the fragmentation relation. 
Furthermore, a content serialization-trigger is created on {\sf FC\_Prem\-Wineries\_\-region} to propagate modifications on fragments' content to according pages.
\end{example}

Serialization triggers comprise extensive generic logic for translating operations on fragments to equivalent operations on pages, and are thus implemented in Java. They are loaded into and executed within the database and use Oracle's XML Parser \cite{OracleXDK} and Xalan's Serializer \cite{ApacheXalan} to perform operations on pages. To efficiently translate operations, serialization triggers need efficient access to fragmentation and page content schemas. Therefore auxiliary meta data relations are used to store this information. 

Operations on pages are carried out by a SAX \cite{Meggi00aXMLDev} filter in our prototype. The page to be modified is parsed by a SAX parser, which generates events for each recognized XML element. The filter listens to the event stream and passes events on to Xalan's Serializer, which constructs an XML document from its incoming event stream. If an event concerns an element that is to be modified, the filter modifies the event before passing it on. To efficiently identify elements that are to be modified, Oracle's {\sf rowid} attribute, which is a database wide unique identifier of a tuple, is stored along with each XML element that represents a tuple. After parsing the original page is replaced with the newly constructed one, thus reflecting the fragment modification. 

Summarizing the presented triggers, the following example shows the effects of modifying an application relation. The activation sequence of triggers is ordered by ascending numbers, however, the order may vary since the execution order of triggers created on the same relation may be undefined (in particular, step 1 and 2 may be interchanged).
%Example~\ref{exmp:act-seq-ins} shows the insertion and deletion of a tuple representing content, %Example~\ref{exmp:act-seq-joinmod} shows the modification of a tuple representing content, %, with and without modifying an attribute that serves as a join attribute in derived fragmentation, and %and Example~\ref{exmp:act-seq-param} shows the insertion, modification, and deletion of a tuple representing a parameter value.

%\begin{example}
%\label{exmp:act-seq-ins}
%When a a premium winery is {\em inserted} into relation {\sf Wineries} (i.e., when a tuple is inserted for which {\sf category=``premium''} applies), 
%1) content trigger {\sf CT-Frag\-Base\-To\-Primary\-FC-Prem\-Wineries\_region} inserts the winery into {\sf FC\_Prem\-Wineries\_region}, 
%2) auxiliary trigger {\sf AT\_Deriv\-Base\-To\-Derived\-FC-Prem\-Wines\_region} inserts the winery into {\sf SMWP\_Worktrace},
%3) the serialization trigger defined on {\sf FC\_PremWineries\_region} inserts the winery into the according page of page class {\sf Prem\-Wines$<$region$>$}, 
%4) content trigger {\sf CT-Deriv\-Base\-To\-Derived\-FC-Prem\-Wines\_region} inserts all wines that are produced by the inserted winery into {\sf FC\_Prem\-Wines\_region}, and
%5) the serialization trigger defined on {\sf FC\_Prem\-Wines\_region} inserts the wines into the according page of page class {\sf Prem\-Wines$<$region$>$}. If the value of the inserted tuple's attribute {\sf category} had been different from ``{\sf premium}'', nothing but an activation of trigger {\sf CT-Frag\-Base\-To\-Primary\-FC-Prem\-Wineries\_region} would have happened.
%When a premium winery is {\em deleted}, the activation sequence above applies as well, except that existing tuples contained in content relations and pages are deleted rather than newly inserted.
%\end{example}

%\begin{example}
%\label{exmp:act-seq-joinmod}
%When attribute {\sf id} of a premium winery is {\em modified}, basically the same activation sequence as shown in Example~\ref{exmp:act-seq-ins} applies, except that step 4) first deletes all tuples that joined with the winery before modification and second inserts tuples from {\sf FC\_Wines} that join with the winery after modification into {\sf FC\_Prem\-Wines\_region}. When an attribute other than {\sf id} of a premium winery is {\em modified}, the same activation sequence as shown in Example~\ref{exmp:act-seq-ins} applies again, except that existing tuples contained in content relations and pages are modified rather than newly inserted.
%\end{example}

\begin{example}
\label{exmp:act-seq-param}
When region ``South Australia" is {\em added} to the parameter domain of {\sf region}, i.e., when a tuple with ``{\sf saus}" as the value of attribute {\sf id} is inserted into application relation {\sf Regions} (cf. Figure~\ref{TriggerArchitecture}),
(1) one of the two fragmentation triggers defined on {\sf Regions} inserts the region into {\sf FR\_Prem\-Wineries\_region},
(1.1) the fragmentation trigger defined on {\sf FR\_Prem\-Wineries\_region} inserts the region into {\sf FR\_\-Prem\-Wines\_region},
(1.1.1) the serialization trigger defined on {\sf FR\_\-Prem\-Wines\_region} does not perform any action since the page the fragment is mapped to does not yet exist,
%creates an empty fragment of fragment class {\sf Prem\-Wines$<$region$>$} in the page created in step @,
(1.2) the serialization trigger defined on {\sf FR\_Prem\-Wineries\_region} creates page {\sf prem\-Wines$<$saus$>$} containing empty fragments {\sf prem\-Wineries\-$<$saus$>$} and {\sf prem\-Wines\-$<$saus$>$},
%
(2) the other one of the two fragmentation triggers defined on {\sf Regions} inserts the region into {\sf FR\_Regions\_id},
(2.1) the serialization trigger defined on {\sf FR\_Regions\_id} creates page {\sf regions$<$saus$>$} containing empty fragment {\sf regions$<$saus$>$},
%
(3) the content trigger defined on {\sf Regions} inserts the region into {\sf FC\_Regions\_id}, and finally
(3.1) the serialization trigger defined on {\sf FC\_Regions\_id} inserts the region into the page's fragment created in step 2.1.
%
When a region is {\em deleted}, the activation sequence above applies as well, except that pages, fragments, and tuples are deleted rather than newly created or inserted.
%
When a region is {\em updated}, a deletion and insertion of a region is performed by the fragmentation triggers defined on relation {\sf Regions}.
\end{example}

The number of triggers that are involved in incremental propagation upon a modification of an application relation by a legacy application depends on 
the kind of data being modified (i.e., contents, fragmentation, or parameters),
the fragmentation schema,
the page content schema,
and the modification itself (i.e., in which respect data is modified). 
Thus only a general statement can be made about the number of triggers involved as follows (for an empirical performance evaluation see \cite{Schr02aIS}):

\begin{itemize}
\item Upon modification of a fragment class {\it F$<$L$>$},
(a) one content trigger is involved per dependent fragment class {\it G$<$KL$>$}, possibly causing multiple modifications of {\it G$<$KL$>$}, e.g., when join attribute values in a derivation base class are modified, and
(b) one serialization trigger is involved if {\it F$<$L$>$} is mapped to at least one page class.
%
\item Upon modification of parameter $P$'s domain $dom(P)$, one fragmentation trigger is involved per fragment class {\it F$<$L$>$} that introduces parameter $P$, causing maximally $2$$*$$|dom(L$$\setminus$$P)|$ modifications of {\it FR\_F\_L} 
%if $|L$$\setminus$$P|$$>$$0$ 
(since an update of a parameter is translated to an according deletion and insertion of fragments).
%
\item Upon modification of the domain of fragment class {\it F$<$L$>$}'s parameter set $L$, 
(a) one fragmentation trigger is involved per dependent fragment class {\it G$<$KL$>$} causing maximally $|dom(K)|$ modifications of {\it FR\_G\_KL}, and
(b) one serialization trigger is involved if {\it F$<$L$>$} is mapped to at least one page class.
\end{itemize} 

==> smwp/smwp_index-intro.tex <==
The chapter gives a quick-tour of the Self-Maintaining Web Pages (SMWP) approach and its underlying concepts in Section~\ref{section:smwp-quicktour}. 
In particular, it briefly presents the concepts of fragmentation schemas for data fragmentation design and of page schemas for web page design. The interested reader is referred to \cite{Schr02aIS,Schr01aADC} for more detailed descriptions.
Subsequently, a novel language is presented in Section~\ref{SchemaDefinitionLanguage} that allows to easily define and maintain fragmentation and page schemas.

\section{A Quick Tour of the SMWP Approach}
\label{section:smwp-quicktour}
\input{smwp/smwp_quicktour}

\section{Schema Definition Language}
\label{SchemaDefinitionLanguage}
\input{smwp/smwp_sdl} 

==> smwp/smwp_index-realization.tex <==
The chapter shows how the SMWP approach can be realized using off-the-shelf relational database technology.
It describes the realization of statical aspects by the relational representation of fragments and the storage of pages in Sections~\ref{FragmentationSchema}. Next, it shows the realization of dynamical aspects by triggers that maintain fragments and pages in Section~\ref{IncrementalDD}.
Subsequently, Section~\ref{section:smwp.pbp} presents how the SMWP approach known from \cite{Schr02aIS,Schr01aADC} is extended by the concept of predicate-based parameters and how they are realized.
Finally, Section~\ref{section:smwp.performance-eval} describes the implemented prototype and presents results of a performance evaluation.

Several advantages are gained by employing the database system that
stores contents published on Web pages to realize the SMWP
approach. In particular, by using the same database system to also
store meta data (e.g., about fragmentation) and Web pages, as well
as to execute application code, the following advantages are
gained. First, no proprietary software other than the database
system itself has to be installed and maintained (opposed to
previous approaches). Second, access to database contents is more
efficient from inside the database than from outside, possibly
from a remote computer. Third, by using the same storage system
for relations, fragments, and pages, fragments and pages are
modified in the same transaction as the triggering modification of
a relation. Thereby modifications to several pages that were
caused by a single modification to a relation become ``visible''
at once, resulting in consistent pages any time
(contrarily, \cite{Labr00SIGMOD,Sind98WebDB,Yago00VLDB} do not deal with this aspect of
consistency). Fourth, database tuning techniques (such as
clustering) can be applied to meta data as well as database
contents.

\section{Relational Representation of Fragments and Pages}
\label{FragmentationSchema}
\input{smwp/smwp_frag-schema}

\section{Maintaining Fragments and Pages}
\label{IncrementalDD}
\input{smwp/smwp_incremental-dd}

\section{Predicate Based Parameters}
\label{section:smwp.pbp}
\input{smwp/smwp_pbparams}

\section{Performance Evaluation}
\label{section:smwp.performance-eval}
\input{smwp/smwp_benchmark}


==> smwp/smwp_pbparams.tex <==
Experience has shown that sometimes a fragment class cannot be parameterized as desired, since it would need a parameter that is not part of the class' schema. 
In such cases one would fall back to on the fly generation or use other less flexible page pre-generation techniques.
However, in many cases it is just sufficient to define a parameter on a derived attribute (i.e., an attribute whose value is derived from existing attributes). To provide for this kind of parameters, we introduce in this section the concept of {\it predicate based parameters} by extending our previous work and refer to parameters mentioned so far as {\it value based parameters}. Like the latter, predicate based parameters are defined upon root fragment classes to provide for reusable parameter definitions featuring consistent semantics.

Predicate based parameter $Q$ can be introduced for primary fragmentation and is defined by a set of label-predicate pairs, $Q$$=$$(l,q)$. If predicate $q_i$ applies for a given tuple, it is ``tagged'' with the according label $l_i$, thus enriching it with derived information. To determine the label of predicate based parameter $Q$ for tuple $t$, function $getLabel(Q,t)$ is used. For each tuple exactly one predicate must apply. The domain of a predicate based parameter is determined by the set of its labels. 

\begin{sidewaysfigure}
   \begin{center}
      \includegraphics[scale=1.2]{\smwpdir figure-5}
      \caption{Parameterized Fragmentation using Predicate Based Parameters}
      \label{ParameterizedFragmentation1}
   \end{center}
\end{sidewaysfigure}

\begin{example}
   The wine shops stores, additionally to wines, wineries, and regions, contents about wine magazines (class {\sf Magazine}), which publish annual rankings of newly available wines (ternary association {\sf Rankings}), as depicted on the left of Figure~\ref{ParameterizedFragmentation1}. It wants to provide web pages enlisting wines that have been ranked in given ranking categories Top20, 21-50, and 51-100. However, the schema of application relation {\sf Rankings(\underline{magazine,year,wine},rank)} (implementing UML association {\sf Rankings}) does not contain an attribute for ranking categories. To derive the latter from attribute {\sf rank}, a predicate based parameter {\sf rCateg} is defined upon {\sf Rankings$<>$} (as shown below). 
   
%    {\sf \footnotesize
    \begin{tabbing}
    \quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \kill
   CREATE PREDICATE BASED PARAMETER rCateg ON Rankings$<>$ \\
   \>PREDICATES \{(``Top20'', \{rank$<$21\}), (``21-50'', \{rank$>$20$\wedge$rank$<$51\}), \\
   \>\>(``51-100'', \{rank$>$50$\wedge$rank$<$101\}), (``other'', \{rank$>$100\})\};
   \end{tabbing}
%   }
\end{example}

The introduction of predicate based parameters slightly affects the definition of primary fragment classes and their content relations as presented in Subsection~\ref{RealizingPrimaryFragmentClasses} as follows. Primary fragment class {\it G$<$KLM$>$} with $FC\_G\_KLM(Y)$ is defined upon fragmentation base {\it F$<$L$>$} with $FC\_F\_L(X)$ using selection predicate {\it p}. The primary fragment class introduces, additionally to value based parameters {\it L} (where {\it $|$L$|$}$\geq$$0$ and $L$$\in$$X$), predicate based parameters $M$ (where {\it $|$M$|$}$\geq$$0$ and $M$$\cap$$X$=$\emptyset$).

\begin{example}
   Predicate based parameter {\sf rCateg} is used to define primary fragment class {\sf Rankings\-$<$rCateg$>$}, which partitions rankings into fragments according to ranking categories as defined by parameter {\sf rCateg} using fragmentation selection predicate {\sf rCateg$\neq$``other''} (as shown below).
   
%   {\sf \footnotesize
   \begin{tabbing}
   \quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \kill
   CREATE PRIMARY FRAGMENT CLASS Rankings$<$rCateg$>$ \\
   \>FRAGMENTATION BASE CLASS Rankings$<>$ \\
   \>FRAGMENT SELECTION PREDICATE \{rCateg$\neq$``other''\};
   \end{tabbing}
%   }
\end{example}

To smoothly integrate predicate based parameters into the presented realization of the SMWP approach, a predicate based parameter's label is stored, like a value based parameter, as part of a fragment's tuple to define the fragment it is contained in. Thereby fragment classes that do not introduce predicate based parameters can handle their parameters equally irrespective of whether they are value or predicate based. 

However, when primary fragment class $G$$<$$KLM$$>$ introduces predicate based parameters $M$, they are not part of the schema of the fragmentation base class' content relation $FC\_F\_L(X)$. To hold these parameters, schema $X$ is extended by $M$. Thereby the primary fragment class' content relation $FC\_G\_KLM$ has schema $Z$=$X$$\cup$$M$. While tuple selection predicate $p_T$ may still reference $X$$\setminus$$KL$, fragmentation selection predicate $p_F$ may only reference introduced predicate based parameter set $M$ additionally to $KL$.

\begin{example}
   Content relation {\sf FC\_Rankings\_rCateg} of primary fragment class {\sf Rankings\-$<$rCateg$>$} comprises attribute {\sf rCateg} additional to attributes of fragmentation base class {\sf Rankings$<>$}. 
   Finally, to provide web pages enlisting wines that have been ranked in a ranking category as defined by {\sf Rankings\-$<$rCateg$>$}, derived fragment class {\sf Wines\-$<$rCateg$>$} is defined upon fragmentation base {\sf Wines$<>$} and derivation base {\sf Rankings$<$rCateg$>$} (cf. Figure~\ref{ParameterizedFragmentation1}). Thereby fragment class {\sf Wines$<>$}, which comprises a single fragment, is partitioned according to the fragmentation of {\sf Rankings$<$rCateg$>$}. Thereafter, fragment class {\sf TopWines$<$rCateg$>$} is mapped to page class {\sf TopWines$<$rCateg$>$}, which is defined upon foundation fragment class {\sf Rankings$<$rCateg$>$}.
\end{example}

%
%{\footnotesize \sf
%\begin{tabbing}
%\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \kill
%\lnnum{3}\>\>CREATE DERIVED FRAGMENT CLASS Wines$<$rCateg$>$ \\
%\>\>\>FRAGMENTATION BASE Wines$<>$ \\
%\>\>\>DERIVATION BASE Rankings$<$rCateg$>$ \\
%\end{tabbing}
%}

Only the algorithm template {\sf CT\_FragBaseToPrimaryFC-}{\it FC\_G\_KL} presented in Subsection~\ref{PrimaryCT} needs to be slightly adapted to support predicate based parameters. It needs to be modified to determine the label of the tuple whose modification is to be propagated.
The remaining algorithm templates can be left unchanged for the following reasons: 
a) a content trigger in derived fragmentation can handle predicate based parameters like value based ones,
b) fragmentation triggers are robust to the introduction of predicate based parameters, because they abstract from differences between reference and fragmentation relations,
c) serialization triggers are concerned with incrementally modifying pages, thus they are not affected at all.

The adapted algorithm template for content triggers on the content relation of the fragmentation base class of a primary fragment class is shown below. The line numbers are identical with the line numbers of the original algorithm presented in Subsection~\ref{PrimaryCT}. Lines that are modified or newly inserted are marked by the symbol ``\lnnum{*}'', and opposed to original or modified lines, newly inserted lines are numbered alphabetically starting from ``\lnnum{a}'' (e.g., \lnnum{a*}). Basically, the algorithm considers predicate based parameters $M$ additionally to parameters $KL$. The actual label of $M$ for a given tuple is determined by function $getLabel$ (lines \lnnum{a*} through \lnnum{d*}). These labels are considered when dealing with parameters, e.g., when testing the selection predicate (line \lnnum{5*}), or when inserting a tuple (line \lnnum{6*}).

%{\sf \footnotesize
\begin{tabbing}
\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \kill
\lnnum{1}\>TRIGGER {\sf CT\_FragBaseToPrimaryFC-}{\it FC\_G\_KL} \\
\lnnum{2}\>AFTER INSERT OR UPDATE OR DELETE ON $FC\_F\_L$ \\
\lnnum{3}\>FOR EACH ROW \\
%
\lnnum{4}\>\>\keyw{if} INSERTING \\
\lnnum{a*}\>\>\>$m_{new}$:=$\prod_{i=1}^{|M|}getLabel(M_i,new)$ \\
\lnnum{5*}\>\>\>\keyw{if} $p_T(new.X')$ AND $p_F(new.KL$$\times$$m_{new})$ \\
\lnnum{6*}\>\>\>\>INSERT INTO $FC\_G\_KL$ VALUES $new$, $m_{new}$; \\
%
\lnnum{7}\>\>\keyw{if} UPDATING \\
\lnnum{b*}\>\>\>$m_{old}$:=$\prod_{i=1}^{|M|}getLabel(M_i,old)$ \\
\lnnum{c*}\>\>\>$m_{new}$:=$\prod_{i=1}^{|M|}getLabel(M_i,new)$ \\
\lnnum{8*}\>\>\>$p_{old}$:=$p_T(old.X')$ AND $p_F(old.KL$$\times$$m_{old}$) \\
\lnnum{9*}\>\>\>$p_{new}$:=$p_T(new.X')$ AND $p_F(new.KL$$\times$$m_{new}$) \\
%
\lnnum{10}\>\>\>\keyw{if} $p_{old}$ AND $p_{new}$ \\
\lnnum{11*}\>\>\>\>\keyw{if} $old.K$=$new.K$ AND $m_{old}$=$m_{new}$ \\ 
\lnnum{12}\>\>\>\>\>UPDATE $FC\_G\_KL$ AS G SET G.$X$=$new.X$ \\
\>\>\>\>\>\>WHERE G.$\phi_G$=$old.\phi_G$; \\
\lnnum{13*}\>\>\>\>\keyw{if} $old.K$$\neq$$new.K$ AND $m_{old}$$\neq$$m_{new}$ \\ 
\lnnum{14}\>\>\>\>\>DELETE FROM $FC\_G\_KL$ AS G WHERE G.$\phi_G$=$old.\phi_G$; \\
\lnnum{15*}\>\>\>\>\>INSERT INTO $FC\_G\_KL$ VALUES $new$, $m_{new}$; \\
%
\lnnum{16}\>\>\>\keyw{if} $p_{old}$ AND NOT $p_{new}$ \\
\lnnum{17}\>\>\>\>DELETE FROM $FC\_G\_KL$ AS G WHERE G.$\phi_G$=$old.\phi_G$; \\
%
\lnnum{18}\>\>\>\keyw{if} NOT $p_{old}$ AND $p_{new}$ \\
\lnnum{19*}\>\>\>\>INSERT INTO $FC\_G\_KL$ VALUES $new$, $m_{new}$; \\
%
\lnnum{20}\>\>\keyw{if} DELETING \\
\lnnum{d*}\>\>\>$m_{old}$=$\prod_{i=1}^{|M|}getLabel(M_i,old)$ \\
\lnnum{21*}\>\>\>\keyw{if} $p_T(old.X')$ AND $p_F(old.KL$$\times$$m_{old}) $ \\
\lnnum{22}\>\>\>\>DELETE FROM $FC\_G\_KL$ AS G WHERE G.$\phi_G$=$old.\phi_G$;
\end{tabbing}
%} 

==> smwp/smwp_quicktour.tex <==
We illustrate newly introduced concepts throughout the section by applying them to an exemplary online wine shop, whose conceptual model is depicted on the left hand side of Figure~\ref{tableSam} by an UML \cite{Rumb99aUML} model. The wine shop manages contents concerning wines on sale (class {\sf Wines}), the wineries they are produced by (class {\sf Wineries}), and regions the wineries are located in (class {\sf Regions}). A transformation of the UML model to a relational model is depicted in the middle of Figure~\ref{tableSam}. It comprises relations {\sf Wines}, {\sf Wineries}, and {\sf Regions} (primary keys are underlined, foreign keys in italics), which are referred to as {\it application relations} throughout the rest of the thesis' Part~\ref{part:1}.

\begin{sidewaysfigure}
%\begin{figure}[h]
    \begin{center}
        \includegraphics[scale=1.25]{\smwpdir figure-1}
        \caption{Simple Fragmentation}
        \label{tableSam}
    \end{center}
%\end{figure}
\end{sidewaysfigure}

\subsection{Data Fragmentation Design}

As mentioned before, the SMWP approach utilizes concepts from DDBS. In particular, the concepts of fragmentation and allocation are exploited  and extended.

\subsubsection{Simple Fragmentation}
\label{QTSimpleFragmentation}

To decompose relations into fragments, three different kinds of fragmentation, namely {\it horizontal fragmentation}, comprising {\it primary} and {\it derived} fragmentation, and {\it vertical fragmentation} as well as combinations thereof, called {\it mixed or hybrid fragmentation}, have been proposed \cite{Ceri84a,Ozsu99a}. In the following, we will focus on horizontal fragmentation, since the other kinds of fragmentation can be integrated straightforwardly in the same way.

{\it Primary fragmentation} builds subsets of the tuples (rows) of a relation or fragment, called the {\it fragmentation base}, by applying a {\it selection predicate} which must evaluate to true for the tuple to be part of the primary fragment. {\it Derived fragmentation} takes into account that in some cases the fragmentation of a relation cannot be based on a property of its own attributes, but is derived from another relation, called the {\it derivation base}.

%Notice that in our context, the three correctness rules for fragmentation in DDBS \cite{Ceri84a}, namely completeness, reconstruction, and disjointness, do not apply. Completeness and reconstruction are irrelevant since a physical image comprising the entire relation is always kept in the database, and disjointness has already been disputed by Meghini \cite{Megh91aTODS}.

\begin{example}
The wine shop wants to provide web pages, each enlisting wineries that are categorized as {\sf premium} and their wines of a given region (cf. Figure~\ref{tableSam}). Therefore primary fragments of {\sf Wineries} are defined for each region, e.g., primary fragment {\sf PremWineries\_rioj} builds a subset of application relation {\sf Wineries} by applying selection predicate {\sf category=``premium'' and region=``rioj''}, collecting all premium wineries that are located in {\sf Rioja}. Fragmentation of {\sf Wines} by regions cannot be based on a property of its own attributes, thus derived fragmentation is used to build subsets of {\sf Wines} according to the primary fragments of {\sf Wineries}, e.g., derived fragment {\sf PremWines\_rioj} builds a subset of {\sf Wines}, collecting all wines that are produced in {\sf Rioja} by a premium winery. Finally fragments are mapped to web pages, using a canonical mapping to serialize tuples as XML elements.
\end{example}

\subsubsection{Fragmentation Schema}
\label{QTFragmentationSchema}

The fragmentation approach as introduced for distributed databases \cite{Ceri84a,Ozsu99a} is rather inflexible and not fully adequate for its use in the web setting. If relations are split into logical fragments for presentation on web pages, the number of fragments will typically be large with each fragment being relatively small. Problems arise if the addition of a tuple gives rise to new fragments or if a relation should be partitioned alternatively according to some new criterion. For example, if wineries and wines of a new region are added to the product line of the wine shop, a new primary fragment of {\sf Wineries}, a new derived fragment of {\sf Wines}, and a new web page as well as the mapping knowledge for mapping these fragments to the web page must be defined.

This inflexibility is addressed by introducing {\it parameterized fragment classes}. Like similar objects are collected into classes in object-oriented design, similar fragments are collected into fragment classes. They define common characteristics of their fragments, such as selection predicate and schema. To define the contents held by fragments at the class level, fragment classes are parameterized. A fragment class comprises a fragment for each parameter value from the parameter domain. A fragment is created by instantiating a fragment class with a parameter value; it contains those tuples of some fragment of the fragmentation base class for which the selection predicate applies and that ``match'' the parameter's value.

\begin{example}
   Using fragment classes instead of fragments, the wine shop can define data fragmentation more easily. Figure~\ref{ParameterizedFragmentation} depicts the wine shop's fragment classes {\sf PremWineries$<$region$>$} and {\sf PremWines$<$region$>$} whose instances are created and maintained automatically, resembling the fragments depicted in Figure~\ref{tableSam}. Fragment class {\sf Regions$<$id$>$} is newly introduced, each of its fragments stores contents about a single region. Figure~\ref{ParameterizedFragmentation} uses UML and stereotypes to model fragment classes. Stereotype {\sf FC} marks fragment classes, {\sf frag-base} marks associations to fragmentation base classes, and {\sf deriv-base} marks associations to derivation base classes.
\end{example}

\begin{sidewaysfigure}
    \begin{center}
        \includegraphics[scale=1.25]{\smwpdir figure-2.eps}
        \caption{Parameterized Fragmentation}
        \label{ParameterizedFragmentation}
    \end{center}
\end{sidewaysfigure}

In order to treat application relations and fragment classes uniformly, we assume that an implicit fragment class with no parameters is defined for each application relation, which contains this relation as a single fragment. Because these fragment classes constitute the ``roots'' of a fragmentation schema, each possibly serving as a fragmentation base class, they are called {\it root fragment classes}.

\begin{example}
   As depicted in Figure~\ref{ParameterizedFragmentation}, root fragment classes {\sf Regions$<>$}, {\sf Wineries$<>$}, and {\sf Wines$<>$} represent application relations {\sf Regions}, {\sf Wineries}, and {\sf Wines}. They serve as fragmentation base classes for fragment classes {\sf Regions$<$id$>$}, {\sf PremWineries$<$region$>$}, and {\sf PremWines$<$region$>$}.
\end{example}

A modification of a relation has to be propagated to all fragment classes that contain the modified tuple as a replica. The SMWP approach provides algorithms for {\it propagating} these {\it modifications incrementally}. Thereby only the replicated tuples are modified, there is no need to regenerate fragments from scratch to reflect the modifications.

A brief introduction to primary and derived fragment classes is given in Section~\ref{SchemaDefinitionLanguage} along with the presentation of a schema definition language.

\subsection{Web Page Design}

Like similar fragments are collected into fragment classes, pages of the same kind are collected into page classes. A {\it page class} is specified by a {\it page schema}, comprising a {\it page content schema} and one or several {\it page presentation schemata}. Page classes comprising more than one page are defined with one or several parameters, where the parameter's values uniquely identify one page of the page class.

Bringing database contents to the web, fragments are allocated to web pages. Instead of defining this allocation for individual fragments and individual pages, fragment classes are mapped to one or several page classes. A page content schema defines among
others, which fragment classes are mapped to this page class. A page class then comprises one page for each fragment from a distinguished mapped fragment class, called the {\it foundation
fragment class}. Pages are pre-generated upon the definition of their page content schema. The contents of a page is determined by reading fragments of mapped fragment classes (including the foundation fragment class) and by transforming them into XML. We use a simple canonical mapping to serialize fragments and tuples therein as XML elements (cf. \cite{Schr01aADC}).

\begin{example}
The wine shop's page class {\sf PremWines$<$region$>$} is depicted in the right upper half of Figure~\ref{ParameterizedFragmentation}. As with fragment classes, UML stereotypes are used to model page classes in Figure~\ref{ParameterizedFragmentation}. Stereotype {\sf PC} marks page classes, {\sf foundation-fc} marks associations to foundation fragment classes, {\sf mapped-to} marks associations to mapped fragment classes, and {\sf link-to} marks links between page classes. Page class {\sf PremWines$<$region$>$} comprises a page for each fragment from its foundation fragment class {\sf PremWineries$<$region$>$}, containing a fragment from the latter and an according fragment of fragment class {\sf PremWines$<$region$>$}.
\end{example}

A modification of a fragment has to be propagated to all pages it is mapped to. Instead of re-generating affected pages completely, as previous approaches \cite{Chal00INFOCOM,Labr00SIGMOD,Sind98WebDB,Yago00VLDB} do, the SMWP approach incrementally modifies pages. Thereby only those XML elements of a page are modified that represent the modified tuple. As performance evaluations have shown \cite{Schr02aIS}, propagating modifications on fragments incrementally to pages generally outperforms re-generating pages from scratch.

For each page class one or several page presentation schemas define the presentation of its pages by the means of XSLT \cite{Clar99aW3C} or CSS \cite{W3C1998CSS2}. The separation of content from presentation is common practice and enables one to define several presentations for the same content to take different user capabilities and preferences into account.
Due to the focus of this chapter, we do not discuss page presentation schemas further but assume a default XSLT stylesheet that is used to format pages. 

==> smwp/smwp_sdl.tex <==
Definition and maintenance of fragmentation and page content schemas is supported by a declarative schema definition language, providing statements for creating, modifying, and deleting fragment classes and page classes. To realize fragmentation with off-the-shelf database technology, issued statements are translated into SQL-DDL and PL/SQL statements. How this is done in detail is described in later sections. In the following we give a brief overview of the language and shortly review the concepts of fragment classes. A full definition of the language in EBNF is presented in the Appendix.

\subsection{Data Fragmentation Design}
\label{SDLDbDesign}
A {\it primary fragment class} is defined upon a {\it fragmentation base class}. It comprises fragments and tuples therein that are taken over from the fragmentation base class. A primary fragment class ``inherits'' the parameters of its fragmentation base class and possibly adds new parameters. If a new parameter is added, fragments from the fragmentation base class are further partitioned according to the added parameter, where the number of sub-partitions is defined by the domain of the added parameter. 

A selection predicate can be used in the definition of a primary fragment class to narrow the contents that is taken over from the fragmentation base class. First, a {\it fragment selection predicate} can be used to narrow the set of fragments that are taken over. It is specified by an SQL expression that may only refer to parameters of the fragment class. Second, a {\it tuple selection predicate} can be used to narrow the set of tuples contained in fragments that are taken over. Again, it is specified by an SQL expression, but this time it may only refer to tuple's attributes that are not used as parameters.

The statement to define a primary fragment class has the following syntax\footnote{In the following {\it F$<$$>$}, {\it F$<$L$>$}, {\it G$<$KL$>$}, {\it H$<$K$>$}, and {\it P$<$K$>$} are variables. {\it P$<$K$>$} conforms to non-terminal symbol {\em PCSignature}, while the others conform to non-terminal symbol {\em FCSignature}.}:
% conforming to non-terminal symbol {\em FCSignature},  conforms to {\em PCSignature}}:
\begin{minipage}[t]{\textwidth}
%   {\sf \footnotesize
   \begin{tabbing}
   \quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \kill
   CREATE PRIMARY FRAGMENT CLASS {\it G$<$KL$>$} \\
   \>FRAGMENTATION BASE CLASS {\it F$<$L$>$} \\
   \>[ FRAGMENT SELECTION PREDICATE {\it SQLExpr} ] \\
   \>[ TUPLE SELECTION PREDICATE {\it SQLExpr} ].
   \end{tabbing}
%   }
\end{minipage} \\

%\example To partition application relation $Region$ into fragments, where for each region a fragment exists that comprises detailed information about the respective region, primary fragment class {\sf Regions$<$id$>$} is defined upon fragmentation base {\sf Regions$<>$}, adding parameter {\sf id}.
%{\footnotesize \sf 
%\begin{tabbing}
%\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \kill
%\lnnum{1}\>\>CREATE PRIMARY FRAGMENT CLASS Region$<$id$>$ \\
%\>\>\>FRAGMENTATION BASE Region$<>$ \\
%\end{tabbing}}

\begin{example} 
\label{CreatePrimaryFC}
To partition relation {\sf Wineries} into fragments, where for each region a fragment exists that comprises all premium wineries of the respective region, primary fragment class {\sf Prem\-Wineries\-$<$region$>$} is defined upon fragmentation base {\sf Wineries$<>$} using tuple selection predicate {\sf category=``premium''}, adding parameter {\sf region} (as depicted in Figure~\ref{ParameterizedFragmentation} and shown below).
   
%   {\sf \footnotesize
   \begin{tabbing}
   \quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \kill
   CREATE PRIMARY FRAGMENT CLASS PremWineries$<$region$>$ \\
   \>FRAGMENTATION BASE CLASS Wineries$<>$ \\
   \>TUPLE SELECTION PREDICATE \{category=``premium''\};
   \end{tabbing}
%   }
\end{example}

\begin{example}
   To illustrate the use of fragment selection predicates, imagine that {\sf PremWineries$<$region$>$} should only contain wineries from regions starting with the letter ``A''. To accomplish this, one would append the fragment selection predicate clause ``FRAGMENT SELECTION PREDICATE \{region LIKE `A\%'\}'' to the statement shown in Example~\ref{CreatePrimaryFC}.
\end{example}

A {\it parameter} must be defined before it can be used by a primary fragment class. Parameters become re-usable by defining them on root fragment classes. Once defined on a root fragment class, they can be used in the definition of any primary fragment class that is defined directly or indirectly via its fragmentation base classes upon the root fragment class. Furthermore, to achieve independence of a parameter's domain from the contents of the root fragment class upon which it is defined, the values of the primary key attribute of a {\it reference relation} keep the values of the parameter's domain. The statement to define a parameter has the following syntax:

%{\sf \footnotesize
\begin{tabbing}
\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \kill
CREATE VALUE BASED PARAMETER {\it Ident} ON {\it F$<>$} \\
\>((USE REFERENCE RELATION {\it Ident}({\it Ident})) $|$ \\
\>(CREATE REFERENCE RELATION)).
\end{tabbing}
%}

\begin{example}
   \label{CreateParameter}
   Parameter {\sf region} must be defined upon root fragment class {\sf Wineries$<>$}, before it can be used in the definition of primary fragment class {\sf PremWineries$<$region$>$} (cf. Example~\ref{CreatePrimaryFC}). Because attribute {\sf region} of {\sf Wineries$<>$} references the primary key attribute {\sf id} of application relation {\sf Regions}, the latter is used as the reference relation to define the parameter's domain (as shown below).
   
%   {\sf \footnotesize
   \begin{tabbing}
   \quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \kill
   CREATE VALUE BASED PARAMETER region ON Wineries$<>$ \\
   \>USE REFERENCE RELATION Regions(id);
   \end{tabbing}
%   }
\end{example}

When defining a parameter two special cases may occur. First, the application relation of the root fragment class the parameter is defined upon may be used as the parameter's reference relation itself. This is possible if the parameter's domain is defined by the values of the primary key attribute of this application relation.

\begin{example}
\label{UseReferenceRelation2}
   Parameter {\sf id} must be defined before it can be used in the definition of fragment class {\sf Regions$<$id$>$}. Because the values of primary key attribute {\sf id} of application relation {\sf Regions} define the parameter's domain, this application relation is used as the reference relation (as shown below).

%   {\sf \footnotesize
   \begin{tabbing}
   \quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \kill
   CREATE VALUE BASED PARAMETER id ON Regions$<>$ \\
   \>USE REFERENCE RELATION Regions(id);
   \end{tabbing}
%   }
\end{example}

The second special case occurs when for a given parameter no application relation can be used as a reference relation. This happens if all application relations have inappropriate primary key attributes. In this case a reference relation has to be created by using the {\sf CREATE REFERENCE RELATION} clause with the statement to create the parameter (as shown below).

\begin{example}
\label{CreateReferenceRelation}
   To illustrate this situation, imagine that parameter {\sf state} is defined upon root fragment class {\sf Regions$<>$} to be used in the definition of primary fragment class {\sf Regions$<$state$>$}. Because no application relation has an appropriate primary key attribute for {\sf state}, a new reference relation has to be created as shown below.

%   {\sf \footnotesize
   \begin{tabbing}
   \quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \kill
   CREATE VALUE BASED PARAMETER state ON Regions$<>$ \\
   \>CREATE REFERENCE RELATION;
   \end{tabbing}
%   }
\end{example}

A {\it derived fragment class} is defined upon a {\it fragmentation base class} and a {\it derivation base class}. It comprises fragments and tuples therein that are taken over from the fragmentation base class, where each fragment from the fragmentation base is further partitioned according to the derivation base. The number of sub-partitions is determined by the domain of the derivation base's parameters. The fragment into which a tuple from a fragment of the fragmentation base class belongs is determined by joining it with tuples from fragments of the derivation base class. The derived fragment class ``inherits'' the parameters of both its fragmentation and derivation base class. The statement to define a derived fragment class has the following syntax, where ``{\sf AS Ident}'' is used to define an alias (like in SQL) that can be used in {\it SQLExpr}:

%{\sf \footnotesize
\begin{tabbing}
\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \kill
CREATE DERIVED FRAGMENT CLASS {\it G$<$KL$>$} \\
\>FRAGMENTATION BASE CLASS {\it F$<$L$>$} [ AS {\it Ident} ] \\
\>DERIVATION BASE CLASS {\it H$<$K$>$} [ AS {\it Ident} ] \\
\>JOIN BY {\it SQLExpr}.
\end{tabbing}
%}

\begin{example}
   \label{CreateDerivedFC}
   Derived fragment class {\sf PremWines$<$region$>$} is defined upon fragmentation base class {\sf Wines$<>$} and derivation base class {\sf PremWineries$<$region$>$} (as depicted in Figure~\ref{ParameterizedFragmentation} and shown below). Thereby single fragment {\sf wines$<>$} is partitioned according to the fragments of {\sf PremWineries$<$region$>$}. The derived fragment class then comprises several fragments, each containing wines that were produced in the respective region by a premium winery (e.g., {\sf premWines$<$rioj$>$} contains wines that were produced in {\sf Rioja}).
   
%   {\sf \footnotesize
   \begin{tabbing}
   \quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \kill
   CREATE DERIVED FRAGMENT CLASS PremWines$<$region$>$ \\
   \>FRAGMENTATION BASE CLASS Wines$<>$ AS wines \\
   \>DERIVATION BASE CLASS PremWineries$<$region$>$ AS premWineries \\
   \>JOIN BY \{wines.producedBy=premWineries.id\};
   \end{tabbing}
%   }
\end{example}

%
% WEB DESIGN
%
\subsection{Web Page Design}

The page content schema defines page classes and the mapping of fragment classes to page classes. A {\it page class} is defined upon a foundation fragment class, which must possess the same parameters as the page class. For each fragment of the foundation fragment class, a page containing the fragment is created. Furthermore other fragment classes can be mapped to a page class, whereas the mapped fragment classes' parameters must be a subset or equal the page class' parameters. The statement to define a page class has the following, shortened syntax, where non-terminal symbol {\it PCFCMapping} details the mapping of a fragment class (see the Appendix and later explanations in this section):

%{\sf \footnotesize
\begin{tabbing}
\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \kill
CREATE PAGE CLASS {\it P$<$K$>$} \\
\>FOUNDATION FRAGMENT CLASS {\it PCFCMapping} \\
\>\{ FRAGMENT CLASS {\it PCFCMapping} \}.
%\\ \>\>{\it PCFCMapping} := {\it FCSignature} $[$ AS {\it Ident}$]$ $[${\it ParameterMap}$]$..
\end{tabbing}
%}

\begin{example}
   \label{UseParameterMap}
   Page class {\sf Regions$<$region$>$} is defined upon foundation fragment class {\sf Regions$<$id$>$} (as shown below). A parameter map ({\sf PARAMETER MAP} clause as defined by {\it PCFCMapping}) defines the parameter {\sf id} of the foundation fragment class to equal parameter {\sf region} of the page class. The page class then comprises a page for each fragment of fragment class {\sf Regions$<$id$>$}.
   
%   {\sf \footnotesize
   \begin{tabbing}
   \quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \kill
   CREATE PAGE CLASS Regions$<$region$>$ \\
   \>FOUNDATION FRAGMENT CLASS Regions$<$id$>$ \\
   \>\>PARAMETER MAP id AS region;
   \end{tabbing}
%   }
\end{example}

When defining a page content schema it is possible to specify links between fragment classes (with symbol {\it PCFCMapping}), which are either mapped to the same page class (internal link) or different page classes (external link). Such meta data about links is used during the formatting process for proper nesting of fragments contained in the same page and determining links between pages.

\begin{example}
   Page class {\sf PremWines$<$region$>$} is defined upon foundation fragment class {\sf Prem\-Wineries\-$<$region$>$} and fragment class {\sf Prem\-Wines\-$<$region$>$} (as shown below). Each tuple of {\sf PremWineries$<$region$>$} links internally to corresponding tuples of {\sf PremWines$<$region$>$} (as specified by the {\sf INTERNAL LINK} clause), and externally to a fragment of fragment class {\sf Regions$<$id$>$} contained in a page of page class {\sf Regions$<$region$>$} (as specified by the {\sf EXTERNAL LINK} clause). Link targets, which are specified at the class level, are determined at the instance level as defined by the {\sf \footnotesize JOIN BY} clause.
   
%   {\sf \footnotesize
   \begin{tabbing}
   \quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \=\quad \kill
   CREATE PAGE CLASS PremWines$<$region$>$ \\
   \>FOUNDATION FRAGMENT CLASS PremWineries$<$region$>$ \\
   \>\>\>AS premWinery \\
   \>\>INTERNAL LINK TO FRAGMENT CLASS PremWines$<$region$>$ \\
   \>\>\>\>AS premWines \\
   \>\>\>JOIN BY \{premWines.producedBy=premWinery.id\} \\
   \>\>EXTERNAL LINK TO PAGE CLASS Regions$<$region$>$ AS pc\_region \\
   \>\>\>CONTAINING FRAGMENT CLASS Regions$<$id$>$ AS fc\_region \\
   \>\>\>JOIN BY \{premWinery.region=pc\_region.region \\
   \>\>\>\>\>AND premWinery.region=fc\_region.id\} \\
   \>FRAGMENT CLASS PremWines$<$region$>$;
   \end{tabbing}
%   }
\end{example} 
